Pitfalls in Language Models for Code Intelligence: A Taxonomy and Survey

Modern language models (LMs) have been successfully employed in source code generation and understanding, leading to a significant increase in research focused on learning-based code intelligence, such as automated bug repair, and test case generation. Despite their great potential, language models for code intelligence (LM4Code) are susceptible to potential pitfalls, which hinder realistic performance and further impact their reliability and applicability in real-world deployment. Such challenges drive the need for a comprehensive understanding - not just identifying these issues but delving into their possible implications and existing solutions to build more reliable language models tailored to code intelligence. Based on a well-defined systematic research approach, we conducted an extensive literature review to uncover the pitfalls inherent in LM4Code. Finally, 67 primary studies from top-tier venues have been identified. After carefully examining these studies, we designed a taxonomy of pitfalls in LM4Code research and conducted a systematic study to summarize the issues, implications, current solutions, and challenges of different pitfalls for LM4Code systems. We developed a comprehensive classification scheme that dissects pitfalls across four crucial aspects: data collection and labeling, system design and learning, performance evaluation, and deployment and maintenance. Through this study, we aim to provide a roadmap for researchers and practitioners, facilitating their understanding and utilization of LM4Code in reliable and trustworthy ways.

==> sections/backup.tex <==


\section{Data Collection and Labeling}
\label{sec:data}
The data-hungry language models require large-scale and high-quality training datasets.
According to a survey by Hou~\ea~\cite{hou2023large}, the majority of LMs for code intelligence are trained using data from open-source platforms, with GitHub and StackOverflow being the most popular options.
However, the data in these platforms are user-contributed, varying significantly in the level of quality and reliability.
It leads to non-negligible noises, bias, and errors in the training dataset and further affects the behavior of the models, which brings significant pitfalls in LMs for code intelligence. 
In this section, we provide a brief description of related studies and discuss the implications and potential solutions during the data collection and labeling stages. 

% Similar to other learning-based systems, LM4Code-based systems require a representative and high-quality dataset.
% According to a survey by Hou~\ea\cite{hou2023large}, the majority of reviewed papers on LMs for software engineering obtained their data from open-source platforms, with GitHub and StackOverflow being the most popular options.
% These platforms serve as rich repositories of authentic developer interactions, code snippets, solutions, and challenges.
% As abundant as these resources are, data collected from these sources often exhibit noise, errors, and inaccuracies~\cite{shi2022we}.
% This is because the data is often unstructured and unlabeled~\cite{tantithamthavorn2015impact}. Additionally, the data may be biased towards certain programming languages, frameworks, or domains.
% Employing language models on such unrealistic data may amplify these issues.
% Additionally, they can lead to unreliable evaluation results.
% In this section, we thus provide a brief description of current research, and discuss the implications and potential solutions of biases and pitfalls that emerge during the data collection and labeling stages.

\input{tables/yy_tables/tab1_data_bias_summary}

\subsection{RQ1-Pitfalls}

From the collected papers, we identified 11 research studies focusing on pitfalls during the data collection and labeling process.
Table~\ref{tab:bias_in_data_collection} presents the statistics of literature on this topic, where the pitfalls can be grouped into three main categories.

\noindent \textbf{Unbalanced Distribution:} 
Unbalanced distribution arises when there is a lack of proper randomization in the selection of samples, leading to certain populations being underrepresented or overrepresented~\cite{shahbazi2023representation}.
In code-related scenarios, it usually refers to the gap between the sample distribution of real-world practices and training datasets.
For example, as emphasized by~\cite{chakraborty2021deep, yang2023does, steenhoek2023empirical}, vulnerable instances in vulnerability detection studies are overwhelming while neutral code instances in real-world environments considerably outnumber their vulnerable counterparts.
This imbalance extends to other code-based tasks.
In software defect prediction, where defective modules are scarce compared with non-defective cases in real-world environments~\cite {yedida2021value,li2022robust}.
Similarly, bug report classification suffers from underrepresentation of the minority bug class~\cite{li2022robust}.

% RobustTrainer~\cite{li2022robust} was proposed to effectively tackle the mislabelling and class imbalance issues and produces significantly better deep predictive models compared to the other six comparison approaches
% \su{Introduce \cite{yedida2021value} and \cite{li2022robust}, one sentence for each.}



% In the development of learning-based systems, particularly those related to code intelligence, an ideal dataset would closely resemble the actual underlying distribution of the input space~\cite{arp2022and}.
% However, the practical constraints of data collection often mean that researchers have to work with datasets that, while comprehensive, might not be a perfect representation of this ideal distribution.
% It is common knowledge that biases, particularly sampling biases, are inherent to many existing datasets.
% From our collected studies, five studies were identified that evaluated the impacts of sampling bias on the efficacy and reliability of LMs for code intelligence.
% For example, three studies~\cite{chakraborty2021deep, yang2023does, steenhoek2023empirical} emphasized the persistent class imbalance problems in vulnerability detection research. 
% They highlighted that in realistic vulnerability distribution scenarios, neutral code instances considerably outnumber their vulnerable counterparts. 
% This class imbalance challenge is also spotlighted in automated bug report classification and defect prediction by~\cite{yedida2021value} and ~\cite{li2022robust}.
% However, comprehending the nature and extent of these biases is paramount to ensure reliable outcomes from trained models.

\noindent \textbf{Data Noise:} 
Data noises are the samples that are meaningless or even harmful for the models to learn, such as samples with deprecated coding conventions, multi-lingual comments, and auto-generated code snippets~\cite{shi2022we}.
Such noises widely exist in code datasets.
For example, as investigated by Sun~\ea~\cite{sun_importance_2022} and Shi~\ea~\cite{shi2022we}, over one-third of the popular code dataset, CodeSearchNet~\cite{husain2019codesearchnet}, are noises that are hardly seen in neural code search.
Their analysis results show that the examined datasets contain a multitude of noise categories, including unrelated comments, non-literal characters, and issues like empty or duplicated code.
Liu~\ea~\cite{liu2018neural} and Zhang~\ea~\cite{zhang2023slice} specifically investigated data noise in commit message generations, where approximately 16\% of the commit messages of benchmark dataset by Jiang et al.~\cite{jiang2017automatically} were identified as noises. 





% The domain of automated code tasks, especially when leveraging language models, relies heavily on the quality of training data. 
% Whether the task is mapping natural language to code or translating code segments into human-understandable descriptions, the reliability of the dataset is critical. 
% However, the unique nature of the software development landscape introduces various sources of noise into these datasets. 
% This includes variations in coding conventions, multi-lingual comments, auto-generated code snippets, and the somewhat unpredictable nature of software development processes~\cite{shi2022we}.
% This data noise can often mislead models into learning irrelevant patterns or establishing spurious correlations, distorting the actual information and hindering the training and evaluation of language models.
% In our examined studies, we found four research studies to explore data noise in LM-based code tasks.
% Liu~\ea~\cite{liu2018neural} and Zhang~\ea~\cite{zhang_slice-based_2023} specifically investigated data noise in commit message generations. 
% Particularly in the benchmark dataset by Jiang et al.~\cite{jiang2017automatically}, 
% approximately 16\% of the commit messages were identified as noise.
% This noise primarily stemmed from "bot messages" — automatically generated content by development tools — and "trivial messages", which, though human-written, provided redundant information that can be readily inferred from data points such as the list of changed files.
% Also, Sun~\ea~\cite{sun_importance_2022} and Shi~\ea~\cite{shi2022we} delved into the popular CodeSearchNet~\cite{husain2019codesearchnet} benchmark dataset for automated code transformation, 
% Their analysis results show that the examined datasets contain a multitude of noise categories, including comment irregularities, variable over-splitting, non-literal characters, incomplete developmental tags, and issues like empty or duplicated code.
% In conclusion, data noise remains an inherent problem in the domain of LM-based code tasks. 

\noindent \textbf{Labeling Errors:}
Labeling errors arise when ground-truth labels are inaccurate, unstable, or erroneous~\cite{arp2022and, tantithamthavorn2015impact}.
In some code-related tasks, such as vulnerability detection, the raw code datasets need to be labeled by human annotators.
Nie~\ea~\cite{nie2023understanding} explored the labeling error problem in vulnerability detection wherein a vulnerable code sample is mislabeled as non-vulnerable, and vice versa.
They found that mislabeling a non-vulnerable sample as vulnerable was a more pervasive issue.
The research further assessed three prominent datasets, D2A~\cite{zheng2021d2a}, Big-Vul~\cite{fan2020ac}, and Cross-Vul~\cite{nikitopoulos2021crossvul}, discovering that in the worst cases, nearly 30\% of the labels in these datasets may cause noisy labels.
Similarly, Li~\ea~\cite{li2022robust} examined the datasets from Herzig~\ea~\cite{herzig2013s} for Bug Report Classification (BRC) and from Yatish~\ea~\cite{yatish2019mining} for Software Defect Prediction (SDP).
Their findings revealed that these datasets possess mislabel rates ranging between 2\% and 29\%.



% As modern language models expand in size and complexity, labeling for the collected data often requires considerable time, effort, and human intervention. 
% This intricate process with vast data inevitably introduces potential inconsistencies and errors.
% On the other hand, many datasets derive their content from open-source platforms like GitHub and Stack Overflow and depend on user-generated labels. 
% Such labels, while extensive, are often subjective and prone to inaccuracies~\cite{wu2021data}. 
% In this study, we identified three papers focusing on labeling errors when employing LMs to automate code transformation~\cite{li2022robust, lin2022xcode,nie2023understanding}. 
% Nie~\ea~\cite{nie2023understanding} explored the labeling error problem in vulnerability detection wherein a vulnerable code sample is mislabeled as non-vulnerable, and vice versa. 
% They found that mislabeling a non-vulnerable sample as vulnerable was a more pervasive issue.
% The research further assessed three prominent datasets, D2A~\cite{zheng2021d2a}, Big-Vul~\cite{fan2020ac}, and Cross-Vul~\cite{nikitopoulos2021crossvul}, discovering that in the worst cases, nearly 30\% of the labels in these datasets may cause noisy labels.
% Similarly, Li~\ea~\cite{li2022robust} examined the datasets from Herzig~\ea~\cite{herzig2013s} for Bug Report Classification (BRC) and from Yatish~\ea~\cite{yatish2019mining} for Software Defect Prediction (SDP) [62].
% Their findings revealed that these datasets possess mislabel rates ranging between 2\% and 29\%.
% Thus, the consistency and reliability of labels in datasets have proven to be a significant concern in current research. 


\begin{figure}[t]
  \centering
  \begin{minipage}{0.5\linewidth}
    \centering
    \includegraphics[height=3.5cm, keepaspectratio]{images/dataset/fig4_stage1_data_bias_distri_time.pdf} 
    \caption{Paper distribution across time (Section~\ref{sec:data}) }
    \label{fig:result_data_bias_time}
  \end{minipage}%
  \hfill
  \begin{minipage}{0.5\linewidth} 
    \centering
    \includegraphics[height=3.5cm, keepaspectratio]{images/dataset/fig4_stage1_data_bias_distri_models.pdf}
    \caption{Distribution of LMs (Section~\ref{sec:data})}
    \label{fig:result_data_bias_models}
  \end{minipage}
\end{figure}


Overall, Figure~\ref{fig:result_data_bias_time} and Figure~\ref{fig:result_data_bias_models} present the distribution of the 11 papers concerning bias in data collection and labeling.
Figure~\ref{fig:result_data_bias_time} shows that the issue of data noise has continuously attracted the attention of researchers, and this attention has intensified significantly in recent years. 
Figure~\ref{fig:result_data_bias_models} reveals that while the emergence and widespread use of sophisticated models such as BERT and GPT~\cite{hou2023large}, the majority of the examined articles on data bias mostly concentrate on conventional language models, specifically LSTM and GRU.
This observation indicates a potential avenue for further investigation into the data biases present in modern language models.


\subsection{RQ2-Implications}
Our review results highlight the pervasive presence of pitfalls during the data collection and labeling processes in various automated code-related tasks. 
However, the deeper implications of these pitfalls remain to be fully discerned.
Thus, in this section, we aim to summarize the reviewed papers and provide insights into how these pitfalls influence the overall efficacy and performance of language models in code intelligence.

\noindent \textbf{Performance Overestimation:}
Train-test-split is a common practice for evaluating the neural models~\cite{arp2022and}.
However, derived from the same datasets, the test set contains the same bias, such as imbalanced data, as in the train set.
It leads to an overestimation of the model's performance since there is a gap between the testing dataset and real-world practices.
For example, Chakraborty~\ea~\cite{chakraborty2021deep} presented that vulnerability detection techniques are implemented on balanced datasets, and the models can achieve more than 90\% F1 scores.
However, the scenario drastically shifts when the same models are evaluated with a realistic dataset (where only 6\% of the examples are vulnerable).
In such cases, while the model could boast a recall as high as 91.24\%, this seemingly perfect metric can be deceptive.
A deeper dive reveals a mere 18.47\% F1 score, leading to a significant number of false positives.
A similar scenario arises with the introduction of data noise. 
Zhang~\ea~\cite{zhang2023slice} demonstrated this by training Transformer-based methods on a noisy dataset that included both bot-generated and trivial messages for code commit generation. 
Remarkably, the model achieved a 42.4\% BLEU-4 score under these conditions.
Yet, once the data noise was removed, the BLEU-4 score dropped sharply to 26.2\%.
Overall, pitfalls in data, whether from sampling imbalances or the presence of data noise, can lead to exaggerated performance metrics in language models for code tasks. 

\noindent \textbf{Compromised Model Efficacy:}
High-quality training data serves as the foundation for the trustworthy training of models.
When the training data introduces inherent noises and errors, language models might inadvertently learn irrelevant patterns or establish spurious correlations.
This not only distorts the model's understanding but can also undermine its performance.
For instance, Sun~\ea~\cite{sun_importance_2022} proved that code search models, when trained on carefully cleaned data without data noise, achieve a significant improvement in the number of answered queries and the rank of ground truth in search results (e.g., MRR improves from 0.407 to 0.512).
Similarly, Nie~\ea~\cite{nie2023understanding} showed that labeling errors severely compromise the performance of prevalent vulnerability detection models, with the worst instances seeing an average F1 score plummet of 20.7\%. 

\subsection{RQ3-Solutions}
Recognizing pitfalls in data collection and labeling has emphasized the need for robust solutions to address and mitigate these issues.
Several solutions have been proposed in the literature that we've reviewed. 
These solutions have been organized into distinct categories based on their underlying principles and methodologies.

\noindent \textbf{Data Cleaning/Denoising:}
Data cleaning/Denoising is the process of improving a dataset by removing or correcting abnormalities, inconsistencies, and inaccuracies. 
This phase is critical to ensuring that the training data is accurate and does not contain any misleading or irrelevant information.
Many pitfalls develop as a result of noisy or erroneous data, and data cleaning is the major method for dealing with such difficulties.
Shi~\ea~\cite{shi2022we} introduced a rule-based cleaning tool, named CAT (Code-comment cleAning Tool), that employs configurable heuristics rules to automatically scan and filter out comments and code with syntactic anomalies, thereby detecting the occurrences and distribution of data noises.
Similarly, Sun~\ea~\cite{sun_importance_2022} presented a data cleaning framework tailored for code search.
It begins with a rule-based syntactic filter configured with heuristic rules to identify syntactically inconsistent comments.
This is followed by a model-based semantic filter, which focuses on comments with the fewest reconstruction discrepancies using a Variational Auto-Encoder model trained on a pre-established bootstrap query corpus. 
Their evaluation results demonstrate that this hybrid filter approach not only significantly save computational resources but also enhances model accuracy.
Nie~\ea~\cite{nie2023understanding} introduced confident learning~\cite{northcutt2021confident} and differential training~\cite{Xu2021DifferentialTA} for denoising-based noisy label detection, aiming to enhance the label quality of vulnerability datasets. They found that the effectiveness of denoising methods heavily relies on the vulnerability detection models' fitting ability to the datasets, and these denoising methods show considerable promise in boosting vulnerability detection performance.

\noindent \textbf{Real-world Benchmarks:}
To precisely evaluate the models, researchers propose to use real-world benchmarks, instead of train-test-spilt datasets.
Many benchmarks are thus constructed.
For example, many benchmarks, such as HumanEval~\cite{chen2021evaluating}, DS-1000~\cite{Lai2022DS1000AN}, and MBPP~\cite{Austin2021ProgramSW}, are constructed using human-written tasks and test cases to evaluate the code generation LMs.
Compared with the code snippets in open-source repositories, such human-written tasks are closer to the real user requests in practice, which better reflects the performance of the model.
In addition, the models can be evaluated directly using the production data accumulated during the operation of LM-based systems.
For example, Hellendoorn \ea ~\cite{hellendoorn_when_2019} and Aye \ea ~\cite{Aye2020LearningAF} adopt the production data of code completion systems as the evaluation dataset to better measure the model's performance.
Similarly, Mozannar \ea~\cite{Mozannar2022ReadingBT, Mozannar2023WhenTS} use the user behavior data to demonstrate the effectiveness of their proposed methods.
Apart from that, Lin \ea~\cite{lin2022xcode} examine their approach on a real-world dataset composed of programming exercises with multiple solutions.



\begin{tcolorbox}[title=Summary - Data Collection and Labeling, left=2pt, right=2pt,top=2pt,bottom=2pt]
Based on 11 relevant studies, our literature review reveals three prevalent pitfalls (i.e., unbalanced distribution, data noise, and labeling errors) in the data collection and labeling process. 
These pitfalls propagate, causing overestimated performance and compromised model efficacy. 
Though initial solutions like data cleaning/denoising and real-world benchmarks have been proposed, the field is far from reaching a comprehensive resolution.
The implications underscore the need for automated and scalable techniques to ensure high-quality data for LM4Code.
\end{tcolorbox}

\section{System Design and Learning}
\label{sec:system_design}
This section examines pitfalls in the system design and learning process for LM4Code.
The training of these LM4Code models directly impacts their quality and efficacy for empowering code intelligence. 
However, several challenges arise in crafting optimal model architectures, formulating strategic training-testing approaches, refining data preprocessing techniques, and selecting suitable learning algorithms. 
Each design decision risks introducing pitfalls that can undermine model robustness and effectiveness.
% First, pitfalls can arise due to data-related factors, including the nature of the training data, inadvertent inclusion of unrealistic or unrepresentative data, and distortions introduced during data preprocessing.
% Beyond data, the learning process itself, with its inherent challenges like the black-box nature of decision-making and the nuances of model design, can be a source of biases. 
% Being cognizant of these potential biases and employing appropriate mitigation strategies is crucial to enhance the robustness and effectiveness of LM4Code.


% \input{tables/tab_model_bias_summary}

\subsection{RQ1-Pitfalls}
We have identified 16 research studies dedicated to the exploration of pitfalls introduced in the system design and learning process. 
These pitfalls can be broadly categorized into three categories: data snooping, spurious correlations, and inappropriate model design.
% Specifically, data snooping represents design flaws introduced through manual intervention, while spurious correlations and inappropriate model design are inherent to the chosen model's design. 
In the following, we provide comprehensive descriptions of these three pitfalls.

\noindent \textbf{Data Snooping:} 
% A learning model is trained with data that is typically not available in practice. (Cross-project, never-seen tests)
Data snooping arises when LMs are inadvertently exposed during training to information that should be inaccessible. 
Such unintentional exposure primarily stems from improper data handling.
% from a combination of factors related to data handling in LM4Code applications. 
A common source is improper train-test split, where evaluation/testing data leaks into training.
For example, research has identified instances where training data incorporates bugs or vulnerabilities that closely mirror those encountered in testing~\cite{ding_patching_2021, wu2023effective}.
This concept of overlap is further supported by Liu~\ea~\cite{liu_can_2021} highlighting the risks associated with functionality similarities between train and test data.
Another dimension to consider is the origin of the data. 
For instance, as emphasized by Steenhoek~\ea~\cite{steenhoek2023empirical} and Wu~\ea~\cite{wu2023effective}, using samples from the same software projects for both training and testing can influence the models. 
Even data structure and representation choices enable snooping.
Liu~\ea~\cite{liu2023towards} and Shi~\ea~\cite{shi2022evaluation} emphasize that pitfalls can emerge from the data processing processes such as test prefix generation or concurrent use of same-class data.


\noindent \textbf{Spurious Correlations:}
Spurious correlations arise when language models mistakenly depend on irrelevant artifacts rather than the code's intrinsic logic or intent for decision-making, leading to misleading associations. 
The artifacts vary across SE tasks. 
For instance, in vulnerability detection, artifacts may manifest as recurring code patterns or reliance on specific function names that LMs incorrectly associate with vulnerabilities~\cite{steenhoek2023empirical, chakraborty2021deep}. 
In code summarization, models might focus more on strings or certain code structures while overlooking elements key for developers ~\cite{paltenghi_thinking_2021}. 
When generating commit messages in the context of code review, models often produce outputs that adhere to a few simple patterns, potentially failing to capture the nuances of the actual code changes~\cite{dong2023revisiting}. 
% To pinpoint these artifacts, it's beneficial to compare model outputs with human standards or to utilize explainable tools. 
Actually, introducing advanced pre-trained models like CodeBERT has not eliminated these pitfalls. 
Specifically, if not fine-tuned appropriately for downstream tasks, these models might still overemphasize basic elements like keywords over richer code semantics~\cite{zhang_diet_2022}. 

\noindent \textbf{Inappropriate Model Design:}
Inappropriate model design in LM4Code arises when the underlying architecture fails to capture critical characteristics of code, such as hierarchy and composition.
The inability to construct robust semantic representations of code's intricate structural and logical attributes hinders model efficacy on downstream code intelligence tasks. 
Such design shortcomings can manifest in several ways. For instance, in vulnerability detection, models may exhibit a significant overlap in the feature space between classes, hindering precise vulnerability identification~\cite{chakraborty2021deep}. Code search models might lean on coarse-grained representations, capturing merely lexical or structural elements, often overlooking the true functionality of the code~\cite{wang_enhancing_2023}. Similarly, the encoder-decoder framework used in code summarization might neglect the hierarchical nature of code or struggle with sequence generation, leading to inadequate summaries~\cite{wan_improving_2018, wang_reinforcement-learning-guided_2022}. This issue is not limited to traditional architectures. Even modern program repair models, adapted from neural machine translation, face design-related challenges that affect their translation accuracy and diversity~\cite{ding_patching_2021, meng2023template}. While there are innovative attempts such as leveraging deep reinforcement learning or shared encoder-decoder architectures~\cite{lin2022xcode}, these approaches still exhibit shortcomings in addressing the diverse needs of various LM4Code applications.

To summarize, Figure~\ref{fig:result_stage2_model_bias_time} and ~\ref{fig:result_stage2_model_bias_models} display the distribution of papers that discuss LM4Code pitfalls in the system design and learning stage.
Figure~\ref{fig:result_stage2_model_bias_time} indicates that while inappropriate model design was first identified in 2018, research efforts on addressing key pitfalls have increased over the past three years. 
Among these, data snooping has garnered increasing research attention. Meanwhile, spurious correlations have become more prominent with the advent of explainable artificial intelligence~(XAI) techniques for elucidating model reasoning~\cite{10109341, 10109328,DBLP:conf/kbse/Tantithamthavorn21}. Discussions around inappropriate model design remain ongoing as new frameworks and learning strategies continue to emerge.
Contrary to our observations regarding the data collection and labeling process, Figure~\ref{fig:result_stage2_model_bias_models} reveals a greater emphasis on modern Transformer-based language models compared to conventional architectures.
Specifically, 19\% of relevant studies employ BERT, 15\% leverage general Transformer models, 11\% utilize CodeBERT, and 7\% investigate CodeT5.
This distribution highlights a shift towards examining potential pitfalls in sophisticated language models for code intelligence tasks, setting the stage for continued research focused on enhancing model transparency, interpretability, and reliability.



\subsection{RQ2-Implications} 
% The biases introduced in design and learning process cause overestimated performance and compromised efficacy in different ways, which we describe as follows.
In the system design and learning phase, pitfalls emerge that can distort LM4Code outcomes. 
Following the pitfalls identified in the previous phase, these design-related pitfalls similarly lead to performance overestimation and compromised model efficacy. 
We will now elaborate on the specific impacts of these pitfalls and how they manifest in various software engineering tasks.

\noindent \textbf{Performance Overestimation:} 
% Data Snooping and Inappropriate Data Preprocessing; inflate the reported results
Pitfalls in system design and learning can lead to over-optimistic performance metrics for LM4Code models.
Data snooping is a major contributor to this overestimation. 
For example, the presence of overlapping functionality between training and test sets can elevate the F1 score of a clone detection model from 0.42 to 0.96~\cite{liu_can_2021}. In vulnerability detection, a mix of projects in both training and testing phases can introduce discrepancies in F1 scores as large as 0.32~\cite{steenhoek2023empirical}. 
Spurious correlations represent a subtler and often more elusive challenge. 
These pitfalls cause models to make correct predictions, but often for the wrong reasons, leading them to rely on irrelevant code patterns or unrelated artifacts.
This not only misleads performance interpretation but also makes the models unreliable in varied scenarios~\cite{steenhoek2023empirical}. 
Models might also give undue attention to superficial code constructs, leading to inefficiencies that don't necessarily enhance outcomes~\cite{zhang_diet_2022}.

\noindent \textbf{Compromised Model Efficacy:} 
% Spurious Correlations and Inappropriate Model Design
While overestimation impacts perceived performance, inappropriate model design directly compromises the efficacy of models in practical scenarios. For example, token sequence-based vulnerability detection models might fail to capture the underlying causes of vulnerabilities and instead focus on surface-level patterns, leaving a significant margin for improvement. 
Chakraborty~\ea~\cite{chakraborty2021deep} highlighted this limitation and showed that the use of gated graph neural networks can improve the baselines by 33.57\% in precision and 128.38\% in recall. 
Similarly, the design limitations in code search models lead them to generate coarse-grained representations that may overlook core functionalities~\cite{wang_enhancing_2023}. Program repair models, based on neural machine translation models, have shown slow learning curves, achieving a mere 4.5\% repair prediction accuracy even after 10 epochs~\cite{ding_patching_2021}. This indicates that the structural design of the model hinders its ability to learn and adapt efficiently.



\subsection{RQ3-Solutions}

To address the three pitfalls related to the system design and learning process, researchers have employed a variety of approaches which we describe as follows. 

\noindent \textbf{Refined Data Handling:}
To mitigate the challenges posed by data snooping, a multifaceted approach is essential.
Emphasizing rigorous data partitioning is foundational, as exemplified by Steenhoek~\ea~\cite{steenhoek2023empirical}, who advocate for cross-project validation to prevent inadvertent overlaps between training and testing sets.
Additionally, techniques like data augmentation and time-based splits can further insulate models from over-relying on specific pattern~\cite{pendlebury2019tesseract, guerra2022relativity}.
Incorporating regularization techniques, such as batch normalization, can curb overfitting and deter models from exploiting inadvertent data correlations~\cite{he2022msdroid}. 
Finally, the importance of external validation, underscored by Liu~\ea~\cite{liu_can_2021}, ensures that performance assessments are unbiased and reflective of real-world scenarios. 
By adopting these strategies, researchers can foster more reliable and generalizable outcomes.

\noindent \textbf{Model Interpretability:}
To address the biases inherent in LM4Code, especially spurious correlations, improving model interpretability has emerged as a crucial solution~\cite{10109341}. 
By examining the decision-making process of LM4Code models, researchers are better positioned to pinpoint and mitigate pitfalls, leading to more reliable predictions~\cite{he2023finer}. 
Within vulnerability detection, Fu~\ea~\cite{fu2023vulexplainer},
Li~\ea~\cite{li_vulnerability_2021} and Zou~\ea~\cite{zou_interpreting_2021} proposed methods to enhance explanation accuracy, leveraging sophisticated visualization tools to correlate the internal dynamics of neural models with code structures, thus providing a comprehensive understanding of model reasoning. 
Cito~\ea~\cite{cito_explaining_2021} offers a distinctive perspective, centering on elucidating mispredictions. 
Their approach, which integrates neural predictions with symbolic logic, allows for precise error detection accompanied by rule-based explanations. 
Additionally, attention mechanisms to explain pre-trained models have also been analyzed.
While Shi~\ea~\cite{shi2023towards} unravels how transformer-based models allocate attention for code summarization, Wan~\ea~\cite{wan_what_2022} probes into the nuances of attention during code-to-code translation. 
These XAI approaches can serve to identify and rectify model pitfalls, ensuring the reliability of LM4Code applications.

\noindent \textbf{Model Optimization Strategies:}
In light of the pitfalls introduced by inappropriate model design, researchers have turned to model optimization strategies to address and minimize their effects. These strategies encompass several techniques designed to enhance a model's structure, training process, and generalization capabilities. 
Firstly, Model Design Adjustments involve refining the architecture to better capture data intricacies. Studies like that by Wan~\ea~\cite{wan_improving_2018} have demonstrated the benefits of introducing novel layers or structures to better understand the tree structure of code, yielding improved performance. 
Secondly, Model Ensembling is gaining traction, where the strengths of multiple models are leveraged to offset individual biases, as seen in the work by Zhang~\ea~\cite{zhang_diet_2022} which employs multiple views of the same data for more robust predictions. 
Lastly, Regularization and Fine-tuning techniques play a pivotal role. Regularization, such as dropout or L2 regularization, helps in preventing overfitting, while fine-tuning allows pre-trained models, like CodeBERT, to adapt to specific dataset nuances, as demonstrated by Fang~\ea~~\cite{fang2023representthemall}. 
By integrating these strategies, models can be better positioned to achieve superior outcomes.



\begin{tcolorbox}[title=Summary - System Design and Learning, left=2pt, right=2pt,top=2pt,bottom=2pt]
In this study, we uncover 16 research studies related to pitfalls in system design and learning. 
These pitfalls can be categorized into three main categories: data snooping, spurious correlations, and inappropriate model design.
These pitfalls lead to overestimated performance and compromised efficacy of LMs. 
Proposed solutions encompass refined data handling, model explainability, and optimization strategies like architecture adjustments, ensembling, and regularization. 

\end{tcolorbox}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{images/design/Distr-design-solution.png}
%     \caption{The Distribution over years.}
%     \label{fig:Distr-design-solution}
% \end{figure}

% As shown in Fig \ref{fig:Distr-design-solution}, we conducted a statistical analysis of the solutions applied in this segment (the number of articles for 2023 is fewer since we did not consider papers from arXiv). What we can observe is that researchers are inclined to use methods based on language models when addressing this category of problems. Out of a total of 43 papers, at least 21 are grounded in language models (including two in the "New Testing Methods or Benchmarks" category\cite{luo_graph-based_2021}\cite{cao_mvd_2022}). Language models have indeed become a significant tool in the researchers' arsenal for solving problems. However, as this Systematic Literature Review (SLR) intends to highlight, there are numerous pitfalls in language models that merit careful attention.

% \begin{enumerate}
%     \item \textit{New testing methods or benchmark.} Whenever a problem arises, it represents the emergence of a class of problems, as nothing exists in isolation. Therefore, the development of testing methods and benchmarks for a class of problems is of paramount importance. For the issues that arise during the system design and learning stage with Language Models (LM), many researchers have proposed testing benchmarks and methods. For example, in facing the problem of bug localization in Automatic Program Repair (APR), \cite{kassianik_bigissue_2023} introduced BigIssue, a realistic bug localization benchmark. For the testing of DL libraries, methods such as CRADLE \cite{pham_cradle_2019}, LEMON \cite{wang_deep_2020}, and graph-based fuzz testing \cite{luo_graph-based_2021} have been put forward. In the context of vulnerability detection, \cite{cao_mvd_2022} proposed MVD, a state-level memory-related vulnerability detection method based on Flow-Sensitive Graph Neural Networks (FS-GNN). Additionally, for the often-encountered word embeddings in LM, where problematic word embeddings might occur, \cite{tao_trader_2020} provided a novel technique to automatically diagnose how these flawed embeddings impact model performance.
    
%     \item \textit{Tools and methods based on language models.} Many methods based on Language Models (LM) have been proposed to tackle these issues. According to the types of models employed in various literature, they can be broadly categorized into: those based on encoder-decoder architectures \cite{zhu_syntax-guided_2021}\cite{zhang_retrieval-based_2020}, AST-based ones \cite{zhang_novel_2019}\cite{wang_modular_2020}\cite{wang_reinforcement-learning-guided_2022}, DNN-based \cite{wang_enhancing_2023}, NMT-based \cite{jiang_cure_2021}\cite{ye_neural_2022}, RNN-based \cite{li_dear_2022}\cite{li_dlfix_2020}\cite{meng_improving_2022}\cite{zou_vuldeepecker_2021}, Transformer-based \cite{izadi_codefill_2022}\cite{liu_multi-task_2021}\cite{zhang_slice-based_2023}, and other types of models. Additionally, some methods leverage pre-trained models, such as \cite{zhang_coditt5_2023}\cite{jiang_cure_2021}\cite{zhang_slice-based_2023}\cite{ahmed_synshine_2023}.
%     Interestingly, a substantial number of LM-based methods are employed to address the vulnerabilities present within language models themselves, while many of these models remain inadequately understood and analyzed by researchers. Utilizing unknown methods to solve unknown problems, through such continuous iteration, even accurate information might become gradually distorted.
%     Language models represent an incredibly useful tool, but the potential pitfalls should not be ignored. Researchers should neither reject them outright nor become complacent. Instead, it is wise to exercise caution, making use of interpretable means wherever possible. Otherwise, successes may merely be coincidental, and the quest for true understanding may be compromised.
    
%     \item \textit{Other proposed technological advancements.} In addition to testing and methods based on language models, researchers have also employed traditional methods, which hold a clear and evident advantage in terms of interpretability and reproducibility compared to language model-based approaches. This makes the understanding and replication of these methods relatively straightforward and convincing. However, it's worth emphasizing that not every new innovation should be applied without critical analysis. If researchers deploy new and expensive processes, these efforts should be juxtaposed with simpler and faster alternatives for baseline comparisons. As emphasized by Fu~\ea~\cite{fu_easy_2017}, critical evaluation and comparison with existing methods can prevent unnecessary complexity and ensure that the chosen techniques truly offer advantages in terms of efficiency, accuracy, or other relevant criteria. 
%     For example, when language models struggle with handling long-term dependency issues, \cite{yang_language_2017} introduced PCC, which manages long token sequences by introducing an intermediate representation (IR) for source code. It further employs a fuzzy matching technique that combines genetic algorithms with the longest common subsequence algorithm to enhance prediction accuracy. Similarly, in \cite{aghababaeyan_black-box_2023}, the authors proposed a method that integrates two mature technologies, symbolic execution, and local interpretability, to automatically generate test inputs for individual discrimination detection, rather than utilizing language models.
%     Similar contributions can be found in works such as \cite{kloberdanz_deepstability_2022}, \cite{li_editsum_2021}, \cite{gao_estimating_2020}, \cite{zhang_merit_2022}, and \cite{dutta_tera_2021}. These studies exemplify the continued effort and diligence of researchers to explore not just cutting-edge techniques, but also to revisit and leverage traditional methods where they may provide more transparent and reliable solutions.
    
%     \item \textit{Empirical study.} Researchers have conducted extensive and wide-ranging empirical studies on the traps and biases in system design and learning. For instance, concerning the issue of hyperparameters, the authors in \cite{liao_empirical_2022} carried out a comprehensive examination of four representative and widely-used DNN models to investigate how different hyperparameters affect standard DNN models. They also explored how hyperparameter tuning, in combination with model optimization, influences various performance attributes of optimized DNN models (such as inference latency or battery consumption). The study observed that model optimization can create confounding effects on the influence of hyperparameters on DNN model performance. Meanwhile, \cite{wang_automatic_2021} conducted an empirical investigation into the effectiveness of DL libraries, offering critical insights. Furthermore, \cite{paltenghi_thinking_2021} examined the extent to which the attention weights of efficient neural models align with skilled human reasoning, uncovering a key insight that models and humans may sometimes focus on different types of tokens. For example, strings may be crucial for humans, but are often ignored by models.
% \end{enumerate}


% \subsubsection{Factors}
% \yue{removed, update it to implications}
% \input{tables/factor_design}
% Design Bias and Subjective Training each have multiple contributing factors. In this section, we further dissect the two components mentioned previously, as shown in Table \ref{tab:factor_design}.

% As illustrated in Fig \ref{fig:Distr-design-factor}, we have analyzed the annual distribution of these 44 papers across various factors. At a glance, the overall trend shows an increase in the number of articles addressing the pitfalls and biases in system design and learning, although the number of articles for 2023 is less, due to the exclusion of the arXiv repository. 
% From the left graph, we observe that the factors "Insufficient Utilization of Knowledge" and "Inappropriate Techniques" are the most prevalent, with 16 and 13 papers, respectively. The abundance of papers on inappropriate techniques is likely due to the broad encapsulation of this concept. On the other hand, the factor "Insufficient Utilization of Knowledge" leads in frequency and maintains a consistent annual count since 2020, indicating a high and steady level of attention. This reveals that researchers are paying significant attention to various aspects such as information granularity, structure, identifiers, etc. Furthermore, articles concerning "Long-term Dependency", "Irreproducibility" and "Poor Reusability and Replaceability" are the least common, each with lower than two instances. The former appeared only before 2019, while the latter emerged in 2021. Finally, the literature related to "Bias in Frameworks and Algorithms" and "Biased Parameters" is relatively sparse and stable, retaining a certain level of attention.
% From the right graph, it is evident that the number of articles related to "Design Bias" and "Subjective Training" are roughly equivalent, standing at 23 and 20 papers, respectively. The nearly identical annual distribution suggests a similar level of interest in these areas.

% \textbf{Design Bias.} Design bias in the context of machine learning and language modeling refers to the systematic biases that may be introduced during the process of model design. This can encompass a wide array of issues, including the selection of inappropriate frameworks or algorithms, Inability to handle the long-term dependency problem, the misuse or overuse of specific techniques, and inherent flaws within the chosen methods. Design bias can have significant implications. It may lead to the model's poor performance on unseen data or give rise to unfair or discriminatory outcomes.

% \begin{figure}[t]
%   \centering
%   \begin{minipage}{0.5\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/design/Distr-design-factor-1.png}
%   \end{minipage}%
%   \begin{minipage}{0.5\linewidth} 
%     \centering
%     \includegraphics[width=\linewidth]{images/design/Distr-design-factor-2.png}
%   \end{minipage}
% \caption{Distribution of papers over years.}
% \label{fig:Distr-design-factor}
% \end{figure}

% \begin{enumerate}
%     \item \textit{Inappropriate techniques.} In the process of model design, the employment of ill-suited techniques often results in various hidden issues, such as increased computational complexity\cite{zhang_diet_2022}, reduced performance, and decreased efficiency\cite{fu_easy_2017}. In the real world, these issues can potentially lead to misunderstandings, financial losses, threats to personal safety and health, as well as political conflicts\cite{he_testing_2021}. The recent trend of utilizing Deep Learning (DL) and Machine Learning (ML) in Automated Program Repair (APR) has brought numerous limitations to the fore\cite{li_dear_2022}. For instance, in APR, employing an encoder-decoder structure to generate repair patches, with the decoder still in a standard form, has revealed serious limitations\cite{zhu_syntax-guided_2021}. These techniques often rely on defect localization technologies for assistance, but the shortcomings of these approaches make the models challenging to implement in practical applications\cite{kassianik_bigissue_2023}. Other tasks in Software Engineering (SE), such as syntax-based auto-completion constrained by dynamic language environments\cite{izadi_codefill_2022}, and pre-trained language models not specifically designed for reasoning about edits\cite{zhang_coditt5_2023}, also face hurdles. Deep learning techniques have been found wanting in code summarization tasks\cite{li_editsum_2021}, and neural network methods have revealed deficiencies in Neural Program Synthesis (NPS) tasks\cite{zhang_merit_2022}. Moreover, Language Models (LMs) display inherent biases and dependencies, such as favoring high-frequency words in their training corpus\cite{zhang_retrieval-based_2020}, or reliance on third-party pre-trained word embeddings\cite{tao_trader_2020}. These factors may lead to pitfalls in model deployment, adding yet another layer of complexity to the task at hand.
    
%     \item \textit{Long-term dependency problem.} The issue of Long-term Dependency is a challenge in deep learning, particularly within Recurrent Neural Networks (RNNs). It involves the model's handling and learning of dependencies across extended time intervals within sequential data. In code auto-completion tasks, Language Models (LMs) are more suitable for predicting short token sequences but perform poorly on longer sentence-level predictions \cite{yang_language_2017}. This problem also manifests in neural models based on Abstract Syntax Trees (ASTs) \cite{zhang_novel_2019}. As the size of ASTs is typically large, existing models are prone to issues related to long-term dependency.Consequently, special attention should be paid to this characteristic during the design process of Deep Learning/Machine Learning (DL/ML) based Software Engineering (SE) tasks. It is essential to either avoid or actively seek solutions to this problem, as it can significantly influence the effectiveness and reliability of the implemented models.
    
%     \item \textit{Bias in frameworks and algorithms.} Bias in frameworks and algorithms refers to the inherent biases and tendencies that may exist within the structure of computational frameworks and the specific algorithms used within systems. These biases can lead to unfair or imbalanced outcomes across various applications, ranging from decision-making systems to data analysis. In recent years, a significant amount of research has focused on the testing of DL models, while there has been less attention paid to the testing of DL libraries\cite{pham_cradle_2019}. However, DL libraries form the foundation of DL models, directly influencing the behavior of DL systems.Regrettably, there are numerous issues with DL libraries. For example, an empirical study by \cite{wang_automatic_2021} revealed that most machine learning libraries do not maintain high quality in terms of commonly used quality metrics such as code coverage and mutation scores. Further complications include the numerical instability in DL algorithms, as examined by \cite{kloberdanz_deepstability_2022}, potential noise introduced into DL libraries by uncertainty factors as highlighted by \cite{wang_deep_2020}, and issues related to algorithmic discrimination in machine learning software as investigated by \cite{peng_fairmask_2023}.These concerns underscore the critical importance of rigorous examination and testing of both the frameworks and the algorithms at play, not only to ensure the accuracy and efficiency of the systems but also to uphold ethical standards and societal fairness. It's a challenging task that requires the combined efforts of researchers, engineers, and policymakers to build more transparent and accountable AI systems.
    
%     \item \textit{Poor Reusability and Replaceability.} The challenge of reusability and replaceability in deep learning models has been a persistent issue in the stages of system design and learning. While previous studies have attempted to address this issue, most methods were confined to dense layers, focusing on one-to-one relationships between nodes in consecutive layers, thus proving difficult to adapt in the shared architecture of CNN models. A novel approach introduced in \cite{pan_decomposing_2022} emphasizes decomposing CNN models used for image classification into modules for each output class, effectively overcoming the limitations of prior work. This strategy provides a new solution for enhancing reusability and replaceability across various scenarios. It not only contributes to reducing the complexity of model design and training but also eliminates the necessity to train the models from scratch each time. This enhances the flexibility and efficiency of the models while reducing costs.
% %\cite{pan_decomposing_2022}先前的工作已经提出将基于密集的网络分解为模块(每个输出类一个)，以实现在各种场景中的可重用性和可替换性。然而，这项工作仅限于密集层，并且是基于连续层中节点之间的一对一关系。由于CNN模型中的共享架构，无法直接适应先前的工作。
%     \item \textit{Irreproducibility.} During the model training phase, considering the reproducibility of the model is of paramount importance. Model reproducibility refers to the ability to achieve similar results under the same experimental settings and conditions in different studies or experiments. In the field of machine learning and deep learning, due to factors such as the inherent randomness in software (e.g., DL algorithms) and the non-deterministic nature of hardware (e.g., GPUs), DL models are often difficult to reproduce\cite{chen_towards_2022}. This lack of reproducibility poses numerous challenges for researchers and practitioners, including model verification, generalization testing, and model improvement. For instance, if a model's results cannot be reproduced, it becomes difficult to accurately assess and verify its performance, and therefore, ensuring its effectiveness in real-world applications becomes a challenge. Furthermore, the inability to reproduce model results hampers further research and improvement of the model. Researchers might find it challenging to accurately replicate the model's performance, identify shortcomings, and subsequently implement effective optimizations and improvements.
% %\cite{chen_towards_2022}由于软件(例如, DL算法)中的随机性和硬件(例如, GPU)中的非确定性等问题，DL模型很难被重现

% \end{enumerate}
% \textbf{Subjective training.} Subjective training in the context of machine learning and language modeling refers to the influence of the researcher's personal biases and judgments during the training process. This can manifest in various ways, such as the subjective choice of hyperparameters, the biased selection of training data, or the interpretation of results based on personal preferences or expectations. For instance, the researcher might tune the model in a specific direction to achieve desired results, without a clear understanding of the underlying implications. This subjectivity can introduce hidden risks, possibly leading to overfitting or a lack of generalizability. Additionally, it might contribute to the neglect of various attributes like granularity, structure, and identifiers in the provided information for training, or other neglected knowledge, all of which could stem from the researcher's subjective bias. Overall, subjective training emphasizes the critical role of objectivity and scrutiny in the model development process, as undue influence of personal biases can significantly impact the model's effectiveness and reliability.

% \begin{enumerate}
%     \item \textit{Biased parameter.} A biased parameter in machine learning models refers to a parameter that may consistently deviate from the true value, and these parameters can be either internal to the model or hyperparameters. Hyperparameters are set before the training process begins, and their selection can have a significant impact on the overall performance of the model. Hyperparameter tuning often emphasizes model accuracy or loss functions, yet this process may inadvertently affect other performance attributes of DNN (Deep Neural Network) models\cite{liao_empirical_2022}. Improper choices of neural architectures or hyperparameters may even lead to failure by exhausting limited GPU memory. Moreover, for certain algorithms (such as random forests), some configurations of hyperparameters (like limiting the attribute search space) have been shown to amplify biases between applications\cite{tizpaz-niari_fairness-aware_2022}. On a related note, hyperparameters are often manually selected during testing, but this selection can be overly conservative, leading to slow test execution and consequently increasing the cost of regression testing\cite{dutta_tera_2021}.
    
%     \item \textit{Insufficient utilization of knowledge.} "Insufficient utilization of knowledge" refers to the inability or failure to fully harness and apply existing knowledge or information. During the process of learning and training models, various forms of knowledge and information are involved, much of which may be inadvertently ignored or overlooked by researchers. For instance, the existing techniques mentioned in \cite{wang_enhancing_2023} offer overly coarse-grained representation learning for information at the lexical, control structure, or data flow level. Summing up, this overlooked information can be categorized into the following types: context \cite{li_dlfix_2020}\cite{liu_multi-task_2021}, semantic and syntactic information \cite{jiang_cure_2021}\cite{zhang_slice-based_2023}, domain-specific knowledge \cite{ye_neural_2022}, structural information \cite{wan_improving_2018}\cite{wang_modular_2020}\cite{wang_reinforcement-learning-guided_2022}, flow information \cite{cao_mvd_2022}, error or warning reports \cite{ahmed_synshine_2023}, and human-focused string tokens that are often ignored by programs \cite{paltenghi_thinking_2021}. These pitfalls are so subtle that researchers may easily fall into the routine of inputting information without considering the finer-grained details, leading to missed opportunities for enhancement and understanding.
% \end{enumerate}


\section{Performance Evaluation}
\label{sec:performance_evaluation}

The performance evaluation stage focuses on precisely assessing and analyzing the model's performance using predefined test sets and evaluation metrics.
Additionally, comparative performance evaluation against benchmarks provides insights into a model's strengths and weaknesses on specific code-related tasks.
However, potential pitfalls can emerge from factors such as improper baselines, test sets, and performance metrics.
These challenges must be thoroughly examined and addressed to ensure that the evaluation is unbiased, comprehensive, and representative of a model's true capabilities.
Thus, this section provides a brief description of related studies and discusses the implications and potential solutions during the performance evaluation stages.

% These challenges need heightened vigilance to preserve the fairness and accuracy of assessments, urging evaluators to steer clear of inappropriate baselines and test sets, ensure reproducibility, and opt for fitting performance metrics. By recognizing and navigating these potential stumbling blocks, the evaluation not only furnishes quantified insights into the model's operational efficacy but also shapes a roadmap for developers to anticipate and address challenges likely to arise in real-world applications. Consequently, this phase crystallizes as a critical feedback loop, fine-tuning the consonance between model capabilities and the practical demands of code intelligence tasks, and steering the developmental trajectory towards robust, reliable solutions.



\begin{figure}[t]
  \centering
  \begin{minipage}{0.5\linewidth}
    \centering
    \includegraphics[height=3.5cm, keepaspectratio]{images/evaluate/fig6_stage3_eval_bias_distri_time.pdf} 
    \caption{Paper distribution across time (Section~\ref{sec:performance_evaluation}) }
    \label{fig:result_stage3_deploy_bias_time}
  \end{minipage}%
  \hfill
  \begin{minipage}{0.5\linewidth} 
    \centering
    \includegraphics[height=3.5cm, keepaspectratio]{images/evaluate/fig6_stage3_eval_bias_distri_models.pdf}
    \caption{Distribution of LMs (Section~\ref{sec:performance_evaluation}) }
    \label{fig:result_stage3_deploy_bias_models}
  \end{minipage}
\end{figure}

% \input{tables/tab_evaluate_bias_summary}
%\input{tables/tab_evaluate_bias_papers}
\subsection{RQ1-Pitfalls}
From the collected studies, we identified 29 research studies focusing on pitfalls during the performance evaluation phase.
We have methodically categorized the collected literature into four categories, as shown in Figure~\ref{fig:result_stage3_deploy_bias_time}.

\noindent \textbf{Inappropriate Baseline:}
Inappropriate baselines arise when the performance evaluation for LM4Code is carried out without, with limited, or with skewed baseline approaches.
Such poor comparisons fail to convincingly demonstrate the improvements or strengths of newly proposed LM4Code approaches, potentially leading to misguided experimental findings or exaggerated efficacy claims.
For instance, comparing only against basic rule-based approaches would inflate capabilities, while limiting comparisons to other advanced LM-based approaches masks potential weaknesses.
Liu~\ea~\cite{liu2023towards} highlight this issue in state-of-the-art Neural Test Oracle Generation (NTOG) evaluation, where the lack of a straightforward baseline causes considerable gaps between reported and real-world performance.

\noindent \textbf{Inappropriate Evaluation Datasets:} 
% \yue{inappropriate evaluation datasets?}
Inappropriate evaluation datasets refer to the use of unsuitable, non-representative, or limited test sets that fail to adequately represent the true complexities of the studied tasks.
Such test sets can provide misleading results, and offer an obscured, over-optimistic, or pessimistic view of a model's realistic capabilities. 
Liu \ea~\cite{liu_deep_2022} highlight the frequent use of small, non-representive, and non-diverse datasets in code generation evaluations that fail to capture real-world software complexities. 
Specifically, the widely-used HS dataset~\cite{ling2016latent} comprises code from a single project, exhibiting poor diversity. 
The average code length in the Django dataset~\cite{oda2015learning} is a mere 33 characters, indicating limited program complexity.
The CoNaLa dataset~\cite{yin2018learning} utilizes automatically extracted Stack Overflow questions instead of real software requirements.
In short, common benchmarks poorly approximate the complexities of realistic code generation scenarios.
In vulnerability detection, Liu \ea~\cite{liu_cd-vuld_2022} highlight that most evaluations make the assumption that training and test datasets are drawn from the same distribution. However, they argue this assumption overlooks the continuous evolution of software vulnerabilities and projects, leading to the Cross-Domain issue where test sets should contain novel vulnerabilities or projects.
Furthermore, Nong \ea~\cite{nong_generating_2022} further reveal that vulnerability datasets like SARD~\cite{black2017sard} comprise unrealistic synthetic examples, which exhibit smaller vocabulary, smaller program length, and higher pattern frequency compared to real-world code.
Zeng \ea~\cite{zeng_deep_2021} claim that the state-of-the-art Just-in-Time (JIT) defect prediction tool, CC2Vec~\cite{hoang2020cc2vec}, was only evaluated on a limited dataset with marginal improvements to demonstrate generalizability and scalability. 
Overall, common benchmarks in code-based research utilize inappropriate test sets that fail to capture real-world complexities, leading to unrealistic performance evaluation.


\noindent \textbf{Low Reproducibility:}
Reproducibility is a fundamental requirement of scientific research to verify the validity and generalizability of findings through consistent replication across settings~\cite{ivie2018reproducibility, li2023trustworthy}.
However, LM-based research introduces specific challenges around efficiently storing big data, communication between distributed clusters, algorithm implementation, and appropriate software/hardware environments~\cite{li2023trustworthy, jiang2023empirical}.
Thus, low reproducibility in LM4Code significantly impacts performance evaluation, affecting the generalizability and trustworthiness of findings.
Zeng \ea~\cite{zeng_extensive_2022} conducted an extensive empirical study revealing reproducibility issues with pre-trained LMs for program understanding and generation.
As described in their study, multiple performance comparison results can be reversed compared to original publications. 
For example, CodeGPT incurred the largest variance across 5 clone detection runs under the benchmark BigCloneBench dataset, able to outperform or underperform other models depending on the run. 
Although PLBART reported a 0.7 F1 advantage over CodeBERT in the original paper, its min-max F1 variations of 0.84 make this finding questionable. 
Additionally, CodeBERT and PLBART's defect detection accuracy reversed between the original PLBART paper and the subsequent research by Zeng~\ea~\cite{zeng_extensive_2022}.
Such statistically significant variations could invert performance comparisons, thereby undermining LM4Code's trustworthiness.


% For example, the research uncovers fluctuating performance metrics in models like CodeGPT across multiple runs in clone detection tasks. Likewise, PLBART's reported advantage over CodeBERT in its original paper was found to be untenable due to performance variability. Such variations are not only statistically significant but could also reverse the performance comparison outcomes, thereby affecting the credibility of language models. 


\noindent \textbf{Inappropriate Performance Measures:} 
Inappropriate performance measures arise from a mismatch between standardized metrics and the distinct challenges inherent to software engineering tasks. 
Prior survey studies~\cite{wang_machinedeep_2023,hou2023large} have shown widespread use of generic metrics like accuracy, precision, BLEU, and Pass@k in LM4Code research.
However, these metrics often provide an incomplete view of model capabilities on code-based tasks, owing to the complex and multifaceted nature of software engineering scenarios. 
For instance, Roy~\ea~\cite{roy2021reassessing} conducted an empirical study with 226 human annotators and showed that popular metrics like BLEU and ROUGE are poor reliable indicators of human judgment. 
This demonstrates how common metrics may not fully align with code quality assessments.
Additionally, when evaluating classification tasks like vulnerability detection, reporting solely accuracy is insufficient, as true-positive and false-positive decisions are not observable~\cite{liu2023towards, chakraborty2021deep}.
Moreover, popular metrics like BLEU derived from natural language processing overlook critical attributes of code. 
As a textual similarity metric, BLEU calculates n-gram precision between generated and reference sentences. However, programming languages contain many "trivially shared n-grams", rendering BLEU ineffective at distinguishing actually similar code from coincidental similarities~\cite{eghbali2022crystalbleu}.
As we discussed before, code-based tasks exhibit multiple distinct challenges such as data imbalance, data snooping, execution correctness, and exception handling.
For example, despite high BLEU scores, CodeT5 generated code with only 6.4\% compilation rate, indicating poor execution correctness~\cite{wu2023effective}.
Overall, it is critical to utilize appropriate evaluation metrics in LM4Code research to provide a comprehensive and accurate understanding of model performance.


Figure~\ref{fig:result_stage3_deploy_bias_time} presents the distribution of relevant literature across years, while Figure~\ref{fig:result_stage3_deploy_bias_models} summarizes the distribution across different LMs.
Between 2018 and 2023, there was a noticeable rise in the number of papers, suggesting a growing focus by researchers on pitfalls in LM4Code during the performance evaluation phase. 
Among the identified studies, inappropriate evaluation datasets have the most mentions, with 19 studies, showing the difficulty in establishing representative datasets of LM4Code for reliable model performance. 
Additionally, inappropriate performance measures also garnered considerable research attention, with 6 identified studies.
From Figure~\ref{fig:result_stage3_deploy_bias_models}, we can observe that Transformer-based models were most discussed, evidencing their increasing adoption for SE tasks. 
In summary, these observations emphasize critical areas for improvement to enable robust evaluation and unbiased analysis of capabilities as LM4Code evolves. 
Careful consideration of evaluation datasets, metrics, and baselines will be integral to advancing progress in the field.



\subsection{RQ2-Implications}
Through a thorough examination of 29 relevant studies, our review has identified several pitfalls present in current approaches to evaluating the performance of LM4Code.
If left unaddressed, these pitfalls can produce misleading or unrealistic results, skewing perceptions of how these models might perform in real-world settings. In this section, we discuss the broader implications of the identified evaluation pitfalls and their potential impacts on LM4Code research and practical applications.


\noindent \textbf{Performance Overestimation:}
Pitfalls during performance evaluation can lead to a concerning overestimation of model capabilities, creating a misleading gap between reported metrics and real-world performance.
Key contributors include the use of inappropriate and unrealistic evaluation datasets and improper performance measures misaligned with practical objectives. 
Small and synthetic evaluation datasets often fail to adequately represent the true complexities that models face in real-world code intelligence tasks. 
Yet these limited datasets yield seemingly “perfect” metrics during evaluation. 
As Liu~\ea~\cite{liu_deep_2022} empirically showed, the capabilities of code generation models are often overestimated due to the use of limited datasets. When evaluated on the small Django~\cite{oda2015learning} and HS~\cite{ling2016latent} datasets, code generation approaches yielded strong BLEU scores of 0.811 and 0.646 respectively. However, simply switching to a new and more practical dataset led to a drastic BLEU score drop to 0.167, revealing how exaggerated initial metrics can be. 
Similarly, performance metrics misaligned with practical objectives tend to provide an unrealistic overestimate of capabilities. These inflated metrics collapse when models face the true complexities of real-world deployment.
As Ahmed~\ea~\cite{ahmed_synshine_2023} showed,  as the length of input tokens increases for program repair tasks, the accuracy of language models can decrease substantially from 82.88\% to 55\%. While overall accuracy may seem high during evaluation, metrics fail to reflect significant drops in certain practical scenarios.
Furthermore, popular metrics like BLEU can fail to accurately assess model capabilities, as demonstrated by Eghbali~\ea~\cite{eghbali2022crystalbleu}. 
Their analysis showed BLEU's shortcomings in distinguishing between a neural code generation model and a dummy model that simply exploited common n-grams. Despite the dummy model producing low-quality code, BLEU scored it equivalent to the neural model. 
This indicates BLEU's inability to differentiate between models genuinely solving complex tasks and those exploiting superficial patterns.
Overall, inappropriate evaluation practices systematically and significantly overestimate the capabilities of LM4Code models, obscuring major gaps between reported metrics and real-world effectiveness. More rigorous and realistic benchmarking is critical.

\noindent \textbf{Compromised Reproducibility:}
The reproducibility of research findings through independent verification is a fundamental requirement of the scientific process that allows reported improvements to be validated and incrementally built upon~\cite{ivie2018reproducibility}.
However, our analysis reveals that performance evaluation in LM4Code research may lack sufficient reproducibility.
The proposed approaches frequently bypass consistent evaluation protocols, datasets, and implementation details, making it difficult for others to replicate the experiments described in the literature and validate their accuracy~\cite{zeng_extensive_2022}.
Furthermore, inconsistent performance across different runs or implementations obscures the reliability of findings, as initial results that appear promising frequently fail to fully replicate in subsequent studies~\cite{zeng_extensive_2022}.
This phenomenon indicates that minor variances in experimental conditions, which are rarely comprehensively reported, can significantly influence outcomes.
Limited methodological transparency through selective reporting of details further inhibits reproducibility~\cite{jorgensen2016incorrect}.



% Reproducibility and scalability are paramount for LM4Code, especially in this ever-evolving era where technology is constantly iterating and industries are continuously upgrading. However, pitfalls during the performance evaluation stage can hinder these two aspects. For instance, Zeng \ea~\cite{zeng_extensive_2022} noted that pre-trained models often do not adhere to consistent evaluation protocols, making it difficult for others to replicate the experiments described in the literature and validate their accuracy. Even if a model demonstrates promising performance, others might find it challenging to build upon or improve it. 
% This highlights the pressing need for standardized evaluation protocols to improve reproducibility. 
% Furthermore, inconsistent performance across different runs may lead to untenable claims in the original papers, compromising the reliability of emerging techniques in the LM4Code field. 
% Moreover, other pitfalls, such as the concealment or embellishment of test sets or baselines, further exacerbate issues of reproducibility and hinder scalability. Therefore, there is an urgent need for the development and implementation of open and transparent standards. The severity of this issue, which obstructs scientific verification and advancement, undoubtedly warrants attention and action.



\noindent \textbf{Misleading Benchmarks:}
Misleading benchmarks and exaggerated claims lead research communities astray and substantially hinder actual progress~\cite{van2019sok}. 
For instance, evaluating models on limited datasets or with improper metrics often amplifies perceived improvements beyond actual capabilities.
However, identifying possible pitfalls remains an open challenge for future LM4Code researchers to address.
As Liu~\ea~\cite{liu2023towards} highlighted, the lack of appropriate baselines frequently causes considerable gaps between reported and real-world performance. 
Promoting such flawed evaluations through publications and conferences propagates unreliable techniques built on shaky foundations. 
This questionable practice squanders precious community resources as researchers may pursue exaggerated claims rather than meaningful progress. 
More alarmingly, it obscures the path forward for meaningful innovation that solves real-world needs, as progress is measured on inflated claims instead~\cite{van2019sok}. 
Ultimately, systemic misleading benchmarks threaten to steer LM4Code research astray, leading the community away from impactful advancements. 
Establishing rigorous and peer-validated standards for benchmarking to guide productive research directions is an urgent need.


% Researchers have limited bandwidth, and it is essential to draw upon the collective knowledge by learning from others' works. However, misleading publications, especially those presented in top-tier conferences or journals, can have a profound impact on the community and the field at large. Common tactics include underestimating costs, overhyping effectiveness, or neglecting subtle performance degradations, all in an effort to amplify perceived contributions and win over reviewers. Such practices can lead to a "bad money drives out good" scenario, inadvertently promoting more benchmarking flaws in future systems and steering the community away from genuine progress and innovation.





% \noindent \textbf{Validity and Rationality:}
% Pitfalls during the performance evaluation phase can undermine the validity and rationality of LM4Code models. One key contributor is the use of inappropriate test sets. For instance, Liu \ea~\cite{liu_deep_2022} highlighted that some test sets are small and lack diversity. When they employed a new dataset, the BLEU score significantly dropped from 0.811 (on Django~\cite{oda2015learning}) and 0.646 (on HS~\cite{ling2016latent}) to 0.167. Similarly, Nong \ea~\cite{nong_generating_2022} pointed out the lack of large-scale and realistic datasets. The introduction of their new dataset led to an improvement in the F1 score. Testing on such limited datasets produces results that can be questionable, often leading to decreased performance when transitioning to cross-project validation, as noted by \cite{zeng_deep_2021}.
% Another significant contributor is the inappropriate performance measures, meaning that the selected performance metrics do not reflect the constraints of the application scenario. Intuitively, under such circumstances, test results fail to validate the model's effectiveness and reasonability in the specific domain. Once real-world data that strongly correlates with the task is used, there can be a drastic drop in performance. Moreover, many models often do not adhere to consistent evaluation protocols—they are seldom assessed using the same benchmarks, tasks, or settings, as pointed out by \cite{zeng_extensive_2022}. Alarmingly, literature containing this pitfall is the most prevalent, encompassing tasks such as vulnerability detection, code summarization, code completion, defect prediction, program repair, and code review. This prevalence underscores the severity of the issue, demanding more attention and awareness in the research community.



% \noindent \textbf{Misleading Result:}
% Researchers have limited bandwidth, and it is essential to draw upon the collective knowledge by learning from others' works. However, misleading publications, especially those presented in top-tier conferences or journals, can have a profound impact on the community and the field at large. Common tactics include underestimating costs, overhyping effectiveness, or neglecting subtle performance degradations, all in an effort to amplify perceived contributions and win over reviewers. Such practices can lead to a "bad money drives out good" scenario, inadvertently promoting more benchmarking flaws in future systems and steering the community away from genuine progress and innovation.


\subsection{RQ3-Solutions}
Given the pitfalls identified during the performance evaluation phase, it is essential to propose solutions to address these challenges and optimize the evaluation process.
We summarize the existing solutions as follows.

\noindent \textbf{Standardized and Realistic Benchmarks:}
Establishing robust and realistic benchmarks is critical for rigorous performance evaluation in LM4Code research.
Researchers should carefully select appropriate baselines based on thorough literature analysis, opting for well-established approaches tailored to specific code intelligence tasks.
This enables comprehensive capability assessment. Moreover, the community must collaboratively institute standardized benchmarks and protocols, fostering consistent evaluation. 
For example, Liu \ea~\cite{liu2023towards} highlight the need for establishing straightforward and realistic baselines to ensure truthful evaluation outcomes. 
For specific tasks, standardized task-specific benchmarks have emerged, such as VJBench proposed by Wu~\ea~\cite{wu2023effective} for automated program repair. 
Such domain-specific benchmarks facilitate targeted capability assessment.
Furthermore, diverse benchmark datasets play a significant role in comprehensively evaluating and advancing LM4Code.
For instance, Lu~\ea~\cite{lu2021codexglue} introduced CodeXGLUE, a comprehensive collection that encompasses 10 SE tasks across 14 datasets. It provides a platform for structured model evaluation and comparison across tasks using standardized baselines.


\noindent \textbf{Enhancing Reproducibility:}
Inconsistent replication remains a key pitfall during performance evaluation in LM4Code~\cite{jiang2023empirical}. 
Some solutions to enhance reproducibility have been proposed.
At its core, it's critical that code, datasets, and evaluation scripts are made publicly accessible, echoing the call for open-source initiative and providing continuously maintained links to high-quality replication packages~\cite{liu2021Reproducibility}.
Furthermore, reporting key statistical measures like variance, confidence intervals, and significance quantifies stability across runs.
Such transparency fosters community collaboration, facilitating the validation of research outcomes and paving the way for future scholarly advancements.
Carefully controlling and reporting experimental conditions like hardware specifications, software versions, random seeds, and tuning details significantly influences outcomes~\cite{hutson2018artificial}.
Chen~\ea~\cite{chen2022towards} introduced a systematic approach to train reproducible AI systems, with general criteria to evaluate reproducibility, and a unified framework to decrease randomness.




% In today's era of open-source initiatives and technological advancements, reproducibility stands paramount, especially in the realm of scientific research. It serves as a cornerstone for peer validation, iterative technological improvements, and the continued progression of science. At its core, it's imperative that code, datasets, and evaluation scripts are made publicly accessible, echoing the call for open-source endeavors and providing enduring links to high-quality replication packages~\cite{liu2021Reproducibility}. Such transparency fosters community collaboration, facilitating the validation of research outcomes and paving the way for future scholarly advancements. 
% Moreover, various methods have been proposed to address this. We recognize that factors like the inherent complexity of models, omitted details in the experimental process, and discrepancies between claimed and actual performance can be potential impediments to reproducibility~\cite{jiang2023empirical}. Hence, there's a pressing need to standardize and harmonize evaluation systems, ensuring evaluations are conducted on identical benchmarks, tasks, or settings~\cite{zeng_extensive_2022}. For instance, Chen~\ea~\cite{chen2022towards} introduced a systematic approach to train reproducible deep learning models, factoring in the stochasticity in software (like deep learning algorithms) and the non-deterministic nature of hardware (such as GPUs). Their proposition comprises three main elements: uniform standards, a unified framework, and a reproducibility guide. Furthermore, Bahaidarah~\ea~\cite{bahaidarah2022toward} unveiled an open-source platform named RE3, designed to assess the readability of R code against machine learning models trained via code readability surveys. This platform executes code files, flagging users about reproducibility errors, thus aiding in ensuring both the reproducibility and readability of projects, thereby streamlining their validation and reuse.

%%Towards Training Reproducible Deep Learning Models ICSE 22~\cite{chen2022towards} \xinyu{This paper was in the collection but deleted}
%由于软件（例如深度学习算法）中的随机性和硬件（例如 GPU）中的非确定性等问题，深度学习模型很难重现
%提出了一种训练可重复的深度学习模型的系统方法。我们的方法包括三个主要部分：(1) 一套通用标准，用于彻底评估两个不同领域的深度学习模型的可重复性；(2) 一个统一的框架，利用记录和重放技术来减轻与软件相关的随机性；以及用于控制与硬件相关的非确定性的配置文件和补丁技术，以及 (3) 可再现性指南，解释了对 DL 模型进行可再现训练过程的基本原理和缓解策略
%%Toward reusable science with readable code and reproducibility e-Science 22
%提出了一个名为RE3的开源平台，平台将评估涉及R代码可读性与通过代码可读性调查训练的机器学习模型和自动容器化服务相结合，该服务执行代码文件并警告用户重现性错误。此过程有助于确保项目的可重复性和可读性，从而快速跟踪其验证和重用 \cite{bahaidarah2022toward}
%%An Empirical Study of Pre-Trained Model Reuse in the Hugging Face Deep Learning Model Registry ICSE 23 \cite{jiang2023empirical}
%PTM 重用的三个挑战是缺少属性、声明的性能与实际性能之间的差异以及模型风险
%Addressing the challenge of reproducibility in LM4Code research necessitates a multi-faceted approach. Fundamental to this is the comprehensive documentation of every step of experimentation and the utilization of version control for both code and datasets. Extending transparency further, models, code, datasets, and evaluation scripts should be made publicly accessible, endorsing open-source initiatives. Such practices encourage community collaboration, enable the verification of findings, and lay the groundwork for subsequent research advancements. To truly capture a model's consistency and versatility, comprehensive performance metrics must be reported across multiple runs, encapsulating both mean and standard deviation values. Additionally, the community should be encouraged to actively engage in replication efforts, providing oversight for peers' work. This initiative would not only ensure model validity but also foster a refined feedback mechanism. Establishing platforms for commentaries and discussions regarding new models will further enhance collective understanding and innovation. Through transparency, open collaboration, holistic performance reporting, and community-driven replication, the reproducibility and credibility of research can be markedly augmented.




\noindent \textbf{Refined Performance Measures:}
Appropriate and comprehensive performance metrics are critical for accurately evaluating model performance on complex code-related tasks.
To address the limitations of common generic metrics like BLEU and accuracy, researchers have proposed more refined measures tailored to LM4Code challenges.
Ren~\ea~\cite{ren2020codebleu} introduced CodeBLEU to improve upon BLEU for assessing deeper semantic similarities in code generation tasks, while Eghbali~\ea~\cite{eghbali2022crystalbleu} introduced CrystalBLEU for minimizing the noise from commonly shared n-grams in programming languages.
Given the runtime nature of programming languages, metrics like compilation rate and execution accuracy on test cases have also been used~\cite{wu2023effective}.
For specific LM4Code tasks, domain-specific metrics can prove more reliable.
For example, for test oracle generation, Liu~\ea~\cite{liu2023towards} presented an evaluation metric named Found@K, which counts how many bugs can be found if developers only check the top-K recommended test cases per bug.
To better capture complex code quality attributes, direct human assessment can complement automated metrics, evaluating aspects like readability, conciseness, and correctness ~\cite{paltenghi_thinking_2021, dakhel2023github}.
Overall, more refined, code-aware, and multifaceted performance measures aligned with practical goals provide a more accurate and reliable model capability assessment.


% Various measures have been proposed to guide the testing and evaluation of neural network models. However, when metrics traditionally used in software engineering are transferred to the context of neural network models, some don't fit seamlessly. For instance, while code coverage standards play a pivotal role in software (white-box) testing, the correlation between neural network model coverage and the model's robustness has been questioned Yan~\ea~\cite{yan2020correlations}. The appropriate metric for evaluating models in different LM4SE tasks varies greatly. For example, code generation may best utilize ChrF, as Evtikhiev~\ea~\cite{evtikhiev2023out} pointed out, while Roy~\ea~\cite{roy2021reassessing} suggested reconsidering the use of BLEU as the standard metric for evaluating code summarization models. Thus, there's a pressing need for more granular and specialized performance metrics. Addressing the disparities between natural and programming languages, Eghbali~\ea~\cite{eghbali2022crystalbleu} introduced CrystalBLEU, a BLEU-based metric adept at accurately measuring code similarity. This metric retains BLEU's advantageous features, such as being language-agnostic, handling incomplete or partly incorrect codes, and efficiency, while minimizing the noise stemming from commonly shared n-grams in programming languages. Additionally, to better gauge the cost-effectiveness of neural test oracle generation in error identification, Liu~\ea~\cite{liu2023towards} presented an evaluation metric named Found@K, which ultimately led to the proposal of a more practical evaluation method, TEval+. Moreover, slight variations in automated evaluation metrics should not be the sole basis for drawing significant empirical conclusions about performance improvements; they should be backed by manual evaluations \cite{roy2021reassessing}. Extra effort should be invested in documenting anticipated use-cases and using various methods to report results, as method selection can influence evaluation outcomes and discoveries \cite{nie2021impact}.



%\cite{liu2023towards} 提出了一个名为 Found@K 的评估指标，以更好地衡量 NTOG 方法在错误查找方面的成本效益。我们提出了一种新颖的无监督排序方法来实例化此排序步骤，显着提高了 TOGA 的成本效益。最终，根据我们的实验结果和观察，我们提出了一种更切合实际的评估方法TEval+
%\cite{eghbali2022crystalbleu} 自然语言和编程语言之间的一个关键区别在于，在后者中，完全不相关的代码片段可能仅仅因为编程语言的语法冗长和编码约定而具有许多常见的 n-gram 语法。我们观察到，这些普通的共享 n 元语法阻碍了度量区分真正相似的代码示例和仅用相同语言编写的代码示例的能力。本文提出了 CrystalBLEU，一种基于 BLEU 的评估指标，可以精确有效地测量代码的相似度。我们的指标保留了 BLEU 的理想属性，例如与语言无关、能够处理不完整或部分不正确的代码、高效，同时减少了由普通共享 n 元语法引起的噪声
%\cite{nie2021impact} 不同的方法导致评估结果相互矛盾,希望未来软件工程机器学习模型的工作能够投入额外的空间来记录预期的用例并使用各种方法报告结果
%\cite{roy2021reassessing}评估指标的微小变化不应作为得出有关绩效改进的重要实证结论的唯一依据，而应得到人工评估的支持。
%\cite{nie2021impact} 我们希望未来软件工程机器学习模型的工作能够投入额外的空间来记录预期的用例并使用各种方法报告结果


%To ensure a thorough and accurate assessment of LMs, several intertwined strategies should be employed. Firstly, it is essential to adopt performance measures that genuinely reflect the task's intricacies. Considering a blend of traditional and novel metrics further enriches understanding. Collaborative workshops and forums can serve as platforms for the community to converge on best practices and share insights on pitfalls and potential refinements in model evaluation. On the dataset front, it's imperative to design test sets that mirror real-world scenarios. These sets should undergo periodic updates to incorporate emerging data and challenges, with cross-validation using diverse datasets ensuring model robustness. Furthermore, rather than exclusively relying on synthetic data, evaluations must integrate real-world scenarios to provide a genuine representation of a model's adaptability and potential limitations. Collectively, these strategies advocate for a holistic, community-driven approach to model evaluation, emphasizing real-world applicability and rigorous scrutiny.\yue{no any specific solution here}


%\noindent \textbf{Holistic Evaluation Beyond Dataset Scores:}
%The phenomenon of tailoring training on models to achieve exaggerated scores on specific datasets, known as "score chasing", has been misleading representations of genuine performance. To address this, the community urgently needs to introduce specialized detection methods and supervision mechanisms to curb this trend and ensure genuine model evaluations. Evaluating a language model's intelligence should not solely rely on dataset-specific scores but should encompass diverse and comprehensive metrics, ensuring a more accurate representation of the model's true intelligence. 
%Li \ea~\cite{li2023flm} shed light on this issue, revealing that their FLM-101B model scored the lowest average score across baseline models. However, a deeper dive into the task's nature reveals that this doesn't necessarily indicate subpar performance\yue{unclear,why}. 
%This underscores the crucial insight that evaluating a language model's intelligence should not solely hinge on scores from specific datasets. A more encompassing evaluation methodology must be employed, ensuring that the assessment of a model's intelligence remains diverse and comprehensive.
%\yue{this paragraph could be deleted, since it may be mentioned in discussion part}


% To tackle the reproducibility issue, researchers should:
% Provide comprehensive documentation detailing every step of their experiments. Use version control for both code and datasets.
% Make models, code, and datasets publicly available. Use established benchmarks that have been tried and tested by the community. Report the performance range observed across multiple runs instead of isolated results.

% \noindent \textbf{Open Source Initiatives:}
% Promoting transparency and reproducibility entails making not only datasets but also model architectures, training protocols, and evaluation scripts publicly accessible. Open-source initiatives bolster collaboration and ensure that findings are verifiable. Encouraging researchers to share their code and trained models will foster community trust and allow others to build upon and refine the presented work.

% \noindent \textbf{Comprehensive Performance Reporting:}
% Rather than focusing solely on a model's peak performance, researchers should report a comprehensive set of metrics and results across multiple runs. This provides a clearer picture of a model's stability and generalization capabilities. It is also advisable to report both the mean and standard deviation of performance metrics over multiple runs to account for variability.



% It is vital to adopt performance measures that capture the true essence of the task. Engaging in discussions and collaborative workshops can help the community converge on standard measures. Moreover, considering both traditional and novel metrics provides a holistic understanding of model performance.

% \noindent \textbf{Regular Peer Review and Feedback:}
% Establishing a system of regular peer reviews, where experts in the field critically assess models and their evaluation protocols, can identify and rectify potential pitfalls. Such collaborative efforts can foster a culture of continual improvement and shared knowledge.


% \noindent  \textbf{Curated Test Set Design:}
% Ensuring the test set is representative of real-world scenarios is crucial. Datasets should be periodically updated to incorporate new data and challenges. Cross-validation using multiple datasets can be employed to guarantee a model's robustness. Researchers should also consider diversifying data sources, and actively seeking out data from different environments and platforms.

% \noindent \textbf{Real-world Scenario Testing:}
% Instead of relying solely on synthetic datasets, incorporating real-world scenarios and data into the evaluation process will offer a more realistic assessment of a model's capabilities. It would help uncover hidden limitations and ensure that models are robust and adaptable to evolving real-world challenges.



% \noindent  \textbf{Appropriate Baseline Building and Selection:}
% To circumvent the issue of inappropriate baselines, it's paramount to adopt universally accepted or well-established baselines that are relevant to the task at hand. Conducting a rigorous literature review can help researchers identify suitable baselines. Moreover, instead of relying solely on one baseline, utilizing multiple can provide a broader perspective on the model's efficacy.
% The authors advocate for the establishment of straightforward and realistic baselines to facilitate an accurate understanding of NTOG approaches’ performance, emphasizing the necessity of addressing this pitfall to ensure reliable and truthful evaluation results in broader code intelligence research.

%To address these issues, researchers have implemented corresponding measures. As shown in Table \ref{}, these methods include updating evaluation metrics or benchmarks, employing new testing methods, developing or introducing new technologies to assist in testing, and conducting empirical studies to attempt to explain the causes and discuss the effects.


%\cite{liu_deep_2022} addresses this gap by introducing a large-scale dataset with more comprehensive and validated software requirements to facilitate a more robust evaluation. This effort underscores the critical need for using appropriate and representative test sets in performance evaluations, not just in code generation but also across a wider spectrum of tasks in code intelligence.


%As illustrated in Fig \ref{fig:Distr-evaluate-solution}, we have compiled statistics for the solutions corresponding to these problems. The four solutions of Proposing new metrics or benchmarks, Introducing new measurements, Developing new technologies, and Empirical study correspond to 6, 9, 11, and 7 pieces of literature, respectively. We will now discuss each solution in detail:
%\begin{enumerate}
    %\item \textit{Proposing new metric or benchmark.} Several innovative approaches have been introduced in recent research to address the assessment and evaluation of deep learning systems. For example, a study by \cite{aghababaeyan_black-box_2023} explores diversity metrics as an alternative to white-box coverage standards, while \cite{hu_empirical_2022} proposes a new perceptual node distribution test selection metric called DAT. There has also been a move towards specialized criteria for deep learning systems, such as the combination testing criteria specifically designed for DL systems by \cite{ma_deepct_2019}, and the introduction of Fairea, a model behavior variation method to benchmark ML bias mitigation techniques \cite{hort_fairea_2021}. Additionally, new methodologies like the importance-driven testing sufficiency standard \cite{gerasimou_importance-driven_2020} and an explainable coverage criterion achieved through constructing DNN's decision structure \cite{xie_npc_2022} further demonstrate the evolving nature of metrics and benchmarks in this rapidly advancing field. The experimental results from \cite{zeng_deep_2021} also underline the need for new metrics, as it shows that existing state-of-the-art techniques like CC2Vec may not consistently outperform other methods, highlighting the importance of continuous innovation in this area.
%\cite{aghababaeyan_black-box_2023}我们研究多样性指标作为白盒覆盖标准的替代。
%\cite{hu_empirical_2022}提出了一种新的感知节点分布测试选择度量指标DAT。
%\cite{zeng_deep_2021}尽管CC2Vec已被证明是JIT缺陷预测的最先进的技术，但它并没有与所有具有代表性的基线进行比较。实验结果表明，CC2Vec不能一致地优于Deep JIT，两者都不能一致地优于传统的JIT缺陷预测。
%\cite{ma_deepct_2019}提出了一套专门针对DL系统的组合测试准则
%\cite{hort_fairea_2021}引入了Fairea，一种模型行为变异方法来对ML偏差缓解方法进行基准测试
%\cite{gerasimou_importance-driven_2020}结合一个重要驱动( Importance-Driven，IDC )测试充分性标准
%\cite{xie_npc_2022}通过构建DNN的决策结构，提出了可解释性覆盖准则
    
    %\item \textit{Introducing new measurement.} In the backdrop of the rapid advancement of deep learning, ensuring the reliability and efficacy of models has become paramount. To this end, researchers have introduced various innovative measurement and testing methodologies. Some studies have focused on enhancing the efficiency and coverage of deep neural network testing. For instance, \cite{wang_bet_2022} proposed a black-box effective testing (BET) method for CNN models; \cite{zhang_cagfuzz_2022} designed a coverage-guided adversarial generative fuzzing method, CAGFuzz, specifically for image-based DL systems; and \cite{xie_deephunter_2019} developed a coverage-guided fuzzing framework called DeepHunter for detecting latent defects in general DNNs.
    %Other research is centered on devising novel priority testing and monitoring metrics. For example, \cite{feng_deepgini_2020} introduced DeepGini, a testing priority technique designed from a DNN's statistical perspective; \cite{pham_deviate_2021}'s DEVIATE can automatically analyze DL training codes and extract essential monitored metrics, such as accuracy and loss.
    %Further studies have concentrated on testing technologies for specific scenarios or attributes. Like \cite{lin_robustness_2019}, which developed a novel method for verifying the robustness of CDNNs with sigmoid activation functions; \cite{lee_effective_2020} offered a new white-box testing technique, Adapt, for deep neural networks that outperforms existing methods in terms of coverage discovery and adversarial input; and \cite{chen_deepperform_2022} focused on detecting IDPB in AdNNs, introducing a scalable method for generating test samples called Deep Perform.
%\cite{wang_bet_2022}提出了一种新的针对CNN模型的黑盒有效测试( BET )方法。
%\cite{zhang_cagfuzz_2022}针对基于图像的DL系统,提出了一种覆盖率引导的对抗生成模糊测试方法CAGFuzz。
%\cite{barash_bridging_2019}将经典软件的测试规划方法应用到ML-based方法中，同时保证业务价值和正确性
%\cite{feng_deepgini_2020}提出了DeepGini，一种基于DNN的统计视角设计的测试优先级技术。
%\cite{xie_deephunter_2019}提出了一种覆盖率引导的模糊测试框架DeepHunter，用于检测通用DNN的潜在缺陷
%\cite{chen_deepperform_2022}提出了Deep Perform，一种可扩展的生成测试样本的方法来检测AdNN中的IDPB
%\cite{pham_deviate_2021}提出了DEVIATE，自动分析DL训练代码并提取被监控的重要度量指标(例如准确性和损失性)
%\cite{lee_effective_2020}提出了一种新的深度神经网络白盒测试技术Adapt,它在发现的覆盖率和对抗输入方面明显比现有的测试技术更有效
%\cite{lin_robustness_2019}发展了一种新颖的方法来验证带有sigmoid激活函数的CDNNs的鲁棒性
    
    %\item \textit{Developing new technology.} In the fields of deep learning, natural language processing, and software testing, the development of new technologies has emerged as a pivotal strategy for enhancing performance evaluation capabilities. Many researchers are now concentrating their efforts in this direction, leading to an array of intriguing and valuable solutions. For instance, AEON has been introduced to meet the demand for automated test case assessment, offering scoring for each generated test case based on semantic similarity and linguistic naturalness\cite{huang_aeon_2022}. Meanwhile, in the testing of deep learning models, COMET employs a creative blend of mutation operators and search algorithms to achieve diversified testing, thereby improving efficiency and accuracy\cite{li_comet_2023}. Additionally, Flakify, a black-box, language-model-based test case predictor, has been presented, furnishing an innovative method for test case generation\cite{fatima_flakify_2023}.Apart from that, the development of Deep Janus, a search-based tool by \cite{riccio_model-based_2020}, serves as a demonstration of technological innovation in generating cutting-edge inputs for DL systems. Similarly, through the introduction of Dynamic Adaptive Neuron Coverage (DANCe), \cite{ye_dance_2022} has augmented the ability to generate adversarial samples in fuzz testing based on coverage, opening new avenues for deep learning testing.
    %In conclusion, the advent of these new technologies not only addresses existing challenges but also pioneers fresh possibilities and directions. They epitomize an in-depth understanding and creative thinking toward solutions at the performance evaluation stage, showcasing the power and potential of science and technology in tackling complex problems. As research and practice continue to evolve, these novel technologies will persist in driving innovation and progress within their respective domains.
    %%提出、应用新的技术，不是测试技术、指标、基准
%\cite{huang_aeon_2022}为了解决这个问题，我们提出了面向NLP测试用例自动评估的AEON。对于每个生成的测试用例，输出基于语义相似度和语言自然度的评分。
%\cite{xie_boosting_2022}提出了第一种对DL软件的MP进行优先级排序的方法，以促进在DL测试中检测到的违规行为的揭示。
%\cite{liu_cd-vuld_2022}提出了一种新的基于深度学习( DL )和域适应( DA )的跨域软件漏洞挖掘系统( CD-VulD )。
%\cite{li_comet_2023}COMET：( 1 )设计了一组变异算子和基于覆盖率的搜索算法，使DL模型中的层输入、层参数值和层序列多样化。( 2 )提出了一种在不牺牲层API调用多样性的情况下提高测试效率的模型综合方法。
%\cite{ye_dance_2022}提出了动态自适应神经元覆盖( DANCe )来对神经元行为进行建模，该机制增强了基于覆盖的模糊测试生成对抗样本作为测试用例的能力。
%\cite{zhang_efficient_2021}提出了一个有效发现个体公平违背的框架EIDIG
%\cite{fatima_flakify_2023}提出了Flakify，一个黑盒的，基于语言模型的片状测试用例预测器
%\cite{riccio_model-based_2020}开发了Deep Janus，这是一个基于搜索的工具，用于为DL系统生成前沿输入
%\cite{chatterjee_testing_2022}在缺乏足够的训练和测试样本的情况下，提出了一种基于真空抽气原理生成新的增广样本集的方法
%\cite{liu_can_2021}提出了一种人在环中机制，帮助神经克隆检测器适应包含大量未知功能的新代码库。

%\end{enumerate}



\begin{tcolorbox}[title=Summary - Performance Evaluation, left=2pt, right=2pt,top=2pt,bottom=2pt]
In the performance evaluation of LM4Code, we identify four pitfalls related to performance evaluation, including inappropriate baseline, inappropriate evaluation datasets, low reproducibility, and inappropriate performance measures. 
From 29 relevant research studies, inappropriate datasets and metrics receive much attention. 
Such pitfalls can lead to overestimated evaluation and compromised reproducibility, misleading benchmarks for the future. 
To address this, tailored solutions like standardized benchmarks, transparency, realistic assessments, and community coordination are needed.
\end{tcolorbox}


\section{Deployment and Maintenance}
\label{sec:deployment}
Systems based on advanced LM4Code, such as GitHub Copilot~\cite{github2021copilot}, Amazon CodeWhisperer~\cite{amazon2022codewhisperer}, and Microsoft IntelliCode~\cite{svyatkovskiy2020intellicode}, have already been deployed in real-world IDEs and have garnered a large number of users.
There exist various challenges when such LM4Code systems are deployed in practice, like security threats and how LM4Code systems should be updated to adapt the rapidly changing software practices.
This section discusses pitfalls, implications, and current solutions when deploying and maintaining LM4Code.


\begin{figure}[t]
  \centering
  \begin{minipage}{0.5\linewidth}
    \centering
    \includegraphics[height=3.5cm, keepaspectratio]{images/maintainance/fig7_stage4_deploy_bias_distri_time.pdf} 
    \caption{Paper distribution across time (Section~\ref{sec:deployment}) }
    \label{fig:result_deploy_bias_time}
  \end{minipage}%
  \hfill
  \begin{minipage}{0.5\linewidth} 
    \centering
    \includegraphics[height=3.5cm, keepaspectratio]{images/maintainance/fig7_stage4_deploy_bias_distri_models.pdf}
    \caption{Distribution of LMs (Section~\ref{sec:deployment}) }
    \label{fig:result_deploy_bias_models}
  \end{minipage}
\end{figure}



\subsection{RQ1-Pitfalls}
In our literature review, we identified 25 research papers involving the pitfalls of LM4Code deployment and maintenance.
This number of identified publications surpasses that related to other stages, highlighting the fact that deploying and maintaining LM4Code presents a complex set of challenges that have gained considerable attention from the research community.

Figure~\ref{fig:result_deploy_bias_time} and Figure~\ref{fig:result_deploy_bias_models} present the distribution of these 25 research studies over time and different types of LLM4Code.
From Figure~\ref{fig:result_deploy_bias_time}, we can observe that there has been a significant increase in the number of research papers focusing on the pitfalls in the deployment and maintenance of LM4Code, especially in the past two years. 
The data presented in Figure~\ref{fig:result_deploy_bias_models} demonstrates a significant preference for utilizing the Codex model for analyzing biases related to deployment and maintenance, which may be due to the fact that the widely used Github Copilot is based on Codex.
Moreover, large pre-trained models such as CodeT5, BERT, Codex, and GPT-2 appear to surpass traditional LMs such as RNN and LSTM in terms of widespread use and popularity.
These observed patterns indicate a shift in research focus towards investigating the complexities of advanced models when deployed in real-world contexts. 
In the subsequent sections, we will examine the particular biases and issues that arise in regard to the development and maintenance of LM4Code.

\vspace{0.2cm}
\noindent \textbf{Real-World Constraints:} 
Evaluating LM4Code systems solely in controlled lab settings often overlooks practical constraints and complexities of real-world deployment~\cite{arp2022and}.
Although controlled evaluations provide useful insights into the effectiveness of a model within specific settings, they sometimes overlook the complexity and diversity of real-world deployments.
It is important to consider runtime and storage constraints when deploying an LM4Code system in the wild.
Svyatkovskiy~\ea~\cite{svyatkovskiy2021fast} mentioned that a reasonable upper bound of model size for an IDE plugin is 50 MB.
However, the size of LM4Code keeps increasing.
For example, the popular LM4Code, CodeBERT~\cite{feng2020codebert}, has 125 million parameters and is 425 MB in size, which is way larger than the suggestion by Svyatkovskiy~\ea~\cite{svyatkovskiy2021fast}.
Recently proposed models are even larger.
Considering LLaMa, developed by Meta, its smallest version has 6.7B parameters~\cite{lu2023llama}.
Models that appear to have good performance in a controlled setting may be resource-intensive or excessively large for practical applications, especially in environments with limited computational power or storage capacity~\cite{feng_performance-sensitive_2021}.
% Secondly, lab-only evaluations often overlook the human aspect: how developers interact with LM4Code like AI coding assistants, their preferences for usability, and potential security issues in collaborative coding settings~\cite{sandoval2023lost, barke2023grounded,hellendoorn_when_2019}.


\vspace{0.2cm}
\noindent 
\textbf{Attack Threats:}
LM4Code systems face various threats from malicious attackers.
Despite the breakthrough capabilities exhibited by LMs, prior works have noted that the state-of-the-art LMs are vulnerable to a variety of attack threats such as evasion attacks~\cite{zhou_adversarial_2022, wang2023robustness, mastropaolo2023robustness}, backdoor attacks, privacy attacks, etc.
These threats can appear across the entire lifecycle of the model, from data collection to model deployment.
% Under such attacks, models consistently fail to produce outputs that are both accurate and trustworthy~\cite{barreno2006can}.
We identified a total of 17 research papers that specifically focus on the analysis of security threats within the LM4Code system.
Figure~\ref{fig:result_deploy_bias_time} shows that the number of these studies has increased over the recent years.
% These findings highlight the growing concern and emphasis on attack threats within the LM4Code domain.
Our study employs the classification scheme mentioned in Battita \ea's work~\cite{biggio2018wild}, which has identified a diverse range of attack types in machine learning.

\begin{enumerate}
    \item \textit{Evasion Attacks:} Evasion attacks (a.k.a. adversarial attacks) leverage adversarial samples~\cite{liu2023contrabert, zhou_adversarial_2022}, which are carefully perturbed instances while appearing as regular and benign inputs to the human observer.
    Yet, these small perturbations can mislead the trained LM4Code model to produce incorrect predictions.
    As shown in Table~\ref{tab:summary_model_attacks}, evasion attacks are a major concern, with 9 out of the 17 examined papers investigating them.
    Zeng~\ea~\cite{zeng_extensive_2022} thoroughly evaluated eight different adversarial attack approaches (i.e., word importance rank, genetic algorithm, random substitution) against widely-used LM4Code, including CodeBERT, GraphCodeBERT, and CodeT5.
    Their findings emphasized the vulnerability of these models to semantics-preserving adversarial samples.
    Interestingly, even simple random attack techniques showed significant effectiveness in degrading pre-trained LM4Code.
    
    \item \textit{Poisoning Attacks:} Poisoning attacks inject malicious examples into the training data, aiming to manipulate the model's behavior~\cite{biggio2018wild, sun2022coprotector}. 
    This can lead the model to produce incorrect or attacker-chosen outputs when certain triggers appear in the inputs~\cite{schuster2021you}.
    Poisoning attacks can be categorized into two main classes: untargeted poisoning attack and targeted poisoning attack~\cite{tian2022comprehensive}.
    One special case of the target poisoning attack is the backdoor attack, where adversaries carefully insert a distinct pattern into a subset of training samples to embed a backdoor.
    When the pattern appears, the model produces pre-defined outputs (e.g., recommending vulnerable APIs).
    Otherwise, the model behaves normally.
    Table~\ref{tab:summary_model_attacks} lists six papers related to poisoning attacks, with all of them specifically focusing on backdoor attacks.
    Among various code scenarios, three studies~\cite{wan_you_2022, sun2023backdooring, sun2022coprotector} target LMs-based code search models, demonstrating that backdoor samples within code search tasks closely resemble clean code and are not easily differentiated. 
    Four studies~\cite{schuster2021you, li2023multi, sun2022coprotector, peng2022security} focus on code generation scenarios, demonstrating that attackers can manipulate code recommendations.

    \item \textit{Privacy Attacks:}  
    Privacy attacks refer to attacks aiming to infer the private information of LM4Code, e.g., parameters of models that are hosted remotely and the model training data.
    One such example is model stealing (a.k.a. model extraction) involves extracting knowledge (e.g., hyperparameters, model architecture, and training data) from a trained model without direct access to its parameters or training data~\cite{carlini2021extracting, oliynyk2023know}. 
    Adversaries use this technique to `copy' the functionality of a model, often by querying it repeatedly and analyzing the outputs~\cite{oliynyk2023know}.
    For example, Lukas~\ea~\cite{lukas2023analyzing} delved into the risk of language models, like GPT-2, leaking personally identifiable information. 
    Yang et al.~\cite{yang2023code} found that simply extracting 20,000 outputs (each having 512 tokens) from CodeParrot~\cite{codeparrot} can produce over 40,125 code snippets that are memorized from its training data.
    In addition, Niu~\ea~\cite{niu2023codexleaks} introduced and evaluated a semi-automated pipeline that employs a membership inference approach on various code generation models like CodeParrot~\cite{codeparrot} and Polycoder~\cite{xu2022systematic}. 
    By leveraging the GitHub Search API's hit rate as a distinguishing heuristic and incorporating human-in-the-loop evaluations, they found that approximately 8\% (43) of the prompts in the Codex model, used in GitHub Copilot, resulted in privacy leaks.

\end{enumerate}


\input{tables/yy_tables/tab2_model_attack_summary}


\vspace{0.2cm}
\noindent 
\textbf{Security Concerns in Generated Code:} 
The outputs from LM4Code, i.e., generated code, will be further used in other software systems. 
Consequently, the safety and robustness of the generated code come under scrutiny. 
Several recent investigations have shown that LM-generated code can contain vulnerabilities, emphasizing the need for rigorous validation and enhancement of their outputs.
Pearce~\ea~\cite{pearce_asleep_2022} analyzed the generated code of GitHub Copilot and identified security vulnerabilities. 
The authors produced 89 different scenarios for Copilot to complete, resulting in 1,689 programs. Alarmingly, they found approximately 40\% of these to be vulnerable. 
Such vulnerabilities arise because code often contains bugs, and given the vast quantity of unvetted code that Copilot processes, the language model is prone to learning from exploitable and buggy code.


\subsection{RQ2-Implications}
According to the reviewed papers, the identified pitfalls and security concerns related to the deployment and maintenance of LM4Code have significant implications for both researchers and practitioners in artificial intelligence and software engineering.
Next, we will describe the implications in detail.

\noindent 
\textbf{Untrustworthy Results:} 
Both the pitfalls from external attackers and internal drawbacks can lead to untrustworthy outputs, requiring the developers to carefully review and test the generated code.
External attacks like evasion, poisoning, and backdoor attacks, can induce LM4Code systems to demonstrate manipulated behavior, i.e., generating outputs specifically chosen by attackers.
For example, Schuster \ea~\cite{schuster2021you} demonstrate that code completion models can be manipulated to use unsafe encryption algorithms and deprecated security protocol so that the system built based on these suggestions is vulnerable to further attacks.
Aghakhani \ea~\cite{aghababaeyan_black-box_2023} reveal that the backdoors in code generation models can inject various insecure code, including Cross-Site Scripting (CWE-79), Path Traversal (CWE-22), and Deserialization of Untrusted Data (CWE-502).
Wan \ea~\cite{wan_you_2022} can mislead the code search models to retrieve the code snippets containing malicious actions, such as deleting specific files.
Attackers can also provoke systems into producing unexpected predictions so that the application behaves in an unintended way.
For example, the adversarial attacks~\cite{yang2022natural, zhang_challenging_2023} against LM4Code Systems can lead to completely wrong predictions.
Even without external attacks, the model itself may also naturally generate untrustworthy results, which has been largely reported in various studies.
For instance, Pearce~\ea~\cite{pearce_asleep_2022} revealed vulnerabilities frequently present in GitHub Copilot's generated code.
Furthermore, Lukas~\ea~\cite{lukas2023analyzing} suggested LMs may inadvertently retain or even leak portions of their training data, which raises concerns regarding unintentional memorization of sensitive information.
Niu~\ea~~\cite{niu2023codexleaks} investigated code completion models like the popular Codex model leaking private information (e.g., passwords and addresses) through generated outputs.

% highlighted that the code generated by GitHub Copilot frequently exhibits vulnerabilities, which can be attributed to the enormous amount of unchecked code that Copilot has been exposed to. Moreover, Lukas~\ea~\cite{lukas2023analyzing} posited that LMs might inadvertently retain portions of information they have learned from their training data. Additionally, concerns about individual privacy breaches in software engineering tasks have emerged. Niu~\ea~\cite{niu2023codexleaks} delved into instances where models leak sensitive personal information through their code completions. Their findings suggest that models often generate indirect leaks, jeopardizing privacy by producing information about individuals who are closely associated with the queried subject from the training dataset, thus compromising contextual integrity.
% \su{1. unsecure output. 2. directly copy training data 3. leak personal information. One example for each.}

\noindent 
\textbf{Copyright Infringement:}
Pitfalls in LM4Code deployment raise significant concerns regarding copyright infringement and loss of intellectual property.
Attackers might resort to model stealing, effectively replicating the functionality of proprietary models without authorization~\cite{johnson2023ru, li2023feasibility}.
Li~\ea~\cite{li2023feasibility} demonstrate that imitation models can even exceed the performance of the victim model.
Additionally, when models are deployed on user clients, they face the potential threat of reverse engineering.
Zhou~\ea~\cite{zhou2023modelobfuscator} highlight that the on-device models may leak their confidential information, such as hyper-parameters and weights.
% Training ata extraction attacks on LM4Code systems can leak private training data and user information~\cite{lukas2023analyzing, niu2023codexleaks}.
The risk of copyright infringement and intellectual property theft not only undermines incentives to develop innovative models, but also threatens the commercialization prospects and trustworthiness of the LM4Code industry.


% Sun~\ea~\cite{sun2022coprotector} highlighted the potential exploitation of open-source code by deep learning models, raising concerns related to copyright, ethical issues, and security implications.
% Peng~\ea~\cite{peng2022security} demonstrated that the text-to-SQL modules in commercial applications can be manipulated to produce malicious code, potentially leading to data breaches.
% Lukas~\ea~\cite{lukas2023analyzing} pointed out that LMs are susceptible to black-box extraction, inference, and reconstruction attacks, which can leak information about the training data and personally identifiable information (PII).
% Niu~\ea~\cite{niu2023codexleaks} discovered that the Codex model used in GitHub Copilot could be vulnerable to semi-automatic filtering methods for blind member inference attacks, leading to privacy leaks.

\noindent 
\textbf{Compromised Model Efficacy:} 
In real-world practice, many constraints, such as latency, device memory, and computational costs, need to be satisfied.
On the one hand, it prevents some powerful models from being deployed.
For instance, Feng~\ea~\cite{feng_performance-sensitive_2021} noted multiple malware detection models are infeasible on mobile devices due to limitations in computational power, memory, and energy consumption. 
Zhang~\ea~\cite{zhang_diet_2022} highlighted that even standard CodeBERT requires extensive resources for pre-training and fine-tuning before use, which may not be affordable for individual developers.
On the other hand, the performance of deployed systems may be compromised as a trade-off. 
For example, to be deployed on the user devices, the models have to be pruned or distilled, where considerable performance degradation can be observed~\cite{shi2022compressing, shi2023smaller}.
Furthermore, Ganesh~\ea~\cite{ganesh2021compressing} showed that while quantization and unstructured pruning can reduce model size, these techniques alone do not improve runtime inference speed or memory usage during execution, unless paired with specialized hardware or processing libraries.
Therefore, while constraints exist in real-world deployment that compels simpler models, such compromises often degrade model performance, highlighting the need for techniques that can provide comparable accuracy with greater efficiency.



% \xinyu{More examples:}
% %Compressing BERT: Studying the Effects of Weight Pruning on Transfer Learning. 
% %中等水平的剪枝会增加预训练损失，并阻止有用的预训练信息转移到下游任务。高水平的修剪还会阻止模型拟合下游数据集，从而导致进一步退化
% Gordon~\ea~\cite{gordon2020compressing} noted that pruning can cause pre-training loss, and excessive pruning may even hinder model adaptation to downstream datasets, causing performance decline
% %Compressing Large-Scale Transformer-Based Models: A Case Study on BERT. TACL 21 
% %架构不变的模型压缩准确率下降较小，非结构化的模型压缩精度/F1 大幅下降
% Ganesh~\ea~\cite{ganesh2021compressing} highlighted that with consistent architecture, model compression results in a minor decline in accuracy, whereas unstructured model compression significantly reduces precision/F1 scores.
% %Improved Knowledge Distillation via Teacher Assistant. AAAI 20 
% %模型容量较低的小型学生模型无法有效地从大型模型中吸收知识，这使得小型模型的性能大大低于大型模型
% Small student models with lower capacity struggle to effectively absorb knowledge from larger models, resulting in their performance being substantially inferior to that of the larger models\cite{mirzadeh2020improved}.

% Zhang~\ea~\cite{zhang_diet_2022} highlighted that even standard CodeBERT requires extensive resources for pre-training and fine-tuning before use.
% For example, despite having 125 million parameters, CodeBERT still demands over 28 hours for pre-training on just 8.5 million code snippets~\cite{zhang_diet_2022}. 
% The performance of LM4Code systems in real-world practice may become compromised due to various constraints including latency, device memory, and computational costs.
% Several studies have shown performance declines when models face security attacks.
% For example, Zhou~\ea~\cite{zhou_adversarial_2022} employed adversarial examples in their research, identifying a drastic decline in the BLEU score of language models used for code comment generation (e.g., decrease from 44.58\% to 13.13\%).
% Similarly, Pearce~\ea~\cite{pearce_examining_2023} demonstrated that neural code completion models are susceptible to poisoning attacks, with accuracy dropping substantially (e.g., decrease from 41\% to 29\%).
% At the same time, performance constraints emerge during deployment as well.

% Furthermore,  while pre-trained models achieve high accuracy in labs, their computational demands often hinder utility in real-world deployment. 
% Although considered small relative to other large language models, 



% Apart from that, while deep learning-based approaches can be efficiently maintained server-side for malware detection, the raw deep learning models are infeasible for direct deployment and execution on mobile devices due to various performance constraints such as computational power, memory size, and energy consumption \cite{feng_performance-sensitive_2021}. 
% Additionally, Schuster~\ea~\cite{schuster2021you} underscored that neural code autocompleters are not only vulnerable to poisoning attacks but also that the existing defenses prove largely ineffective. The false positive rate (FPR) and recall for both defenses (activation clustering and spectral signature) are alarmingly high, with rates of 81.0\%, 86.0\%, 83.2\%, and 80.0\% respectively. 
% Furthermore, Zhang~\ea~\cite{zhang_diet_2022} noted that while pre-trained models have made impressive strides in accuracy, their computational weightiness often impedes practical applications. For example, the standard CodeBERT comprises 125 million parameters and demands 28 hours to pre-train on 8.5 million code snippets. What's more pivotal is that pre-trained models typically necessitate fine-tuning prior to utilization. Given the vast scale of parameters and training data, this process is often cost-inefficient.

\subsection{RQ3-Solutions}
\subsubsection{Improving Model Robustness} 
Improving model robustness is essential to defend against evolving security threats targeting LM4Code systems. 
Here, we summarize some of the available solutions that have been proposed to enhance the robustness of LM4Code models:

\noindent \textbf{Adversarial Training:}
Adversarial training incorporates adversarial examples into training data to improve model robustness against adversarial attacks.
Regarding code comment generation, Zhou~\ea~\cite{zhou_adversarial_2022} demonstrated masked adversarial training can significantly enhance robustness while retaining performance on normal test data. 
Zhang~\ea~\cite{zhang_generating_2020} illustrated that adversarially trained language models exhibit markedly reduced attack success rates (approximately 30\%-40\%).
Moreover, Henkel~\ea~\cite{henkel_semantic_2022} implemented robust optimization employing a semantics-preserving adversary, and this approach outperformed standard data augmentation, optimally balancing accuracy on clean samples with robustness to perturbations.




% for example, introduced ACCENT (Adversarial Code Comment gENeraTor), an identifier substitution methodology devised to generate adversarial code snippets. While these snippets maintaining syntactic correctness and semantic resemblance to the original code, have the potential to lead DNNs astray, prompting them to produce entirely irrelevant code comments. Their exhaustive experiments underscored the effectiveness of this approach in bolstering model resilience. 
% Coincidentally, Zhang~\ea~\cite{zhang_generating_2020} came up with a Metropolis-Hastings sampling-based identifier renaming technique, which generates adversarial examples for DL models specialized for source code processing. 
% Henkel et al. \cite{henkel_semantic_2022} delved deeper into the specifics. To facilitate the training of robust models, they defined a formidable and versatile adversary capable of employing parameterized, semantically-preserving program transformations. They further explored how to train models that exhibit robustness against adversarial program transformations with the aid of such an adversary.


% \su{I merge this section into the external support section}
% \noindent \textbf{Error Detection:}
% A key strategy for improving the safety of LM4Code is detecting errors/anomalies in the training data or model outputs to prevent errors from causing system failures.
% % For data anomalies, Schuster~\ea~\cite{schuster2021you} and Sun~\ea~\cite{sun2022coprotector} demonstrated techniques like activation clustering and spectral signature can identify distinguishable anomalies for poisoning attacks.
% For output anomalies, runtime error detection is commonly used. 
% When the model detects potential output anomalies, it can trigger fail-safe runtime checks to prevent system failure.
% Xiao~\ea~\cite{xiao2022self} proposed SelfChecker that detects inconsistencies in model outputs, demonstrating it triggered correct failure alarms on 60.56\% of incorrect predictions.
% Moreover, Zhao~\ea~\cite{zhao2021attack} developed techniques to distinguish adversarial examples from benign ones, rejecting potentially adversarial inputs by leveraging attack cost estimation for adversarial example detection.


% Despite protective measures applied to models, the emergence and evolution of malicious samples remain relentless, making their detection a focal point of ongoing concern. 
% Xiao et al. \cite{xiao2022self} addressed the challenges presented at runtime. Specifically, they introduced a technique dubbed SelfChecker++, which transforms any runtime inputs that trigger alarms into their semantically equivalent counterparts, which are then reintegrated into the model. This dynamic transformation neutralizes any intentionally designed samples, thereby immunizing the model against attacks using such inputs. Feature detection stands as a prevalent method for detecting malicious samples. 
% However, based on observations by Zhao et al. \cite{zhao2021attack}, the robustness of adversarial samples is notably inferior to benign samples. Consequently, they incorporated a distinct feature to differentiate between the two. They further unveiled a defensive framework named Attack-to-Defend (A2D), designed to pinpoint adversarial examples by adeptly gauging an example's robustness.

% \xinyu{These two articles are not in the final 68 references, but read during manual filtering process.}

% \noindent \textbf{Poison Attack and Defense on Deep Source Code Processing Models:}
% The integrity of LMs has been shown to be compromised by poisoning attacks. Schuster et al. \cite{schuster2021you} demonstrated that the mere addition of specially-crafted files to the training dataset (a method known as data poisoning) or by directly fine-tuning the autocompleter on these files (termed model poisoning) enables an attacker to manipulate its suggestions within specified contexts. Similarly, Wan et al. \cite{wan_you_2022} explored and crafted a set of backdoor attacks tailored for deep-learning-based models used in code search. By employing data poisoning, they revealed a straightforward yet potent method of assaulting neural code search models by contaminating their primary training datasets. Recognizing the impending threats posed by such attacks, Sun et al. \cite{sun2022coprotector} took a proactive stance. They conceptualized and brought to life a prototype named CoProtector. This system leverages data poisoning techniques not for nefarious purposes, but rather as a protective shield, fortifying source code repositories against potential exploitations.


\noindent \textbf{Inference with Self-repair:}
Self-repair is to let the model introspect and correct mistakes or vulnerabilities in its own code.
Delving into this, Olausson~\ea~\cite{olausson2023demystifying} investigated to what extent the GPT models can provide accurate feedback on the causes of code errors, validating the efficacy of GPT-4's self-repair capabilities. 
Moreover, Chen~\ea~\cite{chen2023improving} enhanced the self-repair process by incorporating knowledge from human-written natural language feedback.


\noindent \textbf{Domain Knowledge:}
Beyond the internal capability of the model, external aids with domain knowledge can also be employed to address the challenges.
For instance, Jain~\ea~\cite{jain2022jigsaw} enhances these LLMs by utilizing a post-processing step based on program analysis and synthesis techniques, thereby improving the correctness of the syntax and semantics in code. Wei~\ea~\cite{wei2023copiloting} introduced Repilot, a framework designed to further assist AI "copilots" (i.e., LLMs) by synthesizing more valid patches during the repair process.
Moreover, Johnson~\ea~\cite{johnson2023ru} proposed Random Utility-Driven Synthesis Under Uncertain Regions (R-U-SURE), a method that builds uncertainty-aware suggestions based on a decision theory model of objective conditional utility, using random samples from generative models as proxies for unobserved potential intents of end-users.
Poesia \ea~\cite{poesia2022synchromesh} propose a framework to apply constraints on partial outputs to produce complete correct programs without re-training or fine-tuning of the language model.


% Moreover, Zhao~\ea~\cite{zhao2021attack} developed techniques to distinguish adversarial examples from benign ones, rejecting potentially adversarial inputs by leveraging attack cost estimation for adversarial example detection.

\noindent \textbf{Train with Real-world Dataset:}
Directly learning from the real-world datasets helps the model to better align with the user intention.
For instance, Aye et al.~\cite{aye2021learning} observed a significant decline in the accuracy of Transformer sequence models when tested using real-world data from production logs.
Moreover, they demonstrated that training on real-world examples yields a more robust model.
However, there is a significant shortage of large-scale, real-world datasets, especially for vulnerability.
Nong~\ea~\cite{nong_generating_2022} suggest a promising alternative solution: using deep learning to generate real-world samples.



\subsubsection{Enhancing Computational Efficiency}
To make full use of the limited resources, various measures have been proposed.

\noindent \textbf{Model Compression and Specialization:}
To enable the deployment of large language models in resource-constrained environments, model compression techniques have been widely explored~\cite{polino2018model, gupta2022compression}. 
Shi~\ea~\cite{shi2022compressing} introduced Compressor, which uses a genetic algorithm to guide the simplification of pre-trained code models. 
This compressed models to significantly smaller sizes with acceptable accuracy loss.
In addition to compression, methods to specialize large language models (LLMs) for specific tasks show promise. 
Parameter-Efficient Fine-Tuning (PEFT) effectively adapts LLMs using limited task data. 
As Weyssow~\ea~\cite{weyssow2023exploring} demonstrated, PEFT outperforms approaches like Incremental Curriculum Learning in reducing computational overhead and boosting performance when specializing broad LLMs.



% the Parameter-Efficient Fine-Tuning (PEFT) technique holds great promise in effectively specializing LLMs to task-specific data. Experimental results from \cite{weyssow2023exploring} highlight the superiority of such techniques over Incremental Curriculum Learning (ICL) in both alleviating computational burdens and enhancing performance for broader LLMs. Moreover, high-quality performance testing is crucial when addressing performance requirements in resource-constrained environments. For instance, to tackle the performance degradation caused by redundant computations in AdNN, Chen~\ea~\cite{chen2022deepperform} proposed DeepPerform. This tool generates test samples to detect IDPB in AdNN and addresses optimization challenges effectively by learning and estimating the distribution of computational costs.

%%Compressing Pre-trained Models of Code into 3 MB.
% \cite{shi2022compressing} Compressor，这是一种新颖的方法，可以将预先训练的代码模型压缩为极小的模型，而性能损失可以忽略不计
%%Exploring Parameter-Efficient Fine-Tuning Techniques for Code Generation with Large Language Models
%\cite{weyssow2023exploring} 预见到参数高效微调（PEFT）技术在将法学硕士有效地专业化到特定于任务的数据方面具有很大的潜力。在本文中，我们对自动代码生成场景下 PEFT 技术的影响进行了LLMs的全面研究。我们的实验结果揭示了此类技术在减轻计算负担和提高性能方面比 ICL 更广泛的法学硕士的优越性和潜力。因此，该研究为 PEFT 在软件工程场景中更广泛的应用提供了机会
%%DeepPerform: An Efficient Approach for Performance Testing of Resource-Constrained Neural Networks
%\cite{chen2022deepperform} 为了确保 AdNN 满足资源受限应用程序的性能要求，必须进行性能测试以检测 AdNN 中的 IDPB。现有的神经网络测试方法主要关注正确性测试，不涉及性能测试
%提出了DeepPerform，这是一种可扩展的方法，用于生成测试样本以检测 AdNN 中的 IDPB。我们首先演示如何将生成检测 IDPB 的性能测试样本的问题表述为优化问题。接下来，我们演示 DeepPerform 如何通过学习和估计 AdNN 计算消耗的分布来有效处理优化问题

\noindent \textbf{Efficient Inference:}
Numerous inference optimization strategies have also been proposed. 
For instance, Zhang~\ea~\cite{zhang_diet_2022} adopted input simplification strategies like word dropout and frequency filtering to simplify input programs.
By focusing on the most informative tokens, computational costs are significantly reduced.
Additionally, Chirkova~\ea~\cite{chirkova2023codebpe} introduced a tokenization method that reduces the average token length by 17\% without any downstream performance loss.
They further demonstrated that a properly chosen tokenization can even enhance the model's performance by 0.5-2\%. 
Furthermore, Svyatkovskiy~\ea~\cite{svyatkovskiy2021fast} unveiled an innovative neural completion model by combining static analysis with granular token encoding. This model boasts a lean memory footprint, consuming just 6 MB of RAM — a significant 19x reduction compared to previous models.
It can generate a single piece of code completion in a mere 8 ms and delivers an impressive 90\% accuracy rate for its top five suggestions.

%%Diet Code Is Healthy: Simplifying Programs for Pre-trained Models of Code 
% \cite{zhang_diet_2022}
%Based on these findings, we propose DietCode, which aims at lightweight leverage of large pre-trained models for source code. DietCode simplifies the input program of CodeBERT with three strategies, namely, word dropout, frequency filtering, and an attention-based strategy that selects statements and tokens that receive the most attention weights during pre-training.
%it gives a substantial reduction in the computational cost without hampering the model performance
%%CODEBPE: INVESTIGATING SUBTOKENIZATIONOPTIONS FOR LARGE LANGUAGE MODELPRETRAINING ON SOURCE CODE
%subtokenziation that reduces average token length by 17% without downstream performance drop, and show that a carefully chosen subtokenization may improve quality by 0.5-2%
%%Fast and Memory-Efficient Neural Code Completion
%设计了一种新颖的重新排序神经完成模型，该模型将静态分析与粒度令牌编码相结合。最好的神经重新排序模型仅消耗 6 MB RAM，比以前的模型少 19 倍，可在 8 毫秒内计算出单个完成结果，并在前 5 个建议中实现 90% 的准确率 \cite{svyatkovskiy2021fast}

\subsubsection{Privacy and Copyright Protection}
The ability of large language models to memorize and reproduce training data raises critical privacy and copyright concerns.
Thus, developing effective protection for privacy and copyright has been widely investigated.

\noindent \textbf{Privacy-preserving Techniques:}
The memorization and regeneration capabilities of large language models raise critical privacy concerns that demand research attention.
Some state-of-the-art models like StarCoder employed human annotators to mask any personal information such as keys and addresses present in the training data, in an effort to mitigate privacy risks~\cite{li2023starcoder}.
% However, Niu~\ea~\cite{niu2023codexleaks} demonstrate that despite these protection strategies, privacy leakage remains present in StarCoder.
In addition, differential privacy techniques have emerged as promising strategies for mitigating privacy risks.
Lukas~\ea~\cite{lukas2023analyzing} introduce a sentence-level differential privacy approach, which provides guarantees under the assumption that records are unlikely to be duplicated.
Their results show that while helpful in reducing privacy leakage to a large extent, differential privacy alone cannot completely eliminate risks.
Further research into complementary privacy-preserving mechanisms is needed to develop LM4Code that generates high-quality outputs while provably protecting user privacy.

\noindent \textbf{Model Obfuscation:}
Obfuscating models by hiding their structure and parameters has been proposed as a technique to protect against extraction attacks.
Prior Research has shown that attackers can easily craft white-box-like attacks against models on devices, even to the extent of reversing their training data~\cite{huang2021robustness}.
For example, Zhou~\ea~\cite{zhou2023modelobfuscator} developed ModelObfuscator to apply techniques like model file obfuscation and model structure obfuscation. 
In model file obfuscation, they utilized renaming, parameter encapsulation, and neural structure obfuscation approaches, effectively obfuscating the data and structures of on-device models.
model structure obfuscation utilizes shortcut and extra layer injection, making reverse engineering harder.
Although model obfuscation has shown promise by Zhou~\ea~\cite{zhou2023modelobfuscator}, it can increase library size, introducing extra memory overhead and computation time.
Further research is needed to balance security, efficiency, and accuracy as model obfuscation techniques are applied.


% Research has shown that attackers can easily craft white-box-like attacks against models on devices, even to the extent of reversing their training data. 
% Model obfuscation seeks to hide and scramble crucial model information — its structure, parameters, and attributes — through techniques like renaming, parameter encapsulation, neural structure obfuscation, shortcut injection, and additional layer insertion, thereby safeguarding models on devices from white-box attacks \cite{zhou2023modelobfuscator}. Specifically, Zhou~\ea~\cite{zhou2023modelobfuscator} developed a prototype tool named ModelObfuscator to automatically obfuscate TFLite models on devices. This method significantly bolsters the security of models by markedly increasing the difficulty of parsing their internal information without adding latency to the deep learning models.


%\cite{zhou2023modelobfuscator}
% 为了保护设备上的模型免受白盒攻击，提出了一种称为模型混淆的新技术。具体来说，模型混淆通过重命名、参数封装、神经结构混淆、快捷方式注入、额外层注入等方式隐藏和混淆模型的关键信息——结构、参数和属性。
%这种提出的方法可以通过显着增加解析模型内部信息的难度来显着提高模型的安全性，而不会增加深度学习模型的延迟。

\noindent \textbf{Watermarking:} 
Watermarking techniques can help protect model intellectual property.
For instance, Sun~\ea~\cite{sun2022coprotector} introduced CoProtector, which uses data poisoning to embed watermarks into source code repositories.
This ensures open-source code can't be exploited by models while providing a way to reveal watermark backdoors.
However, CoProtector notably diminishes model performance, making it hard to adopt broadly.
In neural code completion, Sun~\ea~\cite{sun2023codemark} proposed CodeMark which embeds imperceptible user-defined watermarks into code.
This traces code utilization while meeting key watermark properties like harmlessness, verifiability, and robustness.
%%CodeMark: Imperceptible Watermarking for Code Datasets against Neural Code Completion Models \cite{sun2023codemark}
%CodeMark 的方法，将用户定义的难以察觉的水印嵌入到代码数据集中，以跟踪它们在训练神经代码补全模型中的使用情况。 CodeMark 基于自适应语义保留转换，可保留代码数据的确切功能并保持更改的隐蔽性以防止规则破坏。
%%Coprotector: Protect open-source code against unauthorized training usage with data poisoning \cite{sun2022coprotector}
%To mitigate such impacts, we argue that there is a need to invent effective mechanisms for protecting open-source code from being exploited by deep learning models. Here, we design and implement a prototype, CoProtector, which utilizes data poisoning techniques to arm source code repositories for defending against such exploits.

% \textbf{Check exact-match output:}
% %I don't know whether there is a paper. Github Copilot has implemented this as a feature. Maybe we can cite its website instead. (https://github.com/settings/copilot)
% We also noted that in July 2022, GitHub Copilot introduced the "Check exact-match output" feature. This functionality is designed to detect whether the code generated by Copilot precisely matches any code in the GitHub public repositories, thereby preventing Copilot from producing code that might infringe on copyrights or software licenses.








% stringent game-theoretic rules for three types of PII leakage via black-box extraction, inference, and reconstruction attacks, accessing the LM solely through its API. They also demonstrated that sentence-level differential privacy reduces the risk of PII leakage. 
% Additionally, auditing LMs for privacy breaches before deployment is a proactive approach. Niu~\ea~\cite{niu2023codexleaks} proposed a semi-automatic filtering method using blind membership inference attacks, leveraging hit rates from the GitHub search API as a distinguishing heuristic, followed by a human-machine interactive assessment. Alarmingly, they found that about 8\% (43 prompts) of the Codex model used in GitHub Copilot resulted in privacy breaches.
% To mitigate the potential for privacy breaches as much as possible, Li~\ea~\cite{li2023starcoder} have even gone to the lengths of hiring human annotators to mask personal information in the training data. 









%  we have examined whether the corresponding issues were addressed in the 18 articles we reviewed. Overall, 15 of the 18 articles presented solutions to the respective problems. 

% Specifically, for "Lab-Only Evaluation," we found that only one of the three papers offered a solution, while the other two were empirical studies. For instance, although \cite{guo_empirical_2019} did not propose a specific solution, Guo and colleagues not only identified several defects in DL software but also summarized practical guidelines and pointed out new research directions. These include understanding the characteristics of DL frameworks and platforms, avoiding compatibility and reliability issues, detecting DL software errors, and reducing the time cost and memory consumption of developing and deploying high-quality DL systems.

% For the "Inappropriate Threat Model" category, all 14 papers provided solutions or mitigations based on new methods or benchmarks, according to the literature. However, this doesn't mean that these papers didn't conduct empirical analyses. In fact, many of the proposed methods were based on findings and insights derived from large-scale research. For example, \cite{zhang_towards_2020} conducted extensive research to reveal the relationship between Adversarial Examples (AEs) and DL uncertainty. The study uncovered a series of overlooked uncertainty patterns, leading to the proposal of KuK (to Know the UnKnown), an automated testing technique for generating various types of rare AEs and Backdoor Examples (BEs) that existing techniques largely miss.

% As for the "DL library evolution" factor, there was only one related paper, which did not offer a solution but instead raised many challenges. However, this paper was published in 2019, so it is unclear whether this factor remains a pressing issue or if technological advancements have rendered it obsolete. In any case, we acknowledge the importance of this factor and call for more attention to it.


\begin{tcolorbox}[title=Summary - Deployment and Maintenance, left=2pt, right=2pt,top=2pt,bottom=2pt]
Based on 25 relevant studies, our literature review reveals three main pitfalls in deploying and maintaining LM4Code systems: real-world constraints, attack threats, and generated code containing security concerns.
These pitfalls can lead to untrustworthy results, copyright infringement, and reduced model efficacy.
Proposed solutions involve improving robustness through adversarial training and error detection, enhancing efficiency via compression and optimized inference, and protecting privacy and copyright through obfuscation and watermarking.
However, there remains a need for robust evaluation frameworks and techniques that balance security, efficiency, and accuracy. The implications highlight that real-world deployment introduces complex challenges for LM4Code systems.
\end{tcolorbox}

% \subsubsection{Discussion}
% Although researchers have proposed solutions for various issues, new challenges are continually emerging. In particular, for the "Deployment and Operation" stage, which has the lowest attention, it is clearly not possible that the pitfalls and biases of this stage have all been researched thoroughly, as countless unexplored challenges remain.

% Firstly, for the factor of "Lab-Only Evaluation," one idea is to understand the characteristics of DL frameworks and platforms to avoid compatibility and reliability issues, as suggested by Guo et al.\cite{guo_empirical_2019}. Zhang et al.\cite{zhang_empirical_2020} suggest three potential approaches: (1) improve platforms by providing a platform simulator for local development; (2) provide more comprehensive evaluation and analysis tools that take into account real-world environments; and (3) improve DL frameworks to mitigate or solve certain problems, such as automatic GPU memory management or using existing replay techniques to record precise execution sequences and interactions with the environment.

% Moreover, as the most attention-grabbing issue, "Inappropriate Threat Model" has numerous challenges awaiting solutions. For example, the application of uncommon data in robustness enhancement\cite{zhang_towards_2020}, developing effective and robust defense strategies\cite{li_textbugger_2019}, developing specific adversarial attacks against pre-trained models\cite{huang_robustness_2021}, defense mechanisms against adversarial sample attacks on Android and attack modifications to counter such defenses\cite{chen_android_2020}, and exploring robustness issues of machine learning models for various software engineering tasks\cite{zhou_adversarial_2022}.

% Lastly, regarding the issue of "DL library evolution," Nejadgholi et al.\cite{nejadgholi_study_2019} have indicated that future work would further reveal the various maintenance challenges developers may face when testing different components in DL libraries.





% \input{tables/factor_maintainance}
% \begin{figure}[t]
% \caption{Distribution of papers over years.}
%   \centering
%   \begin{minipage}{0.5\linewidth} 
%     \centering
%     \includegraphics[width=\linewidth]{images/maintainance/Distr-maintainance-factor-2.png}
%   \end{minipage}%
%   \begin{minipage}{0.5\linewidth} 
%     \centering
%     \includegraphics[width=\linewidth]{images/maintainance/Distr-maintainance-factor-1.png}
%   \end{minipage}
% \label{fig:Distr-maintainance-factor}
% \end{figure} 
% \subsubsection{Factors.} 
% In the preceding part, we categorized the factors into three classes: (1) Lab-Only Evaluation, (2) Inappropriate Threat Model, and (3) DL library evolution, with the first two classifications deriving from \cite{arp_dos_nodate}. Through our investigation, we collected 18 related papers out of a total of 140, as shown in Table \ref{tab:factor_maintainance}. Notably, this phase has the least number of related papers among the four stages, reflecting a relative lack of attention to the pitfalls and biases in this phase. Indeed, this stage represents a crucial juncture where model programs intersect with the real world, epitomizing the confluence of theory and practice. It serves as a decisive step in transforming successful scientific research into tangible benefits. Therefore, it is imperative to emphasize that the significance of this phase is closely intertwined with the interests of every researcher.

% As illustrated in Fig \ref{fig:Distr-maintainance-factor}, out of the 18 papers, three are related to Lab-Only Evaluation, 14 to Inappropriate Threat Model, and only one to DL library evolution. Analyzing this distribution, it is evident that the majority of researchers (78 percent) have focused on model attacks and defenses, whereas the other two categories have garnered just 17 percent and 5 percent of attention, respectively. Further examination reveals that among the 14 papers discussing Inappropriate Threat Model, 13 delve into adversarial sample attacks. This underscores researchers' pronounced concern for adversarial sample attacks and unveils the pressing challenges faced by LM models in this domain. Additionally, when looking at the annual distribution bar chart, it is apparent that the attention to Inappropriate Threat Model has been steadily growing year by year. In contrast, Lab-Only Evaluation has garnered a steady stream of attention with one paper each year from 2019 to 2021, albeit in small numbers, but has seen no publications in the past two years. As for DL library evolution, there has only been one paper on this topic in 2019, which serves as a stark reminder of the importance of addressing the pitfalls and biases inherent in DL library evolution. If left unattended, some LM-based works may only achieve fleeting success and lack longevity.

% Next, we will discuss each factor in detail, as follows:
% \begin{enumerate}
%     \item \textit{Lab-Only Evaluation.} After completing the training and testing evaluation stages in a laboratory environment, we may think our work is done. However, this is far from the truth. As a model-based software, it is meant to be deployed in the real world and evaluated in practice. As Zhang et al. pointed out \cite{zhang_empirical_2020}, differences between local and platform execution environments are a primary cause of failure in deep learning programs. These environments include two aspects: (1) one is the restrictions of software and hardware environment gaps. In the laboratory environment, researchers usually assume an ideal environment with controlled variables, but it's hard to guarantee such work won't face anomalies when confronted with the complex real world. Feng et al. \cite{feng_performance-sensitive_2021} noted that due to various performance limitations like computing power, memory size, and energy, original deep learning models can't be directly deployed and executed on mobile devices. (2) On the other hand, differences and changes exist between different operating environments. These disparities can be vast, as operating systems for PCs and mobile devices are entirely different, often leading to incompatibilities. As Guo et al. pointed out \cite{guo_empirical_2019}, trained models migrating/quantifying from PCs to real mobile devices and web browsers experienced significant differences in prediction accuracy and performance. Thus, evaluating solely in a lab environment reflects researchers' bias, leading to an overestimation of the actual impact of their work, which is also irresponsible.
%     In our opinion, the proper approach is to step away from ideal environments and instead embrace the scrutiny of real-world data. This shift could uncover more problems and yield greater insights.
%     %不同操作环境（如开发、测试和生产环境）之间可能存在差异或变化，这些差异可能导致软件应用程序，包括深度学习模型在部署和维护过程中的意外行为和挑战。
% %\cite{zhang_empirical_2020}本地和平台执行环境的差异、不恰当的模型参数/结构和框架API误解可能导致故障
% %\cite{guo_empirical_2019}针对部署过程，研究了当训练好的模型从PC迁移/量化到真实的移动设备和Web浏览器时的预测精度和性能(指时间成本和内存消耗)。DL平台的研究表明，迁移和量化仍然存在兼容性和可靠性问题
% %\cite{feng_performance-sensitive_2021}由于计算能力、内存大小和能量等各种性能限制，原始的深度学习模型无法直接在移动设备上部署和执行


%     \item \textit{Inappropriate Threat Model.} We all know that these model-based programs are ultimately meant to run in the real world, and in the real world, malicious attacks are inevitable and should be fully considered. If the security of the model is not considered, it will inevitably be exposed to a variety of attacks, such as adversarial sample attacks and backdoor attacks. Specifically, adversarial sample attacks have received the most attention from researchers. These attacks exploit the vulnerability of DNN models to adversarial samples\cite{zhou_adversarial_2022}\cite{henkel_semantic_2022}\cite{li_textbugger_2019}, which may exhibit unexpected behavior when dealing with unanticipated anomalies or adversarial inputs\cite{xiao_self-checking_2022}. Furthermore, this vulnerability is easy to exploit and hard to defend against. On one hand, there are numerous means of attack, such as effectively attacking NMT models by reversing semantics on the source code or directly using reference translations, or constructing adversarial samples by exploiting the structural vulnerabilities of programming language source code\cite{zhang_generating_2020}. What's more, most deep learning models in Android applications can be easily obtained through mature reverse engineering techniques\cite{huang_robustness_2021}. On the other hand, most of the defense mechanisms proposed to protect DNNs from adversarial sample attacks are ineffective\cite{wang_adversarial_2019}, as pointed out by Zhao et al.\cite{zhao_attack_2021}, adaptive attacks can easily bypass many defense mechanisms.
%     Additionally, deployed models are a black box, and it is impossible to know whether and how the model has been compromised\cite{li_deeppayload_2021}, which provides fertile ground for backdoor attacks.
% %\cite{zhou_adversarial_2022}DNN容易受到对抗样本的攻击
% %\cite{wang_adversarial_2019}大部分被提出的保护DNN免受对抗样本攻击的防御机制是无效的
% %\cite{chen_android_2020}机器学习模型缺乏对对抗样本的鲁棒性
% %\cite{zhao_attack_2021}尽管人们已经提出了各种防御机制来提高深度学习软件的鲁棒性，但其中许多防御机制对自适应攻击是无效的
% %\cite{zhang_challenging_2023}通过CloneGen来将特定代码转换和深度强化学习策略生成的对抗样本，使这些ML based的探测精度急剧下降
% %\cite{zhang_crafting_2021}通过在源代码上反转语义、直接使用参考译文均可以对NMT模型进行有效的攻击
% %\cite{zhang_generating_2020}程序设计语言源代码的结构化特性带来了新的挑战,即也容易被对抗性攻击所迷惑(与大多数自然语言不同，程序设计语言的源代码必须严格遵循严格的词汇、语法和句法约束)

% %\cite{huang_robustness_2021}Android应用中的大多数深度学习模型可以通过成熟的逆向工程轻松获得，而模型的曝光可能会招致对抗性攻击
% %\cite{henkel_semantic_2022}深度神经网络容易受到
% %\cite{zhang_towards_2020}尽管最近提出了一些测试、对抗攻击和防御技术，但仍然缺乏系统的研究来揭示AEs和DL不确定性之间的关系。
% %\cite{wan_you_2022}尽管在训练精确的代码搜索模型方面取得了实质性的进展，但这些模型的鲁棒性迄今为止很少受到关注。
% %\cite{xiao_self-checking_2022}DNN模型在处理非预期异常或对抗性输入时可能会表现出意想不到的行为
% %\cite{li_textbugger_2019}DLTU天生容易受到对抗性文本攻击，其中恶意构建的文本会触发目标DLTU系统和服务的不良行为。
% %\cite{zhang_towards_2022}稳健性作为一个重要的质量指标，仍然缺乏系统的考察，它要求模型在轻微扰动的代码输入下产生一致的决策
% %\cite{li_deeppayload_2021}与程序字节码的漏洞和威胁被广泛讨论不同，在应用程序中部署的深度学习模型是否以及如何被破坏并不清楚，因为神经网络通常被视为一个黑盒子。可以针对部署的DNN模型的Tive黑盒后门攻击

%     \item \textit{DL library evolution.} As time goes by, technology continues to develop and evolve, and nothing remains static. This is true for Deep Learning (DL) libraries as well, with their codes constantly evolving and updating\cite{nejadgholi_study_2019}. This relentless change and update pose a series of operational challenges for programs based on Language Models (LM). Even in the absence of external attacks, developers must continuously invest significant effort and time to adapt to the system's updates and iterations.
%     The constant evolution and change of DL libraries are a double-edged sword for developers. On one hand, they introduce numerous new features and capabilities, providing programs with greater power and flexibility. On the other hand, these changes also make code maintenance and management more complex and challenging. Each library update may lead to compatibility issues in the code, forcing developers to spend considerable time making adjustments and testing.
%     Simultaneously, the ongoing evolution of DL libraries also impacts the program's stability and performance. As new features and capabilities are continuously added, the program may become increasingly complex and bloated, requiring more computational resources and storage space. This demands that developers, while pursuing functionality, also focus on the program's efficiency and stability.
% %\cite{nejadgholi_study_2019}揭示了随着DL库中代码的演化(API的变化、修改Oracle近似、代码重构)，开发人员在维护oracle近似实践时可能面临的重要维护挑战
% \end{enumerate}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsubsection{Solutions.}
% \input{tables/solution_maintainance}

% As shown in Table \ref{tab:solution_maintainance}, we have examined whether the corresponding issues were addressed in the 18 articles we reviewed. Overall, 15 of the 18 articles presented solutions to the respective problems. 

% Specifically, for "Lab-Only Evaluation," we found that only one of the three papers offered a solution, while the other two were empirical studies. For instance, although \cite{guo_empirical_2019} did not propose a specific solution, Guo and colleagues not only identified several defects in DL software but also summarized practical guidelines and pointed out new research directions. These include understanding the characteristics of DL frameworks and platforms, avoiding compatibility and reliability issues, detecting DL software errors, and reducing the time cost and memory consumption of developing and deploying high-quality DL systems.

% For the "Inappropriate Threat Model" category, all 14 papers provided solutions or mitigations based on new methods or benchmarks, according to the literature. However, this doesn't mean that these papers didn't conduct empirical analyses. In fact, many of the proposed methods were based on findings and insights derived from large-scale research. For example, \cite{zhang_towards_2020} conducted extensive research to reveal the relationship between Adversarial Examples (AEs) and DL uncertainty. The study uncovered a series of overlooked uncertainty patterns, leading to the proposal of KuK (to Know the UnKnown), an automated testing technique for generating various types of rare AEs and Backdoor Examples (BEs) that existing techniques largely miss.

% As for the "DL library evolution" factor, there was only one related paper, which did not offer a solution but instead raised many challenges. However, this paper was published in 2019, so it is unclear whether this factor remains a pressing issue or if technological advancements have rendered it obsolete. In any case, we acknowledge the importance of this factor and call for more attention to it.
% \subsubsection{Challenges}
% Although researchers have proposed solutions for various issues, new challenges are continually emerging. In particular, for the "Deployment and Operation" stage, which has the lowest attention, it is clearly not possible that the pitfalls and biases of this stage have all been researched thoroughly, as countless unexplored challenges remain.

% Firstly, for the factor of "Lab-Only Evaluation," one idea is to understand the characteristics of DL frameworks and platforms to avoid compatibility and reliability issues, as suggested by Guo et al.\cite{guo_empirical_2019}. Zhang et al.\cite{zhang_empirical_2020} suggest three potential approaches: (1) improve platforms by providing a platform simulator for local development; (2) provide more comprehensive evaluation and analysis tools that take into account real-world environments; and (3) improve DL frameworks to mitigate or solve certain problems, such as automatic GPU memory management or using existing replay techniques to record precise execution sequences and interactions with the environment.

% Moreover, as the most attention-grabbing issue, "Inappropriate Threat Model" has numerous challenges awaiting solutions. For example, the application of uncommon data in robustness enhancement\cite{zhang_towards_2020}, developing effective and robust defense strategies\cite{li_textbugger_2019}, developing specific adversarial attacks against pre-trained models\cite{huang_robustness_2021}, defense mechanisms against adversarial sample attacks on Android and attack modifications to counter such defenses\cite{chen_android_2020}, and exploring robustness issues of machine learning models for various software engineering tasks\cite{zhou_adversarial_2022}.

% Lastly, regarding the issue of "DL library evolution," Nejadgholi et al.\cite{nejadgholi_study_2019} have indicated that future work would further reveal the various maintenance challenges developers may face when testing different components in DL libraries.



% %\begin{enumerate}
% %    \item \textit{Defense Mechanisms.}
% %\cite{wang_adversarial_2019}提出了一种在运行时检测对抗样本的替代方法
% %\cite{zhao_attack_2021}基于对抗样本的鲁棒性显著低于良性样本的观察，我们提出了一种新的特征来区分对抗样本和良性样本;提出了一种新的防御框架，即攻击防御( A2D )，通过有效地评估一个例子的鲁棒性来检测对抗性例子
% %\cite{xiao_self-checking_2022}SelfChecker + +，它的设计目标既包括非预期的异常测试数据，也包括预期的对抗样本.具体来说，开发了一种技术，可以将任何触发警报的运行时输入转换为语义等价的输入，然后将转换后的输入反馈到模型中。这样的运行时转换会使任何想要的精心设计的样本无效，从而使模型不受精心设计对抗样本的对抗攻击的影响。

% %    \item \textit{Attack Methods.}
% %\cite{zhou_adversarial_2022}提出ACCENT (对抗代码评论gENeraTor)，一种基于标识符替换的方法来生成对抗代码片段，这些代码片段在语法上正确，在语义上接近原始代码片段，但是可能会误导DNN产生完全不相关的代码注释。
% %\cite{chen_android_2020}介绍了一种新的攻击方法，该方法生成Android恶意软件的对抗样本，并避免被当前模型检测到。
% %\cite{zhang_challenging_2023}提出了一种基于深度强化学习的序列生成( DRLSG )策略来有效地指导生成能够逃脱检测的克隆的搜索过程
% %\cite{zhang_crafting_2021}提出了一种有前途的黑盒攻击方法，称为词显著性加速局部搜索( Word Saliency Speedup Local Search，WSLS )，可以有效地攻击主流的NMT架构。
% %\cite{li_deeppayload_2021}介绍了在编译好的深度学习模型上使用一组逆向工程技术实现的高度实用的后门攻击
% %\cite{zhang_generating_2020}提出了一种基于Metropolis - Hastings采样的标识符重命名技术，命名为Metropolis - Hastings Modifier ( MHM )，它为专门用于源代码处理的DL模型生成对抗样本
% %\cite{huang_robustness_2021}通过从TensorFlow Hub中识别高度相似的预训练模型，提出了一种简单但有效的利用对抗攻击对深度学习模型进行黑客入侵的方法
% %\cite{wan_you_2022}针对基于深度学习的代码搜索模型，通过数据中毒的方式，研究并开发了一系列的后门攻击
% %\cite{li_textbugger_2019}提出了一个生成对抗文本的通用攻击框架TEXTBUGGER。
% %\cite{zhang_towards_2022}提出了一种基于优化的攻击技术CARROTA来高效地生成有效的对抗源代码示例

% %    \item \textit{Proposing new technique.}
% %\cite{henkel_semantic_2022}提供了一种新颖的、通用的对手、用于训练源代码鲁棒模型的方法，以及一个已经(已经)允许其他人在代码模型领域推动对手边界的框架
% %\cite{feng_performance-sensitive_2021}提出了一个实用的解决方案( MobiTive )来检测移动设备上的Android恶意软件
% %\cite{qi_patching_2023}受软件工程中模块化和组合的基本概念的启发，提出了一种压缩的模块化方法CNNSplitter，它将用于N类分类的强CNN模型分解为N个较小的CNN模块,然后使用强模块对若模型进行组合补强

% %    \item \textit{Empirical study.}
% %\cite{nejadgholi_study_2019}研究了为测试四个流行的DL库而实现的oracle近似断言
% %\cite{zhang_empirical_2020}对深度学习作业的程序失败进行了全面的实证研究

% %\cite{guo_empirical_2019}总结了实用的指导方针，识别了挑战，并指出了新的研究方向，如了解DL框架和平台的特性，避免兼容性和可靠性问题，检测DL软件错误，以及减少开发和部署高质量DL系统的时间成本和内存消耗
% %\cite{zhang_towards_2020}进行了大规模的研究, 首先考察了多种不确定性度量在区分良性样本( BEs )和AEs方面的能力，从而能够刻画输入数据的不确定性模式。然后对BEs和AEs的不确定性模式进行了识别和分类，发现虽然现有方法生成的BEs和AEs确实遵循常见的不确定性模式，但其他一些不确定性模式在很大程度上被遗漏
% %\cite{ding_patching_2021}研究了将语言模型迁移到软件工程领域的常见例子“将软件修复比作语言翻译”，然而实证研究表明，序列到序列模型和翻译模型之间存在着微妙但关键的区别：程序修复在很大程度上受益于前者的通用建模架构，但在翻译准确性和多样性方面，它实际上受到后者内置的设计决策的影响

% %\end{enumerate}








% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %\textit{Poor Interpretability.}
% %\cite{cito_explaining_2021}由于这些模型的不透明性质以及输入数据的高维性，手动调试现代机器学习模型可能是一项极其艰巨的任务
% %\cite{fu_gpt2sp_2023}最近的工作提出了Deep - SE，一种基于深度学习的敏捷故事点估计方法，但它仍然是不准确的，不能迁移到其他项目，也不能解释
% %\cite{zou_interpreting_2021}由于深度学习模型的黑箱性质，很难解释为什么基于深度学习模型的预测器预测一段代码是脆弱的或不脆弱的
% %\cite{wan_what_2022}目前对于已有的预训练代码模型的可解释性研究仍然很少。目前尚不清楚这些模型的工作原理以及它们能够捕获哪些特征相关性
% %\cite{li_vulnerability_2021}尽管基于机器学习( ML )和深度学习( DL )的漏洞检测器( VD )取得了成功，但它们仅限于提供给定代码是否存在漏洞的决策，而没有提供代码中哪些部分与检测到的漏洞相关的详细信息。
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %solution
% %\cite{cito_explaining_2021}提出了一种模型不可知技术，用于寻找与错误预测高度相关的可解释规则
% %\cite{zou_interpreting_2021}引入了一个高保真度的解释框架，该框架旨在识别少量对检测器预测结果有重要贡献的令牌
% %\cite{wan_what_2022}进行了深入的结构分析，旨在从三个不同的角度为源代码(例如CodeBERT和GraphCodeBERT等)提供预训练语言模型的解释：( 1 )注意力分析，( 2 )词嵌入的探索，( 3 )语法树归纳
% %\cite{li_vulnerability_2021}提出了IVDetect，一个可解释的漏洞检测器，其思想是使用人工智能( Artificial Intelligence，AI )来检测漏洞，同时使用智能助手( Intelligence Assistant，IA )为易受攻击的语句提供VD解释



% %\textit{Inappropriate Model Parameter or Structure.} 
% %\cite{zhang_empirical_2018}与建模错误有关的错误，要么是由于学习率等模型参数不合适，要么是由于节点或层缺失等模型结构不正确。
% %\cite{tian_testing_2020}在流行的DNN图像分类器中，许多报告的错误案例发生的原因是训练的模型将一个类与另一个类混淆或对某些类的偏见超过了其他类, DNN模型中的缺陷是由于模型结构和训练数据之间的次优交互造成的
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %solution
% %\cite{zhang_empirical_2018}研究了构建在TensorFlow之上的深度学习应用，并从Stack Over ow问答页面和Github项目中收集了与TensorFlow相关的程序bug
% %\cite{tian_testing_2020}提出了一种基于类属性违反度的图像分类器鲁棒性测试方法





\section{Discussion}
\label{sec:Discussion}
\subsection{Recommendations for LM4Code Research}
Our systematic literature review reveals numerous pitfalls that can undermine the realistic performance and real-world effectiveness of LM4Code systems. 
These pitfalls span the data, models, evaluation, and deployment phases of the LM4Code lifecycle. 
LM4Code has become an increasingly prominent research area, evidenced by the rapid increase in publications. 
A prior survey by Hou~\ea~\cite{hou2023large} uncovered 229 papers on large language models for software engineering between 2020-2023, while Wang~\ea~\cite{wang_machinedeep_2023} uncovered 350 papers on deep learning for software engineering between 2015-2020. 
However, our focused study on LM4Code pitfalls only identified 67 relevant papers. 
This indicates that research attention to pitfalls in LM4Code is still insufficient, compared to the overall research volume.
Thus, future LM4Code research must not overlook the pitfalls when applying LM4Code models to software engineering tasks.


\noindent \textbf{\underline{Recognizing Existing Pitfalls.}}
In this study, we summarized multiple common pitfalls associated with LM4Code. 
These pitfalls,  each with distinct implications, highlight the inherent complexities in applying LM4Code to real-world software engineering problems. 
As our review results demonstrate, pitfalls can introduce unrealistic performance evaluation, compromise model efficacy, and raise security concerns. 
Thus, it becomes important for future LM4Code research to recognize and avoid potential pitfalls when building LM4Code systems for SE tasks.
To ensure trustworthy findings of LM4Code research, it is essential to demonstrate effectiveness through a rigorous and reliable experimental design that reflects real-world scenarios.
Furthermore, although our review has summarized common pitfalls, as previous surveys like Hou~\ea~\cite{hou2023large} present, there exist more than 50 specific large language models tailored to over 55 software engineering scenarios. 
So while we report general implications in some common settings using prevalent models, further investigation is required to discern more specific implications in specific or unconventional scenarios.


\noindent \textbf{\underline{Addressing Existing Pitfalls.}}
Addressing the identified pitfalls is vital for advancing robust and reliable LM4Code techniques.
As our study reveals, solutions like data cleaning, model explainability, optimized model design, and rigorous benchmarking have shown promise in mitigating certain pitfalls. 
However, these solutions, although effective in specific contexts, may not be universally applicable due to the complexity and ever-evolving nature of the software engineering landscape.
A coordinated effort by the community is required to establish guidelines and best practices that enable mitigating pitfalls in data construction, model design, performance evaluation, and deployment.


\noindent \textbf{\underline{Uncovering New Pitfalls.}}
The dynamic nature of the LM4Code field means novel pitfalls will likely emerge as techniques rapidly evolve. 
Specifically, the ever-evolving software engineering landscape, increasingly complex codebases, and new LM4Code techniques provide fertile ground for novel pitfalls to emerge.
Thus, identifying emerging pitfalls is critical.
The community needs to continuously analyze model reasoning, behaviors, and performance under realistic experimental settings to uncover new pitfalls in a timely manner. 
For example, testing on diverse unexplored situations or probing model decisions via XAI techniques yield valuable insights.
Through periodically updating benchmarks, refining evaluation approaches, and incorporating real-world deployment scenarios, we can ensure that we not only keep pace with the ever-evolving landscape, but also recognize and mitigate new challenges.

% By continually assessing models from multiple perspectives, the community can identify emerging pitfalls in a timely manner and initiate solutions early on.





% \subsubsection{Recommendations for Data Collection and Labeling.}.


% \textbf{Train-Test-Splite.} Although the separation of the dataset and test set should be a matter of course, this acknowledged standard can be violated either intentionally or unintentionally. Such a situation could lead to good performance during the testing phase, but a dramatic drop in performance when evaluated with real-world datasets. We do not discuss subjective cases, as they fall within the realm of academic ethics. Objectively, one possible explanation is the potential overlap among public datasets, as we can learn from Section~\ref{sec:data} that most of these datasets come from open-source platforms like GitHub. Hence, experiments on well-known datasets should be complemented by experiments on the latest data from the considered application domain, and duplication should be appropriately checked.

% \textbf{Unbalanced Distribution.} 
% %数据漂移、类分布
% The distribution of data often falls under the radar, yet this unseen issue can wield substantial impact. One prevalent instance is data drift, a phenomenon where data distribution is altered over time, a topic explored within Just-In-Time (JIT) related literature\cite{zeng_deep_2021,song_procedure_2023}. Another significant concern is unbalanced class distribution, a situation that emerges when an absence of proper randomization in sample selection leads to the underrepresentation or overrepresentation of certain populations. Consequently, for certain specialized tasks, researchers must give due consideration to the real-time nature and category distribution of data, ensuring its validity and relevance for meaningful analysis and conclusions.

% \textbf{Dataset protection.}
% %数据溯源、数据中毒、后门攻击、隐私泄露
% The issue of security within datasets should not be overlooked. In fact, many security issues stem from insufficient protection of datasets, such as problems related to data provenance, data poisoning, backdoor attacks, and privacy leakage, ~\ea. Especially for training data or non-public data, it is imperative to employ methods that ensure the reliability of data sources, such as watermarking for traceability or validation techniques to guarantee that the data has not been maliciously altered, poisoned, or embedded with backdoors. 

% \subsubsection{Recommendations for System Designing and Learning.}
% %利用好细粒度的信息，如语法、语义、结构、流信息、自然性，保证论证过程的逻辑和相关性，使用合适的LM
% %不要无脑使用LM，有些传统方法可以获得更好的效果，使用黑盒模型反而难以解释
% When utilizing LMs to enhance our research efforts, a common starting point is the automation of manual tasks. However, have we justified the suitability and relevance of the model for the specific task at hand? Have we strategically designed the fine-grained information to be leveraged?(including syntactical, semantical, structural, flow information, and ~\ea) Can we elucidate the fine-tuning process and causality? Does the employment of LMs indeed exhibit superior performance and cost-effectiveness compared to traditional techniques? These potential pitfalls should capture the attention of researchers. Addressing these questions can assist in clarifying, broadening perspectives, and significantly enhancing model performance, ensuring that the utilization of LMs in research is not only innovative but also robust and effective.

% \subsubsection{Recommendations for Performance evaluation.}
% %真实数据、环境评估测试，要选择合适的基准和指标测试
% In the end, models are destined for real-world application, underscoring our conviction that assessment using authentic data and environments stands as the most potent and persuasive method. Additionally, the selection of metrics demands a thoughtful consideration of practical factors to ensure the chosen evaluation metrics and benchmarks are both representative and feasible. This approach not only guarantees the applicability of the models but also bolsters the generality and transparency of the tests. Conducting experiments using real-world environments and data further enables the academic community to undertake reproducible experiments effortlessly, affirming the efficacy of the outcomes and reinforcing the credibility of the research.

% \subsubsection{Recommendations for Deployment and Maintenance.}
% %部署的时候需要考虑不同平台的兼容性和可移植性，也要考虑性能和cost的权衡，持续学习以及环境和库的迭代（考虑较长的时间跨度）
% In the stages of deploying and maintaining models, we believe it is imperative not to pursue high performance at the expense of other crucial metrics. The cost of the model stands as a significant criterion; expending substantial resources for a one-time high-performance result is a losing proposition. In addition, given the diverse software and hardware conditions across different platforms, researchers should undertake a comprehensive assessment based on the task's requirements. It is vital not to confine the model’s efficacy to the laboratory setting. Moreover, for models necessitating long-term sustenance, considerations should extend to the model's stability and sustained performance over extended periods, meeting the demands for sustainable learning and ensuring a certain degree of scalability.



% %\subsubsection{Recommendations for Security Issues}
% %注意安全问题（数据集隐私泄露、生成代码是否存在安全问题、模型是否容易被攻击）
% %LM4Code inherits the advantages of Language Models (LM), but it also takes on the drawbacks. Applying LM in the Software Engineering (SE) field is indeed a double-edged sword. If not handled adeptly, it may lead to grave security issues. In this study, we discuss three notable security threats: privacy leakage, attack threats, and security concerns in generated code, each within different stages of the software engineering lifecycle.








\subsection{Open Challenges and Research Directions}
\subsubsection{Improving Data Quality for LM4Code}
The processes of data collection and labeling play critical roles in the model construction, determining their efficiency, trustworthiness, and overall performance~\cite{lo2023trustworthy}.
With the emergence of large language models such as GPT-4~\cite{openai2023gpt4}, the reliance on massive data has increased significantly. 
However, as we have reviewed, there are numerous obstacles and unanswered questions associated with these phases. 

\noindent \textbf{\underline{Volume vs. Quality.}}
The increasing number and widespread use of large language models such as GPT-4,  underscore the inherent conflict between the quantity and quality of data.
These models, with their vast number of parameters, heavily rely on extensive datasets to achieve their remarkable performance.
For example, Codex~\cite{chen2021evaluating}, which is a variant of the GPT-3.5 framework introduced in 2021, conducted training using a dataset that was sourced from 54 million publicly available software repositories on the GitHub platform, resulting in a total data size of 159 GB.
Yet, collecting vast amounts of data, a process that is both time-consuming and labor-intensive, is not a "silver bullet"; data quality is also important.
Even with advanced large models, "garbage in - garbage out"~\cite{liu2023refining, pearce_asleep_2022}.
Notably, even widely-used benchmark datasets like CodeSearchNet~\cite{husain2019codesearchnet} have been observed to contain considerable noise and errors, as highlighted in prior research~\cite{sun_importance_2022,shi2022we}.
Over-reliance on volume can lead to models that are prone to biases, noise, and even adversarial attacks. 
On the contrary, an excessive focus on data quality can inadvertently decrease the diversity and richness of the dataset. 
Finding the ideal compromise between these conflicting requirements offers an appealing opportunity for future investigation.

\noindent \textbf{\underline{Automated Data Quality Assurance.}}
As the implications of low-quality data, it is essential to utilize high-quality datasets to develop LM4Code approaches.
In the dynamic evolution environment of software and language models, manually searching and examining extensive datasets for data noise or errors is neither practical and efficient.
As a result, there is an urgent need for automated tools and frameworks that can assure and maintain data trustworthiness and quality, particularly for LM4Code models.
We can systematically discover and correct data noise, labeling errors, and other anomalies, allowing models to train on robust and reliable datasets and ensuring their reliability and efficiency in real-world applications.



\subsubsection{Strengthening Robustness and Trustworthiness in LM4Code}
LM4Code models are becoming increasingly integrated into the software development lifecycle, influencing everything from code generation to vulnerability detection. 
Ensuring that these models are robust and trustworthy is essential. This does not just relate to their prediction accuracy but extends to the reliability, interpretability, and generalization capacity of the model, especially in diverse and evolving coding environments~\cite{niu2023crosscodebench,wang2022machine}.

\noindent \textbf{\underline{Building Interpretable LM4Code.}}
The black-box nature of language models has been a long-term concern, especially when LM4Code applications directly influence software development outcomes~\cite{wang2022machine, watson2022systematic,10109341, 10109328}. 
Transparency in LM4Code requires an in-depth examination of the correlations and reasoning processes that models depend on, instead of just knowing the model's predictions. 
Our review results show that pitfalls can exist throughout the entire LM4Code lifecycle, potentially resulting in spurious correlations.
These misleading correlations are based on wrong artifacts for generating predictions, presenting significant challenges for practical real-world applications.
Although prior studies~\cite{cito_explaining_2021, shi2023towards, wan_what_2022, zou_interpreting_2021} have introduced various explainable AI (XAI) techniques into LM4Code, the current solutions lag behind the rapid evolution of language models~\cite{zini2022explainability, madsen2022post}.
Existing XAI techniques for LMs, in particular, only provide explanations as either the contribution of individual words to the decision or the layer/neuron at which syntax or semantics are encoded~\cite{zini2022explainability}.
Although helpful, these explanations only offer a fragmented picture of the model's decision-making process, ignoring a considerable amount of its intricate reasoning.
As the complexity of language models grows, there is an imperative need to develop more comprehensive and accessible XAI approaches for LM4Code.


\noindent \textbf{\underline{Improving Robustness Against Errors and Threats.}}
Recent literature~\cite{niu2023codexleaks, sun2022coprotector, peng2022security} reveals that state-of-the-art LM4Code models like Codex~\cite{chen2021evaluating}, GPT-3, and Starcoder~\cite{li2023starcoder} are susceptible to inadvertent data errors and malicious threats. 
Such pitfalls not only degrade model performance, but raise concerns about the security and trustworthiness of LM4Code systems.
Improving model robustness is therefore an urgent need to enable reliable LM4Code adoption.
While prior studies~\cite{sun_importance_2022, sun2022coprotector, sun2023backdooring, zhang_towards_2022} have proven that techniques like adversarial training and data augmentation can enhance robustness, more efforts should be spent by our research community to holistically defend against newly emerging issues and threats. 
Specifically, possible solutions like domain-specific preprocessing and learning, continuous evaluation, hybrid models, and anomaly detection should be explored. 
Overall, a multilayered defense-in-depth strategy is essential to ensure LM4Code reliability and trustworthiness against growing pitfalls or issues.

% As LM4Code models currently permeate various software development steps, they need to be resilient enough to both inadvertent errors and malicious threats. 
% Recent literature~\cite{niu2023codexleaks, sun2022coprotector, peng2022security} has revealed pitfalls of even state-of-the-art models such as Codex, GPT-3, and Starcoder~\cite{li2023starcoder} to data errors, adversarial attacks, and privacy leaks.
% Such pitfalls could not only degrade model performance, but raise concerns about security and trustworthiness in LM4Code systems.
% To enable the safe and ethical deployment of LM4Code, advancing their robustness is an urgent need. 
% Therefore, enhancing the robustness of LM4Code models against data problems and external threats becomes essential, requiring future research efforts and novel methodologies to address these challenges.

\noindent \textbf{\underline{Adapting to Ever-evolving Code Environments.}}
Within the ever-evolving field of software development, new programming languages emerge, old ones get updated, and coding techniques and habits are constantly transforming.
Against this backdrop,  a primary challenge for LM4Code is ensuring the broad applicability and robust generalizability of LM4Code systems.
Prior studies~\cite{nong_generating_2022, thongtanunam_autotransform_2022, rabin2021generalizability, wang2022machine} have highlighted the superior generalizability of advanced LMs over traditional ML/DL techniques,  particularly when it comes to previously unseen distributions.
However, there remain significant research gaps. 
Specifically, while the improvements in models like the advanced Transformer are promising, they may not always translate to practical efficiency. 
For instance, Thongtanunam~\ea~\cite{thongtanunam_autotransform_2022} indicates that while the Transformer demonstrates an improvement of 490\% to 567\% on new tokens, its accuracy remains around 10\%, indicating a significant room for improvement.
Thus, the incorporation of domain-specific knowledge, continuous model updating, and feedback loops with developers could pave the way for more adaptable and reliable LM4Code solutions in an ever-evolving coding landscape.

\subsubsection{Towards Reliable Performance Evaluation of LM4Code}
Performance evaluation plays a key role in demonstrating the efficiency and capability of the proposed LM4Code approaches.
However, as discussed in Section~\ref{sec:performance_evaluation}, there are several pitfalls that can undermine realistic performance, including inappropriate baselines, inappropriate test sets, reproducibility issues, and inappropriate performance measures.
Therefore, it is important to focus future research efforts on solid benchmarks and rigorous evaluation methodology. 

\noindent \textbf{\underline{Towards Reliable and Standardized Benchmarks.}}
It is important to establish a rigorous evaluation methodology supported by trustworthy and standardized benchmarks.
These benchmarks provide consistent frameworks for comparing different LM4Code approaches and set baselines for new techniques~\cite{beyer2019reliable}.
However, our review results reveal that multiple pitfalls related to performance evaluation like inappropriate baselines, limited test sets, and reproducibility issues distort understanding of actual LM4Code capabilities, questioning research correctness~\cite{liu2023towards, zeng_extensive_2022, liu_deep_2022}. 
For example, Laaber~\ea~\cite{laaber2021predicting} emphasize the inherent benchmark instability, stressing the importance of identifying and rectifying these instabilities to ensure accurate evaluations. 
Without addressing pitfalls, perceived model performance can become inflated, leading to potentially misleading conclusions. 
Related benchmarking challenges have been noted across various research domains like computer security~\cite{van2019sok}, and cloud computing~\cite{schwarzkopf2012seven, cooper2010benchmarking}.
Hence, there is an urgent need to prioritize the development of standardized, stable, and reliable benchmarks in LM4Code research. 
Future research should focus on creating benchmarks that are both comprehensive and representative of real-world scenarios.
To achieve this, the community should coordinate on curating representative test sets, establishing strong baselines, quantifying uncertainty, and promoting reproducible experiments, 
ensuring that advancements in the field of LM4Code are grounded in robust and reliable evaluations. 
This will not only foster trustworthiness within the research community but also drive meaningful progress in LM4Code.

\noindent \textbf{\underline{Towards Reliable Evaluation Metrics.}}
As language models like GPT-4 grow in complexity, accurately assessing their capabilities and limitations becomes imperative.
However, as discussed, traditional evaluation metrics, often borrowed from the NLP domain, may fail to capture the intricacies and details that are crucial for code generation and understanding tasks~\cite{scalabrino2017automatically, ren2020codebleu}.
For example, metrics like accuracy and BLEU focusing solely on syntactic correctness fail to account for potential semantic errors with practical consequences, as noted by Fan~\ea~\cite{fan2023automated}. 
In addition, most studies rely heavily on automated metrics, but human evaluation remains indispensable for assessing the quality and utility of generated code~\cite{dakhel2023github,paltenghi_thinking_2021}.
Additionally, the variability and uncertainty inherent in generative models like GPT-4 need to be measured and analyzed in order to understand reliability in real-world settings~\cite{openai2023gpt4}.
Therefore, developing holistic and standardized metrics tailored to code intelligence tasks is urgently needed. 
These should measure syntactic validity, semantic consistency, coherence, human quality judgments, and variability.
For LM4Code to move from impressing lab-only evaluation to transforming real-world applications, reliable evaluation metrics are crucial.

% Such metrics can better align lab measurements with practical utility, bridging the gap between existing NLP techniques and the unique requirements of code intelligence.
% Reliable evaluation is vital for transitioning impressively performing models in controlled settings into transformative real-world applications.


\subsubsection{Optimizing LM4Code Deployment for Real-World Scenarios}
Realizing LM4Code's potential requires addressing deployment challenges in transitioning from controlled research to practice. 
The integration, security, and scalability of LM4Code techniques become important considerations.

\noindent \textbf{\underline{Integrating LM4Code into Developer Workflows and Tools.}}
While modern LM4Code models like GitHub Copilot show potential for integrating AI-driven code suggestions into developers' workflows, realizing this in practice presents unique challenges.
First, it is crucial to ensure the correctness and human comprehensibility of suggestions, especially since the generated code can contain errors and vulnerabilities that may be problematic for real-world usage~\cite{nguyen2022empirical,peng2022security, pearce_asleep_2022}.
Additionally, customization and personalization are also important, since every developer has a unique coding style and preferences.
Modern LM4Code tools should be adaptable and learn from individual developer behaviors to provide personalized code suggestions.
Finally, integration with developer tools like version control and debugging is critical for comprehensive functionality. 
Future research should focus on addressing these challenges, ensuring that the integration of LM4Code models into developer workflows is smooth, efficient, and beneficial.



\noindent \textbf{\underline{Towards LM4Code Security.}}
As discussed in Section~\ref{sec:deployment}, LM4Code faces several security concerns that need to be addressed before responsible and ethical deployment can be achieved. 
These include risks of evasion attacks, data poisoning, privacy leakage, and generated code potentially containing vulnerabilities. 
Implementing comprehensive solutions is thus critical to safeguard models, data, and users.
Advancing the security of LM4Code requires continued research across multiple domains:
(1) Adversarial training techniques~\cite{zhou_adversarial_2022} can potentially increase model robustness against adversarial inputs; 
(2) Employing formal verification approaches to evaluate the security and correctness of generated code~\cite{pearce_asleep_2022}; 
(3) Enhanced data construction and quality assurance processes are needed to systematically identify and eliminate data poisoning, preventing the propagation of risks~\cite{schuster2021you};
(4) Approaches such as differential privacy~\cite{lukas2023analyzing} and federated learning~\cite{li2020federated} may strengthen privacy preservation in model training;
(5) Watermarking and provenance tracking mechanisms can enable authentication of model ownership and detect plagiarism or unauthorized use~\cite{kirchenbauer2023watermark, sun2022coprotector};
(6) Manual examination approaches including code reviews and human-AI collaborative interactions are important.
Substantial multidisciplinary efforts are critical to ensure the secure and ethical development and deployment of powerful generative AI systems like LM4Code. 
This remains an open research challenge requiring continued progress across communities.


\noindent \textbf{\underline{Scalability and Latency Concerns.}}
While powerful general large language models like GPT-4~\cite{openai2023gpt4}, PaLM~\cite{google2023palm}, and Claude~\cite{anthropic2023claude} offer public API access, privately deployed specialized LM4Code models can face greater scalability challenges.
Developing private models is important to customize LM4Code systems to specific domains and tasks. 
However, large language models often comprise billions of parameters, requiring massive computational resources~\cite{hou2023large}.
This poses challenges for real-time efficient integration into developer workflows. 
Reducing inference latency through methods like knowledge distillation~\cite{shi2022compressing} and efficient attention~\cite{kaddour2023challenges} is crucial for reasonable responsiveness.
Additionally, scaling up throughput for concurrent users via cloud-native architectures is also essential. 
Optimizing memory utilization via compression and caching helps in deploying large LM4Code models~\cite{shi2022compressing}. 
Energy-efficient deployment through quantization and lightweight model distillation is likewise critical~\cite{guo2019empirical}.
Tackling these scalability and latency issues will be critical to realize LM4Code's full potential through deployments that smoothly integrate LM4Code into practical developer environments in a sustainable and user-friendly manner.



% \subsubsection{Generalization VS Specialization.}
% Model generalization and specialization have consistently been critical and challenging topics of LM research. 
% Proposing an almighty model which rules all the tasks with current pre-training objectives is challenging or even impractical\cite{zeng_extensive_2022}, for the reason that LMs deeply relies on the knowledge of training data. When facing environment or specific tasks out of the scoop, or even using unseen tokens and identifiers, the performance of the LM decreases sharply\cite{yang2022natural}.
% As shown in Table~\ref{tab:bias_in_evaluation}, we present the related challenges in collected papers, such as OOV(out-of-vocabulary)\cite{meng2023template}, structure difference in programming language\cite{lin2022xcode}, training multiple models for multiple downstream tasks\cite{fang2023representthemall}. Enhancing the generalizability of a model poses a significant challenge, particularly because the broader the problem scope, the more multifaceted the viewpoints that must be contemplated. This necessitates a comprehensive consideration of various layers of information, ranging from syntax and semantics to data structures and natural language nuances, et al.
% More surprisingly, some state-of-the-art works intentionally compromises performance solely for the sake of achieving multi-task capabilities\cite{zeng_extensive_2022}, which suggests that the multi-task capabilities of models are increasingly gaining the attentions and need.
% However, a more prevalent idea is to delve deeply into a specific task and utilize domain knowledge to train the model to be more focused on a particular task, and we have presented 22 kind of the SE tasks in Table~\ref{tab:SE_tasks}.
% For instance, Feng et al  highlight that adversarial attacks on deep learning-based malware are far more domain-specific compared to conventional image or voice classification problems. They also note that these challenges come with their own set of advantages and weaknesses, necessitating specialized research\cite{feng_performance-sensitive_2021}. 

% Striking a Balance Between Generalization and Specialization. Breadth and depth are two sides of the same coin when it comes to addressing real-world issues. The advancement of language models and the emergence of LLMs offer us a unique opportunity to explore this balance. We believe this constitutes a compelling avenue for future research.







% \subsubsection{Explainability and Trustworthy of LM4Code.}
% %从统计模型到LM再到LLM，模型变得越来越复杂，我们也越来越难以直观地理解模型背后庞大的参数所代表的数学逻辑。自然而然，人们希望提出一种可解释性方案来分析和解释各种各样的模型。
% %在我们收集的5篇XAI相关的文献中，attention-based方法有三篇，它们在经验直觉和相关性证明\cite{paltenghi_thinking_2021}、attention can capture high-level structural properties\cite{wan_what_2022}、模型性能与成本\cite{zhang_diet_2022}三个方面都给出了解答。
% %另外两篇都是漏洞检测任务相关的。\cite{zou_interpreting_2021}提出了一个高保真的模型无关的漏洞检测器的预测框架，该框架使用重要的标记来提取一些领域专家可以理解的决策树规则，从而解释为什么将特定示例预测为特定标签（即易受攻击或不易受攻击）。\cite{li_vulnerability_2021}则从使用AI基于数据和控制依赖关系来对漏洞进行定位和解释。
% %然而，这些方案所关注的软件工程任务过于狭窄，集中于code summarization, and clone detection。事实上，更多的软工任务都在与LM产生联系，我们对于模型的可解释需要一种普适性的框架或者方法，在整个SE领域达成一个公认的、可信的、可执行的模型可解释性框架，进而实现可协同的AI4Code\cite{lo2023trustworthy}，这将是a transition towards Software Engineering 2.0。

% From statistical models to LMs and onto LLMs, models have become increasingly complex. As a result, understanding the mathematical logic behind the vast number of parameters has become less intuitive. Naturally, there's a growing need for an explainability approach to analyze and interpret these models.
% In the 5 XAI-related literature we've collected, 3 are attention-based. They address empirical intuition and correlation proof\cite{paltenghi_thinking_2021}, the capability of attention to capture high-level structural properties\cite{wan_what_2022}, and the trade-off between model performance and cost\cite{zhang_diet_2022}.
% The other 2 focus on vulnerability detection tasks. \cite{zou_interpreting_2021} presents a model-agnostic framework for vulnerability detection that uses salient tokens to derive decision-tree rules understandable by domain experts, explaining the classification of specific samples. \cite{li_vulnerability_2021} delves into the use of AI based on data and control dependencies for vulnerability localization and explanation.

% However, the software engineering tasks these schemes address are rather limited, primarily focusing on code summarization and clone detection. As more software engineering tasks intertwine with LMs, there's an imperative for a universally applicable framework or method. The aim is to establish a widely-accepted, credible, and implementable model explainability framework, fostering collaborative AI4Code\cite{lo2023trustworthy}. This direction points towards a transition to Software Engineering 2.0.

%\subsubsection{Testing and Evaluation.}
% In applying Language Models (LM) to code generation and other code-related tasks, the real advancements and breakthroughs of the models often hinge on the benchmarks and evaluation methods we employ. As such, establishing more robust benchmarks and rigorous evaluations becomes paramount.
% A refined evaluation framework involves not just selecting the right evaluation metrics but, more crucially, choosing those that genuinely reflect a model's performance in real-world scenarios. Such metrics can deeply capture the strengths and weaknesses of a model, providing clear direction for researchers.
% Simultaneously, there's an existing challenge of potential discrepancies between standard benchmark datasets and actual application contexts. Given this, considering the construction of diverse datasets from real-world development environments becomes essential, encompassing various programming languages, coding styles, and projects of different complexities.
% With the evolution of LMs, some of the existing benchmarks might start to lose their challenging edge. Thus, regularly updating these benchmarks to ensure models consistently face new challenges is indispensable.
% Furthermore, transparency and innovation in research are crucial. Researchers need to provide thorough experimental details, ensuring that others can easily replicate and further advance their work, fostering collective progress within the research community.
%In the field of deep learning, testing and evaluating the performance and robustness of models remains a persistent challenge, especially in coding and software engineering tasks. For instance, in an end-to-end system, a comprehensive system requires the integration of defect localization and the enhancement of evaluation for testing devices. In certain applications, such as Java vulnerability repair tools, the limited number of evaluation benchmarks further complicates the evaluation process. Furthermore, the unique challenges language models face when handling code make testing their robustness in natural code distributions even more challenging. Particularly, for tasks like program translation, the evaluation of semantic correctness becomes especially critical and challenging. Moreover, a significant obstacle currently facing the robustness benchmark testing for generative tasks is that the evaluation of text generation is often subjective and difficult to quantify. However, it's worth noting that while traditional metrics like accuracy, recall, or F1 score have their value in many contexts, they may not fully capture a model's overall performance or impact. In fact, some literature has even expressed skepticism about metrics like coverage. In summary, the effective testing and evaluation of deep learning models remain an unresolved issue, demanding more research and exploration.

% \subsubsection{Leveraging and Enhancing LLM Performance.}
% In the current research landscape, LLMs like GPT-4 have demonstrated their formidable capabilities across various tasks. As Pearce pointed out in his 2023 study, while LLMs have limitations in certain applications, such as only being able to fix specific locations in a single file, he also emphasized the vast potential and room for optimization in these models\cite{pearce_examining_2023}. To elevate the performance of LLMs, we can explore the following avenues:

% \textbf{Collective Intelligence (CI).} 
% CI is an emerging trend, which illustrates that collective wisdom usually surpass individual intelligence\cite{zhang_merit_2022}.
% By integrating knowledge from multiple models or sources, LLMs can learn and optimize from various perspectives. For example, combining code repositories and feedback from the developer community can provide richer training data for LLMs. CI also illustrate that the cooperation and knowledge merging among isolated software developers is essential for program synthesis.

% \textbf{Model Automatic Fine-tuning.} 
% Adjusting the LLM for specific coding tasks or datasets can further enhance the model's performance in certain scenarios and make it more adaptable to those environments. However, it is undeniable that the number of parameters in LLMs is exceptionally large, making manual tuning a labor-intensive task, not to mention the potential errors that can arise from manual adjustments. Therefore, there is an urgent need for standardized, automated tuning methods to assist or even replace manual efforts, aiming to improve efficiency and accuracy. Thus, automated parameter tuning undoubtedly presents an opportunity for future research.

% \textbf{Self-Evolution of LLM.}
% LM, or even LLM, as models with the ability to learn, pose the question: can they continuously learn and improve themselves just like humans? In the 68 papers we have collected, topics such as continuous learning\cite{}, catastrophic forgetting\cite{gao2023keeping}, and future token\cite{thongtanunam_autotransform_2022}s are mentioned. However, these papers do not take into account the update and replacement of Deep Learning (DL) libraries\cite{guo_empirical_2019}, such as automatic updates of library functions, and related ethical issues.

% While LLMs have achieved notable successes across various domains, further research and optimization are still required to realize their maximum potential in the coding sector. By integrating existing methods with new strategies, we can anticipate a more potent and reliable LLM in the future.

%\subsubsection{Model Design and Optimization.}
%With the widespread application of deep learning in code and software engineering, the design and optimization of models face many inherent challenges. Firstly, proposing outstanding universal models for various program understanding and generation tasks is not straightforward and can sometimes even be regressive. For instance, some cutting-edge encoder-decoder models might perform worse in certain tasks compared to pure encoder models. Moreover, current pre-training objectives, such as Masked Language Modeling and autoregressive loss, make it challenging to develop a jack-of-all-trades model suitable for all tasks. In reality, finding a general pre-trained model that possesses both program understanding and generation capabilities is particularly difficult. Furthermore, the opacity and interpretability of models are also core issues, making fine-tuning and optimization of the models even more intricate. For example, in code completion research, correctly suggesting identifiers is especially challenging since it requires a profound understanding of the program. In some domains, such as robust optimization, addressing these goals within the realm of source code is especially challenging. All in all, the design and optimization of models necessitate in-depth research and innovation to meet the growing demands.
% \subsubsection{Modular and Mobile-Ready Models for LM4Code}
% With the advancement of technology, LM4Code is confronted with new challenges of adapting across various computational devices. Devices like smartphones, tablets, and edge computing hardware, though constrained by hardware and computational capacities, offer broader deployment opportunities for the model. Running the model directly on these devices enhances response time by eliminating network latency and offers an added layer of data privacy. Executing processes directly on user devices prevents the need to transmit user data to external servers, mitigating risks of data breaches\cite{feng_performance-sensitive_2021}.
% Model simplification\cite{zhang_diet_2022}, modularity\cite{qi_patching_2023} and reusability\cite{pan_decomposing_2022} are pivotal for such multi-platform deployment. They not only lower computational and storage requirements but also allow developers to cherry-pick specific parts of the model based on the application's demands.
% To truly harness the opportunities of cross-platform deployment, there's a need for research and development of effective model migration strategies, ensuring that LM4Code models don't suffer significant performance degradation when transitioning from one platform to another. As these techniques continue to innovate and optimize, we anticipate a widespread application of LM4Code across diverse devices, opening new avenues for applications and commercial opportunities.

% \subsubsection{Data-related Issues.}%%
% In the training and evaluation of deep learning models, data has always been a pivotal component, but it also introduces a myriad of challenges. 

% \textbf{Data processing.}

% In Table~\ref{tab:bias_in_data_collection} and Table~\ref{tab:bias_in_model}, we have studied the biases in sampling and data snooping, however, the data processing procedure has not been investigated yet.  xxxxxx%data duplication\cite{chakraborty2021deep}, 有效特征的处理、特征积累&性能与开销\cite{feng_performance-sensitive_2021}, source code’s vocabulary characteristics are very different from natural languages\cite{hellendoorn_when_2019}, non-robust issue of DL for source code processing.\cite{zhang_towards_2022}

% \textbf{In need of high-quality dataset.}
% While standard deep learning tasks often have high-quality training datasets available, collecting large-scale, high-quality datasets for software engineering tasks proves to be a major challenge\cite{li2022robust}. This further amplifies the difficulty in model training and generalization.

% In summary, the selection, processing, and augmentation of data are indispensable elements in model design and evaluation and require continuous research and innovation to address these inherent challenges.


%data processing
%In the training and evaluation of deep learning models, data has always been a pivotal component, but it also introduces a myriad of challenges. For instance, for newly emerged malware families, if their malicious behaviors cannot be represented by the chosen feature types, certain detection methods might fail to identify them. This implies that we need to constantly introduce new effective features to the models, ensuring they don't bring substantial performance overhead at the same time. Additionally, while standard deep learning tasks often have high-quality training datasets available, such as ImageNet, collecting large-scale, high-quality datasets for software engineering tasks proves to be a major challenge. This further amplifies the difficulty in model training and generalization. Notably, when it comes to tasks like code generation, a complete understanding of natural language by the computer becomes particularly crucial as it may determine whether the model can accurately interpret requirements articulated in English. Furthermore, given the lexical (innovative) characteristics of source code differ greatly from natural language, integrating new vocabulary becomes a complex issue. In summary, the selection, processing, and augmentation of data are indispensable elements in model design and evaluation and require continuous research and innovation to address these inherent challenges.

%\subsubsection{Task-specific Issues.}%合并到Generalization VS Specialization
%In the realm of deep learning applications, the uniqueness of specific tasks often introduces a set of distinct challenges. For instance, in few-shot learning, due to the constraints of available data, models frequently face the risk of overfitting, resulting in compromised generalization performance in real-world applications. This has prompted researchers to explore alternative approaches, such as meta-learning or pre-trained models, to leverage previously acquired knowledge. For reinforcement learning, given its real-time interaction with the environment, achieving stable and efficient learning becomes a significant hurdle. Especially when dealing with complex and ever-changing environments, ensuring continuous policy optimization and adaptability is at the forefront of research. Additionally, for generative tasks like text and image generation, ensuring the consistency, authenticity, and diversity of outputs remains a long-standing issue. These task-specific challenges underscore the versatility of deep learning across various domains and drive the exploration of algorithms and techniques tailored to specific scenarios and needs.

%\subsection{Opportunities}

%应用LLM，LLM可以用，但是存在想只能修复单个文件的单个位置的漏洞问题，价值有待挖掘 \cite{pearce_examining_2023}
%构建LLM的可信框架
%集体智慧CI
%LLM可解释性方案XAI
%Boosting LLM Performance
%\subsubsection{Leveraging and Enhancing LLM Performance.}
%In the current research landscape, Large Language Models (LLM) like GPT-4 have demonstrated their formidable capabilities across various tasks. As Pearce pointed out in his 2023 study, while LLMs have limitations in certain applications, such as only being able to fix specific locations in a single file, he also emphasized the vast potential and room for optimization in these models\cite{pearce_examining_2023}. To elevate the performance of LLMs, we can explore the following avenues:

%\textbf{Constructing a Trustworthy Framework for LLM.} By establishing a reliable framework, it can be ensured that the outputs of LLMs are accurate and dependable in specific contexts. For instance, by using validation and test sets, we can ensure that the LLM performs as expected in code-related tasks.

%\textbf{Collective Intelligence (CI).} By integrating knowledge from multiple models or sources, LLMs can learn and optimize from various perspectives. For example, combining code repositories and feedback from the developer community can provide richer training data for LLMs.

%\textbf{Explainable Artificial Intelligence(XAI).} Offering interpretable outputs from the model can help developers better understand and trust the model's decisions. Moreover, when errors arise, these explanatory outputs can aid developers in quickly identifying and rectifying issues.

%\textbf{Model Fine-tuning and Adaptability.} Adjusting the LLM for specific coding tasks or datasets can further enhance the model's performance in certain scenarios. For example, training the model specifically for certain programming languages or frameworks can make it more adaptable to those environments.

%In conclusion, while LLMs have achieved notable successes across various domains, further research and optimization are still required to realize their maximum potential in the coding sector. By integrating existing methods with new strategies, we can anticipate a more potent and reliable LLM in the future.
%More Solid Benchmarks and Rigorous Evaluations
%更好的评估框架
%更好的数据集和真实世界测试集、benchmark
%可重复性
%\subsubsection{Strengthening Evaluation Metrics.}
%In applying Language Models (LM) to code generation and other code-related tasks, the real advancements and breakthroughs of the models often hinge on the benchmarks and evaluation methods we employ. As such, establishing more robust benchmarks and rigorous evaluations becomes paramount.
%A refined evaluation framework involves not just selecting the right evaluation metrics but, more crucially, choosing those that genuinely reflect a model's performance in real-world scenarios. Such metrics can deeply capture the strengths and weaknesses of a model, providing clear direction for researchers.
%Simultaneously, there's an existing challenge of potential discrepancies between standard benchmark datasets and actual application contexts. Given this, considering the construction of diverse datasets from real-world development environments becomes essential, encompassing various programming languages, coding styles, and projects of different complexities.
%With the evolution of LMs, some of the existing benchmarks might start to lose their challenging edge. Thus, regularly updating these benchmarks to ensure models consistently face new challenges is indispensable.
%Furthermore, transparency and innovation in research are crucial. Researchers need to provide thorough experimental details, ensuring that others can easily replicate and further advance their work, fostering collective progress within the research community.

%泛化：跨功能、跨语言、跨项目、交叉
%针对特定领域的模型performance更好，领域知识
%\subsubsection{Broadening Generalization and Harnessing Domain-Specific Expertise.}
%The vast and dynamic realm of coding presents multifaceted challenges and opportunities for Language Models tailored for code (LM4CODE). As the field progresses, the emphasis on generalization becomes even more prominent. The vision is not merely to have models that work on a single-function, single-language, or single-project basis but to transcend these boundaries.
%A truly versatile LM4Code should be adept at handling tasks across functions, bridging gaps between languages, seamlessly transitioning between projects, and showcasing adaptability in cross-domain scenarios. Such robust generalization capabilities would eliminate the need for developers to switch between multiple tools and models, offering a more streamlined and efficient coding experience.
%However, as we strive for wider generalization, the importance of domain-specific expertise cannot be sidelined. Models fine-tuned to a particular domain often outshine their generic counterparts, primarily due to their innate capability to harness domain knowledge. This understanding, deeply ingrained within specialized models, allows them to make more contextually accurate suggestions, predictions, or fixes that resonate with domain-specific nuances.
%In essence, the future of LM4Code lies in achieving a fine balance: broadening its horizon for a wide array of applications while nurturing and integrating domain-specific knowledge for those specialized use-cases where expertise can make all the difference.
%信息利用: 语法、语义信息、结构信息、自然性(cos相似度)、专业知识
%\subsubsection{Delving Deep into the Multidimensional Information.}
%The complexity of coding goes beyond mere textual representation. Within code lies a myriad of information dimensions, presenting both challenges and opportunities for LM4CODE. For effective code handling, the model must seamlessly integrate and interpret these diverse information resources.
%Syntax information ensures the correctness of the code; only with meticulous syntax can a program run smoothly. Concurrently, LM4Code needs to delve into the semantic layer of the code, guaranteeing outputs that are not only logically structured but also accurately mirror the developer's original intent.
%The structural essence of code reflects its inherent logic, such as loops, conditional statements, and function calls. The naturalness and readability of the code are equally crucial, and measuring using cos similarity can further enhance the fluidity and maintainability of the code.
%Among these dimensions, the integration of professional knowledge is paramount. LM4Code should be adept at identifying and employing best practices within the domain, ensuring the generated code is both accurate and efficient.
%We believe that by fully harnessing these multidimensional information resources, LM4Code can achieve unparalleled precision and efficiency in code processing, paving the way for a new era in code generation, repair, and optimization.

%on-device，模型简化、模块化、可重用性、可拆分性，模型迁移（到手机等多种平台），兼容性
%LM4Code的模块化和移动设备适配模型
%\subsubsection{Modular and Mobile-Ready Models for LM4Code}
%With the advancement of technology, LM4Code is confronted with new challenges of adapting across various computational devices. Devices like smartphones, tablets, and edge computing hardware, though constrained by hardware and computational capacities, offer broader deployment opportunities for the model. Running the model directly on these devices enhances response time by eliminating network latency and offers an added layer of data privacy. Executing processes directly on user devices prevents the need to transmit user data to external servers, mitigating risks of data breaches.
%Model simplification, modularity, reusability, and divisibility are pivotal for such multi-platform deployment. They not only lower computational and storage requirements but also allow developers to cherry-pick specific parts of the model based on the application's demands.
%To truly harness the opportunities of cross-platform deployment, there's a need for research and development of effective model migration strategies, ensuring that LM4Code models don't suffer significant performance degradation when transitioning from one platform to another. As these techniques continue to innovate and optimize, we anticipate a widespread application of LM4Code across diverse devices, opening new avenues for applications and commercial opportunities.

%Model Adaptability and Generalization
%通用模型的问题：提出统治所有任务的万能模型是有挑战性的。
%模型在不同的编程语言或域之间的知识转移挑战。
%对新的恶意软件家族或新的攻击方法的适应性问题。
%OOV问题：由于存在低频率和项目特定的令牌，NMT修复方法通常面临OOV问题的挑战。

%Model Opacity and Explanation Difficulty
%深度学习模型的不透明性：无法解释为什么模型会认为某个标记比其他标记更重要。
%深度学习模型的黑盒性：难以区分有用和误导的标识符对模型性能的影响。
%如何完全理解深度学习模型的工作原理。

%Testing and Evaluation
%完整系统的挑战：完整的系统需要整合错误定位和改进的测试装置进行评估。
%句子相似性的评估：对于诸如神经机器翻译和图像字幕等任务来说，评估两句话之间的相似性一直是一个艰巨的挑战。
%测试或acles的合成：合成功能oracles是一个众所周知的挑战性问题。
%缺乏高质量的、大规模的评估数据集。

%Model Design and Optimization
%平衡模型性能和计算资源需求。
%动态与静态分析：有其各自的优势和弱点。
%鲁棒优化的实际挑战：在源代码领域解决鲁棒优化目标尤为困难。
%负优化问题：模型优化的目标是降低学习成本和资源消耗，但这可能会牺牲模型的性能和准确性。
%大型语言模型的精炼：保留从大模型中提炼的知识是一项挑战。

%Data-related Issues
%数据收集：对于SE任务来说，收集大规模、高质量的数据集可能会很困难。
%如何从有毒数据中学习和提取有用的知识。
%数据集的清洁性：提出一个可以构建清洁数据集的数据收集方法是极为困难的，如果不是不可能的。
%OOV问题：由于存在低频率和项目特定的令牌，NMT修复方法通常面临OOV问题的挑战。
%交叉功能泛化的研究方向：需要解决OOV问题、探索更好的模型结构、利用大量无标签代码片段进行无监督或半监督学习。

%Attacks and Security
%面对对抗性攻击的挑战，尤其是针对代码的攻击。
%深度学习模型的非稳定性和脆弱性。

%Task-specific Issues
%可扩展性：查询LLM集合对于大量开发者可能无法扩展。
%深度学习对于代码生成的自然语言理解：计算机难以完全理解自然语言，这可能是代码生成的主要障碍。
%编程语言的结构化特性：带来了新的挑战。
%代码补全的挑战：正确建议标识符在现有的代码补全研究中是具有挑战性的。
%代码修复的复杂性：代码作者在修改代码时可能引入新的缺陷。



\begin{figure}[t]
  \centering
  \begin{minipage}{0.5\linewidth}
    \centering
    \includegraphics[height=3.5cm, keepaspectratio]{images/design/fig5_stage3_model_bias_distri_time.pdf} 
    \caption{Paper distribution across time (Section~\ref{sec:system_design}) }
    \label{fig:result_stage2_model_bias_time}
  \end{minipage}%
  \hfill
  \begin{minipage}{0.5\linewidth} 
    \centering
    \includegraphics[height=3.5cm, keepaspectratio]{images/design/fig5_stage3_model_bias_distri_models.pdf}
    \caption{Distribution of LMs (Section~\ref{sec:system_design}) }
    \label{fig:result_stage2_model_bias_models}
  \end{minipage}
\end{figure}



==> tables/Data_Extraction.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table}[ht]
  \centering
  \caption{Extracted Data Items and Related Research Questions}
    \begin{tabular}{r|l}
    \toprule
    \textbf{RQ} & \multicolumn{1}{c}{\textbf{Data Item}} \\
    \midrule
    1,2,3,4 & The category and stage of SE task \\
    1,2,3,4 & The category of LM \\
    1,2,3 & The type of bias and its impact \\
    1,2,3 & The factor of the bias and is it solved \\
    2,3   & The XAI proposed in the solution \\
    2,3,4 & The Attack method proposed in the solution \\
    2,3,4 & The RQs, main findings, and challenges proposed \\
    4     & The dataset and code source \\
    \bottomrule
    \end{tabular}
  \label{tab:Data_extraction}%
\end{table}%


==> tables/tab_evaluate_bias_papers.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[t]
  \centering
  \resizebox{\linewidth}{!}{
    \begin{tabular}{ll}
    \toprule
     & \multicolumn{1}{c}{\textbf{Paper}} \\
    \midrule
    \textbf{Inappropriate Baseline} & \cite{liu2023towards} \\
    \midrule
    \textbf{Inappropriate Test Set} & \cite{liu_deep_2022,liu_cd-vuld_2022,nong_generating_2022,zeng_deep_2021} \\
    \midrule
    \textbf{Low Reproducibility} & \cite{zeng_extensive_2022} \\
    \midrule
    \textbf{Inappropriate Performance Measures} & \cite{chakraborty2021deep,wan_improving_2018,liu_multi-task_2021,yedida2021value,ding_patching_2021,ahmed_synshine_2023,dong2023revisiting,zhu2023tare,wu2023effective,liu2023towards,dakhel2023github,thongtanunam_autotransform_2022,gao2023keeping,liu2023syntax} \\
    \bottomrule
    \end{tabular}%
    }
     \caption{Summary of Common Biases in Performance Evaluation from Reviewed Research Studies}
     \label{tab:bias_in_evaluation}%
\end{table}%

==> tables/tab_evaluate_bias_summary.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet5'
\begin{table}[t]
  \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{llp{12em}p{20em}p{20em}}
    \toprule
    \textbf{Bias Type} & \multicolumn{1}{c}{\textbf{Paper}} & \multicolumn{1}{c}{\textbf{SE Tasks}} & \textbf{Description} & \textbf{Implications} \\
    \midrule
    \textbf{Inappropriate Baseline} & \cite{liu2023towards} & Test Generation & Lacking a straightforward baseline & 61\% of the bugs can be found by the straightforward baseline NoException with twice the Precision, and 4.7 bugs found by NoException cannot be found by TOGA. \\
    \midrule
    \multirow{4}[8]{*}{\textbf{Inappropriate Test Set}} & \cite{liu_deep_2022} & Code Generation & Test set is small and not diverse & (existing datasets ->new dataset) =>  BLEU: reduced significantly from 0.811 (on Django) and 0.646 (on HS) to 0.167. The reduction is up to 79\% and 75\% \\
\cmidrule{2-5}      & \cite{liu_cd-vuld_2022} & Vulnerability Detection & The test data often differs from the training data in terms of distribution (different projects, differ in the types of vulnerability) & CD-VulD-> 0.83 F1 scores (every vulnerability types)\newline{}VulDeePecker + MTLF -> 0.615 F1 measure \\
\cmidrule{2-5}      & \cite{nong_generating_2022} & Vulnerability Detection & Lacking large-scale and realistic datasets & new dataset -> improvements (by up to 49.51\% in F1-score), much higher than (up to 10.40\%) the same number of synthetic samples, lower than (up to 68.76\%) real-world samples \\
\cmidrule{2-5}    & \cite{zeng_deep_2021} & Defect Prediction & Limited dataset with marginal improvements (around 7\% in terms of the AUC score); a decreased performance when switching to cross-project validation & AUC loss (within-project => cross-project prediction) -> (-3.63\%, -4.03\%) for two recent deep learning approaches \\
\midrule
\textbf{Low Reproducibility} & \cite{zeng_extensive_2022} & Defect Detection, Clone Detection, Code Search, Code Summarization, Program Repair, Code Translation, Code Generation & Pre-trained models seldom follow equivalent evaluation protocols (hardly evaluated on the identical benchmarks, tasks, or settings) & / \\
\midrule
\multirow{14}[28]{*}{\textbf{Inappropriate Performance Measures}} & \cite{chakraborty2021deep} & Vulnerability Detection & Class imbalance problem of real-world vulnerability distribution, leading to bad performance & Real-world vulnerability-> drop by more than 50\% \\
\cmidrule{2-5}      & \cite{wan_improving_2018} & Code Summarization, Code Representation & Code length affect the representation of code and the comment length affect the performance of text generation & BLEU-1: 0.2527, best baseline 0.1887 \\
\cmidrule{2-5}      & \cite{liu_multi-task_2021} & Code Completion & Models perform poor on completing identifiers, and the type information of the identifiers & accuracy  (84.06\% and 55.19\%) outperforms best Transformer-XL (72.12\% and 43.63\%) \\
\cmidrule{2-5}      & \cite{yedida2021value} & Defect Prediction & Class imbalance is a problem for deep learners & \multicolumn{1}{l}{} \\
\cmidrule{2-5}      & \cite{ding_patching_2021} & Program Repair & Transformers struggle to model very long sequences as their memory usage increases quadratically with sequence length. & \multicolumn{1}{l}{} \\
\cmidrule{2-5}      & \cite{ahmed_synshine_2023} & Program Repair & Token length,  don’t work as well even for moderately longer programs,  error types like keyword or operator & Token Range (1-100) -> (901-1000) => 82.28\% -> 55.00\% \\
\cmidrule{2-5}      & \cite{dong2023revisiting} & Code Review & Pattern Ratio Distribution, (~90\%) of their generated commit messages belong to simple patterns & \multicolumn{1}{l}{} \\
\cmidrule{2-5}      & \cite{zhu2023tare} & Program Repair & generating lots of untypable patches\newline{}the existing models do not consider the constraints of code captured by a set of typing rules & Tare achieves 44.7\% improvement over Recoder \\
\cmidrule{2-5}      & \cite{wu2023effective} & Program Repair & compilation rate & Codex has the highest compilation rate of 79.7\%. Others have low compilation rates (the lowest being 6.4\% with CodeT5 and the rest between 24.5\% to 65.2\%) \\
\cmidrule{2-5}      & \cite{liu2023towards} & Test Generation & FPR (False Positive Rate) is not a realistic evaluation metric and the Precision of TOGA is only 0.38\% & \multicolumn{1}{l}{} \\
\cmidrule{2-5}      & \cite{dakhel2023github} & Code Generation & Copilot has some difficulties in combining multiple methods to generate a solution & \multicolumn{1}{l}{} \\
\cmidrule{2-5}      & \cite{thongtanunam_autotransform_2022} & Code Review & for future tokens and identifiers & AutoTransform can correctly transform 353 methods, which is 67\% higher than the prior work \\
\cmidrule{2-5}      & \cite{gao2023keeping} & Code Summarization, Vulnerability Detection, Clone Detection & forget knowledge learned from previous datasets when learning from the new dataset & BLEU-4 and F1 score drop by 7.46 and 33.28 on two tasks on the first dataset (after training on the fifth dataset) \\
\cmidrule{2-5}      & \cite{liu2023syntax} & Code Translation & perform poorly on unseen language tanslation scenarios & zero EM Acc and a low BLEU score. \\
    

    \bottomrule
    \end{tabular}
}
  \caption{Summary of Common Biases in Performance Evaluation from Reviewed Research Studies}
  \label{tab:bias_in_evaluation}%
\end{table}%
    




==> tables/tab_model_bias_summary.tex <==
\begin{table}[t]
  \centering
  \resizebox{\linewidth}{!}{
    \begin{tabular}{llp{11.82em}p{21.68em}l}
    \toprule
    \textbf{Bias Type} & \multicolumn{1}{c}{\textbf{Paper}} & \multicolumn{1}{c}{\textbf{SE Tasks}} & \multicolumn{1}{c}{\textbf{Description}} & \multicolumn{1}{c}{\textbf{Implications}} \\
    \midrule
    \multirow{6}[12]{*}{\textbf{Data Snooping}} 
                    & \cite{liu_can_2021} & Clone Detection & The functionality overlap between training set and test set & \multicolumn{1}{p{22em}}{F1 score can increase from 0.42 to 0.96 when training data are collected from the same functionality group as the test set} \\
\cmidrule{2-5}      
                    & \cite{ding_patching_2021} & Program Repair & The training data contains many “similar" bugs to those seen at test time & \multicolumn{1}{p{22em}}{/} \\
\cmidrule{2-5}      
                    & \cite{steenhoek2023empirical} & Vulnerability Detection & Traing and test samples can originate from the same projects & \multicolumn{1}{p{22em}}{The data split setting of mixed-projects perform significantly better than cross-projects for all the models, where the average and the largest differences in F1 score were 0.11 and 0.32 respectively} \\
\cmidrule{2-5}      
                    & \cite{wu2023effective} & Program Repair & Vulnerabilities in the public datasets might have been included in the training data & \multicolumn{1}{p{22em}}{/} \\
\cmidrule{2-5}      
                    & \cite{liu2023towards} & Test Generation & Generating test prefixes from bug-fixed program versions & \multicolumn{1}{p{22em}}{Inflates the number of bugs found by the state-of-the-art NTOG approach TOGA by 61.8\%} \\
\cmidrule{2-5}      
                    & \cite{shi2022evaluation} & Code summarization & Code from the same class/project exist in both training and test set & \multicolumn{1}{p{22em}}{BLUE scores can be increased by 18.51/6.66, 11.3/6.66, and 10.96/18.07 on different split settings and datasets} \\
    \midrule
    \multicolumn{1}{l}{\multirow{10}[20]{*}{\textbf{Spurious Correlations}}}    
                    & \cite{steenhoek2023empirical} & Vulnerability Detection & The models try to capture patterns of a vulnerability, instead of reasoning about the values, and have difficulty capturing long range semantic dependencies in the code. & \multicolumn{1}{p{22em}}{Among all the features, error, print, and alloc ranked the highest ratios, where the I/F is 2.79, 1.78, 1.52, respetively} \\
\cmidrule{2-5}      
                    & \cite{paltenghi_thinking_2021} & Code Summarization & The regular attention of models is mostly uncorrelated with human attention, e.g., strings are important to humans but mostly ignored by models. & \multicolumn{1}{p{22em}}{Models often struggle to predict more challenging kinds of methods, such as checkers and test methods, where the average F1 score is lower than 0.4.}  \\
\cmidrule{2-5}        
                    & \cite{zhang_diet_2022} & Code Search, Code Summarization & CodeBERT focuses on keywords and data-relevant statements such as method signatures and return statements, which can be useless for downstream tasks & \multicolumn{1}{p{22em}}{Achieving comparable results while taking 40\% less computational cost in fine-tuning and testing if input programs are simplified} \\
\cmidrule{2-5}      
                    & \cite{dong2023revisiting} & Code Review & The majority (˜90\%) of generated commit messages fit with a few simple patterns & \multicolumn{1}{p{22em}}{Many generated commit messages fitting with patterns would be wrong and they should belong to non-pattern.} \\
\cmidrule{2-5}      
                    & \cite{chakraborty2021deep} & Vulnerability Detection & Learning unrelated artifacts from the dataset (e.g., specific variable/function names, etc.) instead of the actual cause of the vulnerabilities & / \\
    %\midrule
    % \multicolumn{1}{p{11.775em}}{\textbf{Inappropriate Data Proprocessing}} 
    %                 & \cite{chakraborty2021deep} & Vulnerability Detection & slicing and pre-processing techniques introduce data duplicates &  \\
    \midrule
    \multirow{8}[16]{*}{\textbf{Inappropriate Model Design}} 
                    & \cite{chakraborty2021deep} & Vulnerability Detection & All the existing approaches exhibit a significant degree of overlap in the feature space between classes & \multicolumn{1}{p{22em}}{Leaving room for 33.57\% precision improvement and 128.38\% recall boost over state-of-the-art} \\
\cmidrule{2-5}      
                    & \cite{wang_enhancing_2023} & Code Search & DNN-based techniques capture lexical-, control structure-, or data flow-level information of binary code for representation learning, which is often too coarse-grained and does not accurately denote program functionality & \multicolumn{1}{p{22em}}{Under-constrained symbolic execution can boost the MRR accuracy by 17.2\%~37.9\%} \\
\cmidrule{2-5}      
                    & \cite{wan_improving_2018} & Code Summarization & Encoder-decoder framework suffers from two drawbacks: the encoder ignores the tree structure of code; the decoder cannot generate entire sequences & \multicolumn{1}{p{22em}}{Actor-critic network can boost the BLUE-1 perfomance by 33.2\%~53.2\% } \\
\cmidrule{2-5}      
                    & \cite{ding_patching_2021} & Program Repair & Program repair suffers from design decisions built into neural machine translation (NMT) models, both in terms of translation accuracy and diversity & \multicolumn{1}{p{22em}}{Complete repair prediction accuracy reaches just 4.5\% after 10 epochs, making nearly all its substantial progress afterwards} \\
\cmidrule{2-5}      
                    & \cite{wang_reinforcement-learning-guided_2022} & Code Summarization & Code representation ignores code hierarchy; the encoder ignores correlations between comments and code; the decoder trained to predict subsequent words instead of the entire word sequence  & \multicolumn{1}{p{22em}}{Deep reinforcement learning (DRL) framework improves the baselines by around 22\%~45\% in BLEU-1} \\
\cmidrule{2-5}      
                    & \cite{lin2022xcode} & Code Translation, Clone Detection, Code Search & The structural differences among programming languages make it more difficult to process multiple languages in a single neural architecture & \multicolumn{1}{p{22em}}{Shared Encoder-Decoder (SED) architecture outperforms the baseline by more than 20\% in accuracy@1 and accuracy@5.} \\
\cmidrule{2-5}      
                    & \cite{fang2023representthemall} & Bug Report Summarization, Duplicate Bug Report Detection, Vulnerability Detection & Training multiple models for multiple downstream tasks faces three issues: complexity, cost, and compatibility, due to the customization, disparity, and uniqueness of these automated approaches & \multicolumn{1}{p{22em}}{The pre-trained approach can bring 3.39~12.42 points improvement in F1-score and 3.59~13.89 points improvement in accuracy} \\
\cmidrule{2-5}      
                    & \cite{meng2023template} & Program Repair & NMT-based methods generate the small range of fixed code for better performance and may suffer from the OOV (Out-of-vocabulary) problem & \multicolumn{1}{p{22em}}{The combination of template-based and NMT- based methods is able to fix 12 more bugs on Defects4J-v1.2 dataset (79 in total)} \\

    \bottomrule
    \end{tabular}%
}
  \caption{Summary of Common Biases in System Design and Learning from Reviewed Research Studies}
  \label{tab:bias_in_model}%
\end{table}%
